Global-to-local Expression-aware Embeddings for Facial Action Unit Detection

Expressions and facial action units (AUs) are two levels of facial behavior descriptors. Expression auxiliary information has been widely used to improve the AU detection performance. However, most existing expression representations can only describe pre-determined discrete categories (e.g., Angry, Disgust, Happy, Sad, etc.) and cannot capture subtle expression transformations like AUs. In this paper, we propose a novel fine-grained \textsl{Global Expression representation Encoder} to capture subtle and continuous facial movements, to promote AU detection. To obtain such a global expression representation, we propose to train an expression embedding model on a large-scale expression dataset according to global expression similarity. Moreover, considering the local definition of AUs, it is essential to extract local AU features. Therefore, we design a \textsl{Local AU Features Module} to generate local facial features for each AU. Specifically, it consists of an AU feature map extractor and a corresponding AU mask extractor. First, the two extractors transform the global expression representation into AU feature maps and masks, respectively. Then, AU feature maps and their corresponding AU masks are multiplied to generate AU masked features focusing on local facial region. Finally, the AU masked features are fed into an AU classifier for judging the AU occurrence. Extensive experiment results demonstrate the superiority of our proposed method. Our method validly outperforms previous works and achieves state-of-the-art performances on widely-used face datasets, including BP4D, DISFA, and BP4D+.

==> abstract_bk.tex <==
\begin{abstract}
Expression and facial action units (AUs) are two levels of facial behavior descriptors. Great efforts have been dedicated to exploiting expression auxiliary information which may improve AU detection performance. However, most of them process expression as a series of predetermined discrete categories (e.g. Angry, Disgust, Happy and Sad, etc.), which just has a coarse-grained perception on full facial movements and is insufficient to capture micro expression transformation like AUs.
\ZH{
Expression and facial action units (AUs) are two levels of facial behavior descriptors. Expression auxiliary information has been widely used to improve the AU detection performance. However, most of existing expression representation can only describe predetermined discrete categories (e.g. Angry, Disgust, Happy and Sad, etc.) and cannot capture micro expression transformation like AUs. In this paper, we propose a novel fine-grained expression representation, which can capture subtle and continuous facial movements, to promote AU detection. To obtain such expression representation, we propose to train the expression embedding model on a large scale expression dataset using expression similarity learning strategy.

Moreover, due to the local definition of AUs, it is also essential to extract local AU features. To this end, we design a Facial Component Module (FCM) to generate local facial representation for each AU. Specifically, FCM consists of a facial feature decoder and a facial mask decoder, which can transfer the global expression representation into local facial features and local attention, respectively. A series of AU-specific local components are generated by multiplying facial features and attention. For each component, an AU classifier is further employed to extract AU-related feature and predict the results. In addition, an image reconstruction task is introduced to ensure that the generated facial components deposit the complete face information. Extensive experiments results demonstrate the superiority of the proposed method. Our framework can generated irregular attention regions highly related to each AU and works well on unseen data. It validly outperforms previous works and achieves new state-of-the-art performance on BP4D, DISFA and BP4D+.
} 

In this paper, we propose a novel end-to-end deep learning network utilizing expression similarity to enhance the global fine-grained expression perception ability, which has not been explored before for AU detection. In particularly, we pretrain a global facial feature encoder on a large scale expression dataset by expression similarity learning with triplet loss, and then decode its outputs with two branches of decoders capturing local attention and feature maps respectively. %Specially, to get better AU-related attention and feature maps, we project the global facial expression representation to \ZH{resolution or dimension} a high-dimensional space that is conducive to enlarge local facial details. 
A series of AU-specific local components (local feature maps) are generated by pixel-wise production on the outputs of the two decoders. In addition, an image reconstruction task is designed for reserving facial information as much as possible. Extensive experiments results demonstrate the superiority of the proposed method. Our framework can generated irregular attention regions highly related to each AU and works well on unseen data. It validly outperforms previous works and achieves new state-of-the-art performance on three benchmarks of BP4D, DISFA and BP4D+.

%Expression and facial action units(AUs) are two levels of facial behavior descriptors. Great efforts have been dedicated to exploiting expression auxiliary information which may improve AU detection performance. However, most of them process expression as a series of predetermined discrete categories (\textcolor{red}{e.g. xxx}), which just has a global coarse-grained perception on full facial movements and is insufficient to capture micro expression transformation like AUs. Precise local features have been demonstrated to be crucial for AU detection, which can be decoded from the global expression representation theoretically. In this paper, we propose a novel end to end deep learning network utilizing expression similarity learning task to enhance the global fine-grained expression perception ability, which has not been explored before. In particular, we pretrained the global facial feature encoder on a large scale expression dataset by expression similarity learning with triplet loss, and then decoded its outputs with two branches of decoders capturing local attention and feature maps respectively. Specially, to get better AU-related attention and feature maps, we project the global facial expression representation to a high-dimensional space which is conducive to enlarge local facial details. A series of AU-specific local components(local feature maps) are generated by pixel-wise production on the outputs of the two decoders. In addition, an image reconstruction task is designed for reserving facial information as much as possible. Extensive experiments results demonstrate the superiority of the proposed method. Our framework can generated irregular attention regions highly related to each AU and works well on unseen data. It validly outperforms previous works and achieves new state-of-art performance on three benchmarks of BP4D, DISFA and BP4D+.
\end{abstract}

==> acknowledgments.tex <==
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi

==> exoeriment_bk.tex <==
\section{Experiments}



% \begin{table*}[!t]
% %\small
% \footnotesize
% \setlength{\tabcolsep}{2pt}
% \renewcommand\arraystretch{1.5} 
% \centering
% {
%   \caption{Ablation study on BP4D measured by F1 scores (\%).}
%   \vspace{-1em}
%   \label{tab:F1 on Ablation}
%  \begin{tabular}{l|cccccccccccc|c}
%     \hline
%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Classifier} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{Position-Encoding} &\textbf{F1-Score} \\[1pt]
%     \hline\hline
%     Baseline        &- &- &$\surd$  &- &- &- &52.6\\
%     Baseline-ImageNet         &$\surd$ &- &$\surd$ &- &- &- &61.6 \\
%     Baseline-FEC         &- &$\surd$ &$\surd$ &- &- &- &63.3 \\
%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &$\surd$ &- &- &63.8 \\
%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &$\surd$ &- &- &64.0 \\
%     Baseline-FEC-DF-DM       &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &- &66.3 \\
%     Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\
%     \hline
%   \end{tabular}}
% \end{table*}

\begin{table*}[!t]
%\small
\footnotesize
\setlength{\tabcolsep}{8pt}
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Ablation study on BP4D measured by F1 scores (\%).}
  \vspace{-1em}
  \label{tab:F1 on Ablation}
 \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{F1-Score} \\[1pt]
    \hline\hline
    Baseline        &- &-  &- &- &52.6\\
    Baseline-ImageNet         &$\surd$ &- &- &- &61.6 \\
    Baseline-FEC         &- &$\surd$ &- &- &63.3 \\
    Baseline-FEC-DF          &- &$\surd$ &$\surd$ &- &63.8 \\
    Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &- &64.0 \\
    Baseline-FEC-DF-DM       &- &$\surd$ &$\surd$ &$\surd$ &66.3 \\
    % Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\
    \hline
  \end{tabular}}
\end{table*}



%To validate our proposed method, the evaluation is conducted on three public datasets commonly-used for AU detection. These datasets contain face expression images with manually-annotated action unit labels. For fair comparisons, our evaluation follows the prior works, using three-fold cross validation. The reported results are the averages from three-fold experiments. This section introduces the detail experiment settings, evaluate the effectiveness on each module, and visualize the intermediate results generated by the framework at last.

This section reports extensive experiments to verify the effectiveness of our proposed method. These experiments are conducted on three public benchmarks commonly-used for AU detection, all of which contain face expression images with manually-annotated action unit labels. 

We first introduce the above three datasets in detail, then display the implementation details of the whole training and validation progress. Furthermore, we compare our method with previous start-of-the-art methods and demonstrates its superiority. For fair comparisons, our evaluation follows the prior works \cite{li2018eac}\cite{shao2021jaa}, using three-fold cross validation. 
%The specific three-fold data is proposed by previous works (See below).
%F1 score is utilized as the metric to quantify the AU detection performance. %v(需要考虑下，是否在这里提F1，因为看到后面有对F1的定义解释)
%anrudong:已删除该句
The reported results are the averages from three-fold experiments. For the purpose of further getting insight into our method, we designed intensive experiments to observe the 
impact of the built sub-modules. Finally, we visualize several samples to further verify the validity of our proposed ideas.

% -datasets
% - impletmenttation dedails
% - results, validate our method by comparing with baselines
% - further to get insight to our method, validate our careful-designe, ablation study...
% - visual reatuls


\subsection{Datasets}
As mentioned above, the evaluation is performed on three widely-used AU detection datasets: BP4D \cite{BP4D}, DISFA \cite{MavadatiDISFA}, and BP4D+ \cite{zhang2016multimodal}. All the above datasets are annotated with AU labels by certified experts for each frame.

%可以展开说下标注过程，比如观看视频，还是观察单帧，等等。如果标注过程没有区别，那么就集中写在前面，否则可以写在每个数据集文字内部。
%anrudong: 三个数据集均在视频序列上逐帧进行标注，标注方式写在了每个数据集各自的介绍部分
%yuding: 是的，我知道，需要在前面整体说一下三个数据集的共性和区别（概括说就好），说了之后，你再分数据集单独说，读者读起来就顺，知道下面三个数据集是在对上面共性和差异性的展开。如果不说，下面三个数据集就像三块砖头摆在那里，没有语言把它们拎起来。
\textbf{BP4D} consists of 328 video clips from 41 participants (23 females and 18 males). Each video frame is annotated with the occurrence or absence of 12 AUs(1,2,4,6,7,10,
12,14,15,17,23,24). In total, about 140,000 frames were annotated frame-by-frame by a team of experts. Following the same subject division \cite{li2018eac}\cite{shao2021jaa}, we perform three-fold subject exclusive cross validation for all experiments.
%（哪12个，列出来，AU1, AU2,...AU12。可以提供一张图把三个数据集涉及到的所有AU的样例图都集中画出来，让读者看起来舒服，能快速明白AU对应是哪一个）.

\textbf{DISFA} contains 27 video clips from 27 participants (12 females and 15 males). Each video records facial activity of a participant when watching a 4-minutes video clip. Each clip is consisted of 4845 frames evenly. Altogether around 130,000 frames are annotated with intensities from 0 to 5. Following previous works \cite{jacob2021facial}\cite{li2018eac}\cite{shao2021jaa}\cite{yang2021exploiting}, we regard intensity labels $\{0,1\}$ as absence and others as presence. The evaluation is performed on 8 AUs(1,2,4,6,9,12,25,26). We also perform the same three-fold subject exclusive cross validation on 8 AUs as prior works \cite{li2018eac}\cite{shao2021jaa}.% following the subject division of \cite{li2018eac, shao2021jaa}.

\textbf{BP4D+} contains 1400 video clips from 140 participants (82 females and 58 males). Compared to BP4D, it has larger identity variations and video numbers. About 198,000 frames are annotated with the same 12 AUs in BP4D. We perform subject exclusive three-fold cross validation to compare with the state-of-the-art. Besides, to evaluate the generalization performance, the proposed method is trained on BP4D and then evaluated on BP4D+, following the works \cite{attnetionTrans2019}\cite{shao2021jaa}.

To sum up, the order from largest to smallest of the three datasets is BP4D+, BP4D and DISFA. BP4D and BP4D+ were recorded in similar shooting environment and illumination condition. Both of them share the same 12 AU species. In comparision, DISFA is the smallest dataset containing only 8 AU class, and was captured in \textcolor{red}{a quite different environment.}

%以上是列举了三个数据，接下来可以做一个数据集的总结，比如说从数据量来说，xxx最少，xxx居中，最多是xxxx。也包括AU的个数也可以提一下，这里重在讲三个数据集的区别。这样方便后面实验讨论，比如我们工作可能在数据量大的数据集上表现好，等等，分析讨论结果的时候可以到这里来找理由，找依据。
\begin{table*}[!t]
%\small
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Ablation study on BP4D measured by F1 scores (\%). }
  \vspace{-1em}
  \label{tab:F1 on Ablation 2}
 \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline\hline
    
    w/o pretrain &34.9 &24.2 &36.7 &76.1 &71.4 &81.0 &86.3 &58.7 &25.9 &51.9 &27.4 &31.6 &50.5\\
    w. fixed FE &52.3 &45.8 &59.8 &[79.4] &78.1 &\textbf{84.8} &89.0 &64.0 &46.5 &64.0 &38.6 &49.8 &63.5\\
    
    \hline
    w. ResNet &[56.9] &46.5 &57.2 &78.1 &[79.2] &84.2 &87.9 &63.8 &51.0 &64.7 &49.5 &[53.5] &[64.4]\\
    w/o DM  &53.3 &44.2 &58.7 &78.6 &76.9 &83.9 &[89.8] &62.2 &48.9 &65.1 &[52.5] &51.8 &63.8\\
    w/o DM\&DF &55.4 &\textbf{65.1} &\textbf{73.9} &49.0 &46.9 &77.1 &\textbf{92.9} &54.1 &48.1 &64.7 &[52.5] &47.5 &63.3\\
    w. PE & 54.8 &45.3 &[63.4] &78.4 &79.1 &[84.6] &89.1 &60.7 &49.7 &64.2 &50.7 &50.3 & 64.2\\
    
    \hline
    w. None & 53.7 &44.6 &55.4 &78.6 &78.4 &83.7 &89.2 &[64.6] &[51.4] &\textbf{65.9} &51.2 &52.6 &64.1\\
    w. SoftMax & 53.6 &43.8 &58.5 &\textbf{79.7} &[79.2] &84.5 &89.6 &63.4 &50.3 &62.7 &50.8 &53.0 &64.0\\
    w. Tanh &55.1 &46.2 &60.2 &79.1 &\textbf{79.3} &84.6 &88.6 &63.0 &49.6 &[65.3] &51.8 &50.2 &[64.4]\\ 
  
    \hline
    GLEE-Net (Full) &\textbf{58.2} &[48.7] &61.5 &78.7 &[79.2] &84.2 &[89.8] &\textbf{66.3} &\textbf{56.7} &64.8 &\textbf{53.5} &\textbf{53.6} &\textbf{66.3}\\
    %GLEE-Net (Full) & 53.7 &[48.4] & 59.8 & \textbf{79.7} & 78.9 &83.5 & 89.5 &\textbf{64.0} &[50.6] &64.1 &50.2 &[53.4] &\textbf{64.7}\\
    \hline
  \end{tabular}}
\end{table*}

%%%%%%%%%%%%%pipeline figure
\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/sample1.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the decoded mask attention map. Left: Samples of DISFA, learned masks(odd lines) and display on corresponding face images(even lines). Right: Samples of BP4D and BP4D+.}
    \label{fig:figure1}
\end{figure}
%%%%%%%%%%%%%

\subsection{Implementation Detalis}
Face images are first aligned and cropped according to landmark detection result. Before fedding to our network, the input images are resized to $256\times256$. The resolution of feature map is reduced to $16\times16$ after passing through the Feature Encoder.

In order to utilize the feature extraction ability of low-level convolution layers, the Feature Encoder is initialized with corresponding pretrained network parameters(ImageNet or FEC), and the rest of our networks are set to Kaiming initialization. Except for the Mask Decoder, the whole model parameters are updated by employing an Adam optimizer with hyper-parameters $\beta = 0.9$ and weight decay $10^{-6}$.
%可能要斟酌一下要不要写MaskDecoder部分参数冻结，要写的话如何说清和证明它的作用

The network is trained for 20 epochs with initial learning rate $10^{-5}$ on each dataset fold. The mini-batch size is set to 10. We use a warmup stage with $10^3$ step and then decay the learning rate exponentially with an exponent $-0.5$. The training and inference pipelines are implemented in Pytorch on 4 GeForce GTX 2080ti GPU. 
%这里就可以给一张训练集和验证集，随着时间，收敛的情况，可以分AU来说，我们也可以观察下，哪些AU收敛快，哪些慢，哪些容易过拟合，哪些比较好泛化，等等，这个图都是可以用来分析后面的实验结果，避免实验结果太干涩，没话说。


\subsection{Comparison with the State-of-the-Art}
We first compare our method with the state-of-the-art ones. The compared methods include LSVM \cite{LSVM}, JPML \cite{JPML}, DRML \cite{DRML}, APL \cite{LP48}, EAC-Net \cite{li2018eac}, DSIN \cite{LP8}, ARL \cite{attnetionTrans2019}, SRERL \cite{SRERL},AU-GCN\cite{liu2020relation},AU-RCNN\cite{ma2019r}, ML-GCN \cite{chen2019multi}, MS-CAM \cite{you2020cross}, LP-Net \cite{LP}, FACS3D-Net \cite{yang2019facs3d}, UGN-B \cite{song2021uncertain}, J{\^A}A-Net \cite{shao2021jaa}, MHSA-FFN \cite{jacob2021facial}, SEV-Net \cite{yang2021exploiting}, HMP-PS \cite{song2021hybrid}, D-PAttNe$t^{tt}$\cite{Onal2019D-PAttNet} and CaFNet\cite{chen2021cafgraph}. Among the above methods, 
EAC-Net, ARL , J{\^A}A-Net and SEV-Net were evaluated on all three datasets. D-PAttNe$t^{tt}$ was evaluated only on BP4D. FACS3D-Net, ML-DCN and MS-CAM were evaluated merely on BP4D+. The rest works were evaluated on both BP4D and DISFA.  %这里就可以说下，哪些方法是在三个数据集上测试，哪些仅仅是两个数据，这些都是为后面分数据集汇报结果准备，避免人家说，为什么不同数据集，baseline方法却不一样。

%%%%%%%%%%%%%mask figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample2.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of mask attention maps(odd lines) and displays on corresponding input images(even lines) in BP4D. The first column is different expression faces images. We can observe that similar AU-related local mask distribution can be learned by our framework even though the identity and expression vary dramatically.  }
    \label{fig:mask visualization}
\end{figure*}
%%%%%%%%%%%%%

Following the experimental settings of most previous works, we also employ the F1 score \cite{F1} on the frame level as the evaluation metric. F1-score is a harmonic mean of precision(P) and recall(R), which is defined as $F1 = 2PR/(P+R)$. Since F1-score takes both false positives and false negatives into account, it reflects a more rational measurement of model's performance than accuracy, especially on datasets of uneven class distribution like BP4D, DISFA and BP4D+.

\textbf{Evaluation on BP4D.}
The results on BP4D are shown in Table \ref{tab:F1 on Bp4D}. The average F1 score of our method is 66.3\%, which significantly outperforms all the other competing methods, improving about 1.4\% compared with the second highest one, CaFNet. In terms of the performance on single AUs, our work achieves the highest F1 score among all the methods on 5(AU1,AU4,AU12,AU15 and AU23) and second highest on 2(AU7 and AU17) of the 12 evaluated AUs, showing around 4\% superiority on AU15 and AU23 than the second highest ones. 

Compared with the EAC-Net, ARL and JAA-Net, which also utilize attention mechanism, our method gets improvements of 10.4\%, 5.2\% and 3.9\% separately. In terms of AU feature learning, our method outperform JMPL, DRML and D-PAttNe$t^{tt}$ about 20.4\%, 18\% and 1.6\%, demonstrating our method is more superior in AU feature extracting than patch-learning. \textcolor{red}{I think we can improve the structure of the above text.}

%\textcolor{red}{Compared to SEV-Net and J{\^A}A-Net that employ textual embedding and facial landmarks as auxiliary training information, our method obtains better results with the compact expression embedding as prior knowledge. WHAT DO WE WANT TO EXPRESS}



\textbf{Evaluation on DISFA.}
Table \ref{tab:F1 on DISFA} shows the results on DISFA. As we can see, our method achieves the average F1 score of 66.6\%, outperforming all the compared state-of-the-art methods. 

Compared to the most recent works SEV-Net, HMP-PS, MHSA-FFN and CaFNet, our method obtains the improvement of 7.8\%, 5.6\%, 5.1\% and 0.8\%, respectively. Unlike EAC-Net and J{\^A}A-Net which supervised by both AU and landmark labels, our method only utilize AU labels, but still obtains significant improvement of 18.1\% and 3.1\%, demonstrating the effectiveness of our method in AU feature and attention learning. Note that our method doesn't model AU relationship explicitly, but significantly exceeds all relation-based methods like JMPL, DSIN, ARL, AU-GCN and AU-RCNN etc as well.

%As the number of subjects in DISFA is smaller than that of BP4D, \textcolor{red}{most of the previous methods suffer from overfitting to the appearance of training subjects more severely. WHY?} Therefore, benefiting from our identity-independent expression representations, our method achieves an even more significant improvement.

\textbf{Evaluation on BP4D+.}
Table \ref{tab:F1 on ThreeFoldBp4DPlus} shows the results of the three-fold cross validation on BP4D+.
In particular, results of SEV-Net, ML-DCN and MS-CAM are all reported by\cite{yang2021exploiting} while EAC-Net is by\cite{shao2021jaa}. 
Our method achieves the F1 score of 65.7\% and outperforms all the state-of-the-art methods, exceeds SEV-Net over 4.2\%.

To further evaluate the generalization performance on large scale testing identities, we train our method on BP4D and evaluate it on the full BP4D+ of 140 subjects. The results are shown in Table \ref{tab:F1 on Bp4DPlus}. We use the reported results in the work \cite{shao2021jaa} for comparison. Again, our method outperforms all the compared methods under the large-scale cross-dataset evaluation. It proves that our method can extract identity-independent information and generalize well to new identities.



%From the evaluation results on the three datasets, we can see that AU7, AU12 and AU17 rechieve best performances on BP4D, and AU1 and AU2 gets best results on DISFA. 
%综合看三个数据集的结果，可以谈谈哪些AU，我们的方法总是获胜，哪些总是不好，然后可以分析原因。



\subsection{Ablation Study}
%先简要回顾下我们的算法框架，其实有挑选的介绍，然后再说我们要逐一验证这些框架子模块的设计，才进行了ablation study。（提高文章的过度和可读性）
As described in the previous method section, our framework includes a global feature encoder followed by two branches of feature decoders, namely facial image decoder($D_f$) and facial mask decoder($D_m$). The $D_f$ module decode feature map of each action unit and the $D_m$ module is responsible for learning feature mask that filters out the areas irrelevant to current AU. After a point-wise multiplication on the outputs of $D_f$ and $D_m$ modules, we can get the feature map that focuses on AU related local regions.
In this section, we conduct a series of ablation studies to evaluate the effectiveness of each proposed module. 
%We firstly construct a baseline model(Baseline), of which the feature extractor is DLN without pretrained parameters, followed by AU classifiers. Besides,to verify the validity of the pretrained DLN, we replace the baseline feature extractor with InceptionV3 pretrained on ImageNet(Baseline-INC) and DLN pretrained on FEC(Baseline-DLN) . To further validation of, By adding modules on a baseline method, The results shown in Table \ref{tab:F1 on Ablation} are reported . While results in Table \ref{tab:F1 on Ablation 2} are regularized by removing or replacing our full framework' sub-modules.    %既然这里提到了表格4，这里就定义出表格4中各种消融方法的定义
%anrudong: 表格中涉及到的各个消融实验方法的定义下文有分模块详细介绍，如果在这里再写一遍显得有些重复,因此删掉

%%%%%%%%%%%%%avtivation figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample3.pdf}
    %\vspace{-0.5em}
    \caption{Illustration of mask maps generated by different activation functions(Sigmoid, softmax and Tanh from top to bottom) on each AU from BP4D.  The masks of softmax are more sparse that that of Sigmoid and Tanh, because it has extra restriction between AU channels. However, softmax may filters out much of useful regions beneficial for AU detection as well}
    \label{fig:avtivation}
\end{figure*}
%%%%%%%%%%%%%


\textbf{Prior Knowledge.}
\textcolor{red}{here we need a head text to briefly introduce what we will presents.}

We first test the effectiveness of \textcolor{red}{pretrained models}. As illustrated in Table~\ref{tab:F1 on Ablation},  the baseline is constructed based merely on an InceptionResNetV1 network without being pretrained. It has the same structure as the feature encoder of our full network, using the intermediate features which has a resolutioin of 16 x 16. The feature encoder of the baseline is followed by several classifer modules similar to AU Classifer Module. The number of classifier modules is corresponding to the AU classes. Each classifier module predicts a specific AU's probability and shares the same structure that contains 3 CNN layers and a Sigmoid activation at the last layer. Then we test the baseline with pretrained parametes on ImageNet, namely Baseline-ImageNet. As shown in Table \ref{tab:F1 on Ablation}, it achieves 61.6\% and brings over 9\% improvement compared with baseline (52.6\%), proving the importance of pretraining.

To test the effectiveness of our feature encoder pretrained on FEC with facial expression similarity task, we replace it with different architecture or parameters and finetune the whole network on DISFA. As we can see in the Table \ref{tab:F1 on pretrain}, we take ResNet50 and InceptionResNetV1 as the feature encoder of our full network. In each case we use the intermediate features of same resolutioin(16 $\times$ 16). When taking different parameters initialization pretrained on different dataset and task, we get the best result when load our parameters pretrained with expression similarity task, gaining improvement over 3.1\% and 1\% in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet by image classification task. It proves the significance of prior knowledge from the compact expression embedding.
\textcolor{red}{looks no table for the above results. I dont know why the above uses DISFA and teh below uses the other two datsets.}

To futher indicate the significance of the pretrained facial expression embedding network, we also test it on the BP4D dataset. First, we replace the feature encoder with a ResNet~\cite{Resnet34}~(w. ResNet50 in Table~\ref{tab:F1 on Ablation 2}). The results show that using pretrained facial expression embedding network as backbone improves the score by 3\% on BP4D. We also set up an experiment with feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in the Table \ref{tab:F1 on Ablation}. This indicates a domain gap exists between FEC and BP4D datasets.
\textcolor{red}{Any more discussion here?.}
%%%%%%%%%%%%%pose_mask figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample4.pdf}
    %\vspace{-0.5em}
    \caption{Illustration of attention map on different head pose. The Mask Decoder generates  similar masks with various pose images input, demonstrates that the mask decoder is robust to head pose}
    \label{fig:pose_mask}
\end{figure*}
%%%%%%%%%%%%%


\textbf{Facial Components.}
To validate the effectiveness of representations extracted by the Facial Components module, based on the feature encoder pretrained on FEC, we construct the model only with the Feature Encoder ~(w/o MD \& FD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC in Table~\ref{tab:F1 on Ablation}) or the Facial Decoder branch~(w/o MD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation}) individually. A decline of 0.9\% \textcolor{red}{from 0.xx\% to 0.xx\%} is caused when the Mask Decoder is removed (w/o MD) and 1.4\% decline \textcolor{red}{from 0.xx\% to 0.xx\%} when the Facial Decoder is also removed(w/o MD \& FD) respectively. Note that the inclusion of just Facial Decoder brings an improvement by 0.5\% compared with the pre-trained baseline(w/o MD \& FD). The F1-score improves 2.3\% when further add the Mask Decoder module and construct our full network, GLEE-Net. It validates the significance of attention and local feature learning.
% In the experiment without pretraining on the expression dataset~(w/o pretrain), we can see an apparent drop in average F1-score of .


\textbf{Mask Activations. }
We tried different activation methods on the output of Mask Decoder. As expected, the Sigmoid function (GLEE-Net (Full) in Table \ref{tab:F1 on Ablation 2}) gets the best result on BP4D dataset. Softmax(w. SoftMax in Table\ref{tab:F1 on Ablation 2}) achieves F1-score of 64.0\% and Tanh(w. Tanh in Table\ref{tab:F1 on Ablation 2}) 64.4\%. For the reason that mask generated by Softmax tends to get sparse attention map and excludes most other parts, including regions related to the target AU in most cases, it may result in the downstream recognition task unable to learn sufficient information. While Sigmoid avoids above shortcoming and reserves the regions which are closely correlated with the target AU, making the subsequent Classifier Module to have better performance. \textcolor{red}{It looks ignoring Tanh in discussion.}



\subsection{Visual Analysis}
In this section we visualize the feature and mask results of our framework to further validate the effectiveness of our proposed methods.

\textbf{Mask Attention Learning.} Due to the anatomy definition,  each AU is a group of muscle motions and relative to a specific  region in the face. For instance AU1 is  inner brow raising and AU9 is nose wrinkle. Theoretically our framework should learn a regional mask activation map for per AU corresponding to its muscle action. To validate the proposed mask feature learning's effectiveness, we visualize several 
examples of DISFA, BP4D and BP4D+ of their attention mask map learned by our network in Figure~\ref{fig:figure1}, from these samples we can see that the proposed method successfully captures discriminative attention mask for each AU. Taking AU4(brow low) and AU7(lid tight) as example, the learned spatial mask is around the brows and 
lower eyelids respectively, which proves that our proposed mask decoder is effective for AU related local regional attention learning.

From the Figure~\ref{fig:mask visualization} we can see that each AU's mask is closely relative to it's muscle region, even for various expressions such as happy, sad and fear.
It also can be seen that several different AUs cover similar area. This is attributed to that different AUs may share same or similar muscle distribution. For instance, AU1, AU2 and AU4 are involved with forehead,  while AU14, AU15,AU17 AU23 and AU24 are all closely related to mouth area. Besides, take the mutual relation of various action units into consideration, the mask learned merely supervised by AU labels will include other facial region of correlative AU in nature. For instance, masks of AU1, AU2 and AU4 not only covers region of brows, but also contains areas around mouth.

%%%%%%%%%%%%%tsne figure
\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/tsne.pdf}
    %\vspace{-0.5em}
    \caption{t-SNE visulalization for the AU embeddings generated by our framework w/ or w/o mask decoder module on BP4D dataset. \textcolor{red}{It is too small. How about make two figure in a column.}}
    \label{fig:tsne}
\end{figure}
%%%%%%%%%%%%%

\textbf{Mask Features Analyse.} 
Baseline-FEC-DF is a network of encoder-decoder structure, based on which further adding an mask decoder(DM) is our full framework, namely Baseline-FEC-DF-DM. The only difference between them is the absence and presence of mask decoder sub-module(DM). For the purpose of verifying the importance of mask learning, we further visualize the embedding of AU classifiers of the above two structures. We sampled some images and got their AU embeddings, showing the t-SNE visualization of them. As illustrated in Figure~\ref{fig:tsne}, each color refers to a class of AU presentations. Obviously the presentations learned with mask decoder is more compact and has a better distribution than that without mask decoder. Moreover, all the AU embedding learned with mask decoder tend to gather into two clusters(positive and negative).  While the presentations generated without mask decoder display like a long strip and doesn't divide into two clusters on AU2, AU4, AU15, AU17 and AU23, which means that it can not distinguish the positive and negative samples well on these AUs. This demostrates that the mask learning module is significant for capturing discriminative local features beneficial to AU recognition.

\textbf{Analysis of Different Mask Activation Function}
Each AU is responsible to a mask in our framework, and the mask indicates where of the spatial location is important for recognizing the target AU. We tried three different activation functions to get our mask, namely Softmax, Tanh and Sigmoid. As shown in Figure~\ref{fig:avtivation}, different activations on the outputs of Mask Decoder bring various mask attention maps. As expected, masks generated by Softmax activation function are the most sparse among these three activation functions. This attribute to the restriction on the sum of all AU masks that values must range from 0 to 1, reducing the overlap between each mask. In comparison, the other two activation approaches, Sigmoid and Tanh, get more dense map for each AU because there is no restriction between different masks. Besides, Sigmoid learns better mask map than Tanh for the reason that its estimation value domain exactly mach the attention. Sigmoid can also capture the relation between different AUs. For instance, AU1, AU2 and AU4 not only activate the location of brows, but also the area around mouth, because expressions with brow movement usually accompany with mouth movements in the training dataset. 











==> experiment_bk2.tex <==
\section{Experimental Results}

% \begin{table*}[!t]
% %\small
% \footnotesize
% \setlength{\tabcolsep}{2pt}
% \renewcommand\arraystretch{1.5} 
% \centering
% {
%   \caption{Ablation study on BP4D measured by F1 scores(\%).}
%   \vspace{-1em}
%   \label{tab:F1 on Ablation}
%  \begin{tabular}{l|cccccccccccc|c}
%     \hline
%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Classifier} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{Position-Encoding} &\textbf{F1-Score} \\[1pt]
%     \hline\hline
%     Baseline        &- &- &$\surd$  &- &- &- &52.6\\
%     Baseline-ImageNet         &$\surd$ &- &$\surd$ &- &- &- &61.6 \\
%     Baseline-FEC         &- &$\surd$ &$\surd$ &- &- &- &63.3 \\
%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &$\surd$ &- &- &63.8 \\
%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &$\surd$ &- &- &64.0 \\
%     Baseline-FEC-DF-DM       &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &- &66.3 \\
%     Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\
%     \hline
%   \end{tabular}}
% \end{table*}

%To validate our proposed method, the evaluation is conducted on three public datasets commonly-used for AU detection. These datasets contain face expression images with manually-annotated action unit labels. For fair comparisons, our evaluation follows the prior works, using three-fold cross validation. The reported results are the averages from three-fold experiments. This section introduces the detail experiment settings, evaluate the effectiveness on each module, and visualize the intermediate results generated by the framework at last.





In this section we report extensive experiments to validate the effectiveness of our method. These experiments are conducted on three public benchmarks commonly-used for AU detection, all of which contain face expression images with manually-annotated AU labels. 

We first introduce the used three datasets in detail and then describe the implementation details of the training and validation processes. Furthermore, we compare our method with the start-of-the-art methods to demonstrate the superiority of our approach. For fair comparisons, our evaluation follows the prior works \cite{li2018eac,shao2021jaa}, using three-fold cross-validation and also their specific division of training and validation data(see below). The reported results are the averages from three-fold experiments. To further obtain insight into our method, we designed ablation experiments to study the impact of the built sub-modules. Finally, we visualize several samples to further validate our method.

% -datasets
% - impletmenttation dedails
% - results, validate our method by comparing with baselines
% - further to get insight to our method, validate our careful-designe, ablation study...
% - visual reatuls

\subsection{Datasets}
As mentioned above, our evaluation was performed on three widely-used AU detection datasets: BP4D \cite{BP4D}, DISFA \cite{MavadatiDISFA}, and BP4D+ \cite{zhang2016multimodal}. All the above datasets were annotated with AU labels by certified experts for each frame.

%可以展开说下标注过程，比如观看视频，还是观察单帧，等等。如果标注过程没有区别，那么就集中写在前面，否则可以写在每个数据集文字内部。
%anrudong: 三个数据集均在视频序列上逐帧进行标注，标注方式写在了每个数据集各自的介绍部分
%yuding: 是的，我知道，需要在前面整体说一下三个数据集的共性和区别（概括说就好），说了之后，你再分数据集单独说，读者读起来就顺，知道下面三个数据集是在对上面共性和差异性的展开。如果不说，下面三个数据集就像三块砖头摆在那里，没有语言把它们拎起来。
\textbf{BP4D} consists of 328 video clips from 41 participants(23 females and 18 males). Each video frame was annotated with the occurrence or absence of 12 AUs(1, 2, 4, 6, 7, 10,
12, 14, 15, 17, 23, and 24. Their definition can be seen in Table \ref{tab:AUs definition}). In total, about 140,000 frames were annotated frame-by-frame by a group of FACS experts. Following the same subject division \cite{li2018eac,shao2021jaa}, we performed three-fold, subject-exclusive, cross-validations for all experiments.
%（哪12个，列出来，AU1, AU2,...AU12。可以提供一张图把三个数据集涉及到的所有AU的样例图都集中画出来，让读者看起来舒服，能快速明白AU对应是哪一个）.

%%%%%%%BP4D%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*} 
\footnotesize
%\small
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art methods on BP4D in terms of F1 scores(\%). The best results are shown in bold, and the second best results are in brackets.}
  \vspace{-1em}
%   \vspace{-1em}
  \label{tab:F1 on Bp4D}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline 
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4}&\textbf{AU6}&\textbf{AU7}&\textbf{AU10}&\textbf{AU12}&\textbf{AU14}&\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline 
    LSVM    &23.2 &22.8 &23.1 &27.2 &47.1 &77.2 &63.7 &64.3 &18.4 &33.0 &19.4 &20.7 &35.3 \\
    JPML    &32.6 &25.6 &37.4 &42.3 &50.5 &72.2 &74.1 & 65.7 &38.1 &40.0 &30.4 &42.3 &45.9\\
    DRML    &36.4 &41.8 &43.0 &55.0 &67.0 &66.3 &65.8 &54.1 &33.2 &48.0 &31.7 &30.0 &48.3\\
    EAC-Net &39.0 &35.2 &48.6 &76.1 &72.9 &81.9 &86.2 &58.8 &37.5 &59.1 &35.9 &35.8 &55.9\\
    % ROI     &36.2 &31.6 &43.4 &77.1 &73.7 &85.0 &87.0 &62.6 &45.7 &58.0 &38.3 &37.4 &56.4\\
    %JAA-Net &47.2 &44.0 &54.9 &7 7.5 &74.6 &84.0 &86.9 &61.9 &43.6 &60.3 &42.7 &41.9 &60.0\\
    DSIN    &51.7 &40.4 &56.0 &76.1 &73.5 &79.9 &85.4 &62.7 &37.3 &62.9 &38.8 &41.6 &58.9\\
    ARL     &45.8 &39.8 &55.1 &75.7 &77.2 &82.3 &86.6 &58.8 &47.6 &62.1 &47.4 &55.4 &61.1\\
    LP-Net  &43.4 &38.0 &54.2 &77.1 &76.7 &83.8 &87.2 &63.3 &45.3 &60.5 &48.1 &54.2 &61.0\\
    AU-GCN &46.8 &38.5 &60.1 &[80.1] &79.5 &84.8 &88.0 &67.3 &52.0 &63.2 &40.9 &52.8 &62.8 \\
    SRERL   &46.9 &45.3 &55.6 &77.1 &78.4 &83.5 &87.6 &63.9 &52.2 &63.9 &47.1 &53.3 &62.9\\
    AU-RCNN &50.2 &43.7 &57 &78.5 &78.5 &82.6 &87 &67.7 &49.1 &62.4 &50.4 &49.3 &63.0 \\
    UGN-B   &54.2 &46.4 &56.8 &76.2 &76.7 &82.4 &86.1 &64.7 &51.2 &63.1 &48.5 &53.6 &63.3\\
    J{\^A}A-Net &53.8 &47.8 &58.2 &78.5 &75.8 &82.7 &88.2 &63.7 &43.3 &61.8 &45.6 &49.9 &62.4\\
    SEV-Net &\textbf{58.2} &\textbf{50.4} &58.3 &\textbf{81.9} &73.9 &\textbf{87.8} &87.5 &61.6 &[52.6] &62.2 &44.6 &47.6 &63.9\\
    HMP-PS &53.1 &46.1 &56.0 &76.5 &76.9 &82.1 &86.4 &64.8 &51.5 &63.0 &[49.9] &54.5 &63.4\\
    MHSA-FFN &51.7 &[49.3] &[61.0] &77.8 &\textbf{79.5} &82.9 &86.3 & \textbf{67.6} &51.9 &63.0 &43.7 &[56.3] &64.2\\
    CISNet &54.8 &48.3 &57.2 &76.2 &76.5 &85.2 &87.2 &66.2 &50.9 &[65.0] &47.7 &\textbf{56.5} &64.3\\
    D-PAttNe$t^{tt}$ &50.7 &42.5 &59.0 &79.4 &79.0 &85.0 &[89.3] &67.6 &51.6 &\textbf{65.3} &49.6 &54.5 &64.7\\
    CaFNet &[55.1] &49.3 &57.7 &78.3 &78.6 &[85.1] &86.2 &[67.4] &52.0 &64.4 &48.3 &56.2 &[64.9]\\
    \hline
    \textbf{GLEE-Net(Ours)}  &\textbf{58.2} &48.7 &\textbf{61.5} &78.7 &[79.2] &84.2 &\textbf{89.8} &66.3 &\textbf{56.7} &64.8 &\textbf{53.5} &53.6 &\textbf{66.3}\\
    %Ours  &[57.8] &45.3 &\textbf{61.1} &[80.0] &[78.6] &[85.6] &[87.9] &\textbf{68.2} &[52.3] &[63.8] &[49.0] &\textbf{56.8} &\textbf{65.5}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

\textbf{DISFA} contains 27 video clips from 27 participants(12 females and 15 males). Each video records the facial activity of a participant when watching a 4-minutes video clip. Each clip consists of 4,845 frames evenly. Altogether, around 130,000 frames were annotated with intensities from 0 to 5. Following previous works \cite{jacob2021facial}\cite{li2018eac}\cite{shao2021jaa}\cite{yang2021exploiting}, we regard intensity labels $\{0,1\}$ as absence and others as presence. The evaluation was performed on 8 AUs(1, 2, 4, 6, 9, 12, 25, and 26. Their definition can be seen in Table \ref{tab:AUs definition}).  . We also performed the same three-fold, subject-exclusive, cross validations on 8 AUs as in the previous works \cite{li2018eac}\cite{shao2021jaa}.% following the subject division of \cite{li2018eac, shao2021jaa}.

\textbf{BP4D+} contains 1400 video clips from 140 participants(82 females and 58 males). Compared to BP4D, it has larger identity variations and video numbers. About 198,000 frames were annotated with the same 12 AUs in BP4D. We performed three-fold, subject-exclusive, cross-validations to compare our method with the state-of-the-art. Besides, to evaluate the generalization performance, our method was trained on BP4D and then evaluated on BP4D+, following the previous works \cite{attnetionTrans2019}\cite{shao2021jaa}.

To sum up, the order from largest to smallest of the three datasets is BP4D+, BP4D, and DISFA. BP4D and BP4D+ were recorded in similar shooting environments and lighting conditions. Both of them share the same 12 AU classes. In comparison, DISFA is the smallest dataset containing only 8 AU classes and was captured in quite different lighting conditions.

%以上是列举了三个数据，接下来可以做一个数据集的总结，比如说从数据量来说，xxx最少，xxx居中，最多是xxxx。也包括AU的个数也可以提一下，这里重在讲三个数据集的区别。这样方便后面实验讨论，比如我们工作可能在数据量大的数据集上表现好，等等，分析讨论结果的时候可以到这里来找理由，找依据。



% \begin{table}[!t]
% %\small
% \footnotesize
% %\setlength{\tabcolsep}{6.5pt} 
% \renewcommand\arraystretch{1.5} 
% \centering
% {
%   \caption{Ablation study of different global feature encoder pretrained on different dataset and task. Measured on BP4D by F1 scores(\%). InpResNetv1 is the abbreviation of InceptionResNetv1 }
%   \vspace{-1em}
%   \label{tab:F1 on pretrain}
%  \begin{tabular}{l|cccccccc|c}
%     \hline
%   %\textbf{Arch.} &\textbf{ResNet50} &\textbf{InceptionResNetv1} &\textbf{InceptionResNetv1}\\[1pt]
%     \textbf{Arch.} &ResNet50 &InpResNetv1 &InpResNetv1\\[1pt]
%     \hline\hline
%     \textbf{Data.} &ImageNet &ImageNet &FEC\\[1pt]
%     \textbf{Task.} &Classification &Classification &Expression similarity \\[1pt]
%     \hline
%     \textbf{F1-Score} &64.4 &63.5 & 66.3\\
%     \hline
%   \end{tabular}}
% \end{table}

%%%%%%%DISFA%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\footnotesize
\setlength{\tabcolsep}{0.9pt} 
\renewcommand\arraystretch{1.5} 
\centering
{ 
  \caption{Comparisons of our method and the state-of-the-art methods on DISFA in terms of F1 scores(\%). 
%   The best results are shown in bold, and the second best are in brackets.
  }
  \vspace{-1em}
  %\vspace{-1em}
  \label{tab:F1 on DISFA}
 % \setlength{\tabcolsep}{1.9mm}{
  \begin{tabular}{l|cccccccc|c}
   \hline 
 \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU9} &\textbf{AU12} &\textbf{AU25} &\textbf{AU26} &\textbf{Avg.}\\[1pt]
    \hline\hline
    LSVM       &10.8 &10.0 &21.8 &15.7 &11.5 &70.4 &12.0 &22.1 &21.8\\
    DRML       &17.3 &17.7 &37.4 &29.0 &10.7 &37.7 &38.5 &20.1 &26.7\\
    APL        &11.4 &12.0 &30.1 &12.4 &10.1 &65.9 &21.4 &26.9 &23.8\\
    EAC-Net        &41.5 &26.4 &66.4 &50.7 &8.5 &\textbf{89.3} &88.9 &15.6 &48.5\\
    %JAA-Net    &43.7 &46.2 &56.0 &41.4 &44.7 &69.6 &88.3 &58.4 &56.0\\
    DSIN       &42.4 &39.0 &68.4 &28.6 &46.8 &70.8 &90.4 &42.2 &53.6\\
    ARL        &43.9 &42.1 &63.6 &41.8 &40.0 &76.2 &[95.2] &66.8 &58.7\\
    LP-Net     &29.9 &24.7 &72.7 &46.8 &49.6 &72.9 &93.8 &56.0 &56.9\\
    AU-GCN      &32.3 &19.5 &55.7 &57.9 &61.4 &62.7 &90.9 &60.0 &55.0\\
    AU-RCNN  &32.1 &25.9 &59.8 &55.4 &39.8 &67.7 &77.4 &52.6 &51.3 \\
    SRERL      &45.7 &47.8 &56.9 &47.1 &45.6 &73.5 &84.3 &43.6 &55.9\\
    UGN-B      &43.3 &48.1 &63.4 &49.5 &48.2 &72.9 &90.8 &59.0 &60.0\\
    J{\^A}A-Net    &[62.4] &[60.7] &67.1 &41.1 &45.1 &73.5 &90.9 &[67.4] &63.5\\
    MHSA-FFN   &46.1 &48.6 &72.8 &\textbf{56.7} &50.0 &72.1 &90.8 &55.4 &61.5\\
    SEV-Net    &55.3 &53.1 &61.5 &[53.6] &38.2 &71.6 &\textbf{95.7} &41.5 &58.8\\
    HMP-PS     &38.0 &45.9 &65.2 &50.9 &50.8 &76.0 &93.3 &\textbf{67.6} &61.0\\
    CISNet     &48.8 &50.4 &[78.9] &51.9 &47.1 &[80.1] &[95.4] &65.0 &64.7\\
    CaFNet     &45.6 &55.7 &\textbf{80.2} &51.0 &\textbf{54.7} &79.0 &95.2 &65.3 &[65.8]\\
    \hline
    \textbf{GLEE-Net(Ours)}    &\textbf{63.5} &\textbf{62.5} &69.8 &48.6 &[53.9] &75.6 &94.7 &64.4 &\textbf{66.6}\\
    \hline
  \end{tabular}}%}
\end{table}

%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art methods on BP4D+ in terms of F1 scores(\%). 
%   The best results are shown in bold.
  }
 \vspace{-1em}
  \label{tab:F1 on ThreeFoldBp4DPlus}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline
    FACS3D-Net     &43.0 &38.1 &\textbf{49.9} &82.3 &85.1 &87.2 &87.5 &66.0 &48.4 &[47.4] &50.0 &[31.9] &59.7\\
    ML-GCN &40.2 &36.9 &32.5 &84.8 &[88.9] &89.6 &[89.3] &81.2 &[53.3] &43.1 &55.9 &28.3 &60.3\\
    MS-CAM &38.3 &37.6 &25.0 &85.0 &\textbf{90.9} &\textbf{90.9} &89.0 &[81.5] &\textbf{60.9} &40.6 &58.2 &28.0 &60.5\\
    SEV-Net &[47.9] &\textbf{40.8} &31.2 &\textbf{86.9} &87.5 &89.7 &88.9 &\textbf{82.6} &39.9 & \textbf{55.6} &[59.4] &27.1 &[61.5]\\
    \hline
    \textbf{GLEE-Net(Ours)}  &\textbf{51.5} &[46.6] &[43.5] &[86.8] &89.6 &[91.0] &\textbf{89.8} &82.3 &46.8 & 49.3 &\textbf{60.9} &\textbf{50.9} &\textbf{65.7}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art on cross-dataset evaluation(trained on BP4D and evaluated on BP4D+) in terms of F1 scores(\%). 
%   The best results are shown in bold.
  }
 \vspace{-1em}
  \label{tab:F1 on Bp4DPlus}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline
    EAC-Net     &38.0 &[37.5] &[32.6] &82.0 &83.4 &87.1 &85.1 &62.1 &44.5 &43.6 &45.0 &32.8 &56.1\\
    ARL         &29.9 &33.1 &27.1 &81.5 &83.0 &84.8 &86.2 &59.7 &[44.6] &43.7 &48.8 &32.3 &54.6\\
    J{\^A}A-Net &\textbf{39.7} &35.6 &30.7 &[82.4] &[84.7] &[88.8] &[87.0] &[62.2] &38.9 &[46.4] &[48.9] &\textbf{36.6} &56.8\\
    \hline
    \textbf{GLEE-Net(Ours)}  &[39.5] &\textbf{37.7} &\textbf{44.0} &\textbf{84.5} &\textbf{84.9} &\textbf{89.6} &\textbf{87.7} &\textbf{72.3} &\textbf{44.9} & [45.3] &\textbf{52.6} &[33.9] &\textbf{59.7}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

\subsection{Implementation Details}

Face images were first aligned and cropped according to landmark detection results. Before feeding to our networks, the input images were resized to $256\times256$. The resolution of feature maps was reduced to $16\times16$ after passing through the Feature Encoder.

To enhance the feature extraction capability of low-level convolution layers, the feature encoder was initialized with the corresponding network parameters pretrained on the dataset of ImageNet or FEC, and the rest of our networks were set to Kaiming initialization \cite{he2015delving}. Except for the Mask Decoder, the whole model parameters were updated by employing an Adam optimizer with hyper-parameters $\beta = 0.9$ and weight decay $10^{-6}$.
%可能要斟酌一下要不要写MaskDecoder部分参数冻结，要写的话如何说清和证明它的作用

The networks were trained for 20 epochs with an initial learning rate of $10^{-5}$ on each dataset fold. The mini-batch size was set to 10. We used a warm-up stage with $10^3$ steps and then decayed the learning rate exponentially with an exponent $-0.5$. The training and inference pipelines were implemented in Pytorch on 4 GeForce GTX 2080ti GPU. 
%这里就可以给一张训练集和验证集，随着时间，收敛的情况，可以分AU来说，我们也可以观察下，哪些AU收敛快，哪些慢，哪些容易过拟合，哪些比较好泛化，等等，这个图都是可以用来分析后面的实验结果，避免实验结果太干涩，没话说。


\subsection{Comparisons with the State-of-the-Art}
We compared our method with many state-of-the-art AU detection methods, including LSVM \cite{LSVM}, JPML \cite{JPML}, DRML \cite{DRML}, APL \cite{LP48}, EAC-Net \cite{li2018eac}, DSIN \cite{LP8}, ARL \cite{attnetionTrans2019}, SRERL \cite{SRERL}, AU-GCN\cite{liu2020relation},AU-RCNN\cite{ma2019r}, ML-GCN \cite{chen2019multi}, MS-CAM \cite{you2020cross}, LP-Net \cite{LP}, FACS3D-Net \cite{yang2019facs3d}, UGN-B \cite{song2021uncertain}, J{\^A}A-Net \cite{shao2021jaa}, MHSA-FFN \cite{jacob2021facial}, SEV-Net \cite{yang2021exploiting}, HMP-PS \cite{song2021hybrid}, D-PAttNe$t^{tt}$\cite{Onal2019D-PAttNet}, CISNet\cite{chen2022causal} and CaFNet\cite{chen2021cafgraph}. 


Specifically, while EAC-Net, ARL, J{\^A}A-Net, and SEV-Net were evaluated on all three datasets, LSVM, JPML, DRML, APL, DSIN, SRERL, AU-GCN, AU-RCNN, LP-Net, UGN-B, MHSA-FFN, HMP-PS, CISNet and CaFNet were evaluated on both BP4D and DISFA. Particularly, D-PAttNe$t^{tt}$ was only evaluated on BP4D. FACS3D-Net, ML-GCN and MS-CAM were evaluated merely on BP4D+. Since BP4D+ is released later, it is not used by all the methods.
%\textcolor{red}{[Reviewers may question why not evaluate all the methods on all the three datasets? Any particular reasons doing so? If so, it would be better to explain the reasons here.]} %这里就可以说下，哪些方法是在三个数据集上测试，哪些仅仅是两个数据，这些都是为后面分数据集汇报结果准备，避免人家说，为什么不同数据集，baseline方法却不一样。

Following the experimental settings of most previous works, we also employed the F1 score \cite{F1} on the frame level as the evaluation metric. F1-score is a harmonic mean of precision(P) and recall(R), which is defined as $F1 = 2PR/(P+R)$. Since F1-score takes both false positives and false negatives into account, it reflects a more rational measurement of the model's performance than accuracy, especially on datasets with uneven class distributions like BP4D, DISFA, and BP4D+.



\textbf{Evaluation on BP4D.}
The results on BP4D are shown in Table \ref{tab:F1 on Bp4D}. The average F1 score of our method is 66.3\%, which significantly outperforms all the other comparison methods, improving about 1.4\% over the second highest one, CaFNet. In terms of the performances on single AUs, our method achieves the highest F1 scores among all the methods on 5 AUs(i.e., AU1, AU4, AU12, AU15, and AU23) and second highest on 1 AUs(AU7) of the 12 evaluated AUs. Besides, our method shows over 3.5\% superiority on AU15 and AU23 over the second highest ones. 


In terms of AU feature learning, our method outperforms JMPL, DRML, and D-PAttNe$t^{tt}$ about 20.4\%, 18\% and 1.6\%, demonstrating that extracting local features by attention is more effective and our method is superior in AU feature extraction than patch learning. 

Compared with EAC-Net, JAA-Net, and MHSA-FFN, which utilize attention mechanisms with the supervisions of pre-defined AU centers, our method achieves improvements of 10.4\%, 5.2\% and 3.9\% over them(EAC-Net, JAA-Net, and MHSA-FFN), respectively. This validates the superiority of our non-predetermined AU attention learning approach.  %\textcolor{red}{I think we can improve the structure of the above text.}


%\textcolor{red}{Compared to SEV-Net and J{\^A}A-Net that employ textual embedding and facial landmarks as auxiliary training information, our method obtains better results with the compact expression embedding as prior knowledge. WHAT DO WE WANT TO EXPRESS}


\textbf{Evaluation on DISFA.}
Table \ref{tab:F1 on DISFA} shows the evaluation results on DISFA. As shown in this table, our method achieves the average F1 score of 66.6\%, outperforming all the compared state-of-the-art methods. 

Compared to the most recent works SEV-Net, HMP-PS, MHSA-FFN, CISNet and CaFNet, our method achieves an improvement of 7.8\%, 5.6\%, 5.1\%, 1.9\% and 0.8\% over them, respectively. Unlike EAC-Net and J{\^A}A-Net which are supervised by both AU and landmark labels, our method only utilizes AU labels, but still obtains significant improvements of 18.1\% and 3.1\% over EAC-Net and J{\^A}A-Net, respectively, demonstrating the effectiveness of our method in AU feature and attention learning. Note that our method does not explicitly model AU relationships, but significantly exceeds all relation-based methods including JMPL, DSIN, ARL, AU-GCN, and AU-RCNN.

%As the number of subjects in DISFA is smaller than that of BP4D, \textcolor{red}{most of the previous methods suffer from overfitting to the appearance of training subjects more severely. WHY?} Therefore, benefiting from our identity-independent expression representations, our method achieves an even more significant improvement.

\textbf{Evaluation on BP4D+.}
Table \ref{tab:F1 on ThreeFoldBp4DPlus} shows the evaluation results of the three-fold cross-validation on BP4D+.
In particular, the results of SEV-Net, ML-DCN and MS-CAM are reported in\cite{yang2021exploiting} while the results of EAC-Net are reported in \cite{shao2021jaa}. 
Our method achieves the F1 score of 65.7\% and outperforms all the state-of-the-art methods, exceeding SEV-Net over 4.2\%.

%%%%%%%%%%%%%
% %%%%%%%%%%%%%pose_mask figure
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[ width=18cm]{images/sample4.pdf}
%     %\vspace{-0.5em}
%     \caption{Illustration of attention map on different head pose. The Mask Decoder generates  similar masks with various pose images input, demonstrates that the mask decoder is robust to head pose}
%     \label{fig:pose_mask}
% \end{figure*}
% %%%%%%%%%%%%%

To further evaluate the generalization performance of our method on large-scale test identities, we trained our method on BP4D and evaluated it on the full BP4D+ of 140 subjects. The results are shown in Table \ref{tab:F1 on Bp4DPlus}. We use the reported results in the work \cite{shao2021jaa} for comparison. Again, our method outperforms all the compared methods under the large-scale cross-dataset evaluation. It indicates that our method can extract identity-independent information and generalize well to new identities.

%\textcolor{red}{[if possible, I suggest to move the tables/figures to the same page as the first cited place/page. Or if it cannot be achieved, the place of tables/figures should be as close as possible to the first cited place/page. This would increase the readability.]}

%From the evaluation results on the three datasets, we can see that AU7, AU12 and AU17 rechieve best performances on BP4D, and AU1 and AU2 gets best results on DISFA. 
%综合看三个数据集的结果，可以谈谈哪些AU，我们的方法总是获胜，哪些总是不好，然后可以分析原因。

\subsection{Ablation Study}
%先简要回顾下我们的算法框架，其实有挑选的介绍，然后再说我们要逐一验证这些框架子模块的设计，才进行了ablation study。（提高文章的过度和可读性）

%As described in Section \ref{sec:methodology}, our framework includes the global feature encoder followed by two branches of feature decoders, namely, facial feature decoder($D_f$) and facial mask decoder($D_m$). While the $D_f$ module creates one initial feature map for each AU, the $D_m$ module is responsible for learning feature masks that filter out the areas irrelevant to current AU. Then, by a point-wise multiplication of the initial feature map $xx$ and the feature mask from $D_f$ and $D_m$, we obtain the feature map  $xx$ of AU-related local regions for each AU. $we have to clearly indicate what we will validate by our ablation studies.$
In this section, we conduct ablation studies to evaluate the effectiveness of each key sub-module in our framework, including: 1) the prior knowledge of expression similarity learning, 2) the facial components module, 3) and mask activation.In particular, all the ablation experiments are conducted on the BP4D dataset due to space limitations.

%As shown in Table~\ref{tab:F1 on Ablation}, we firstly construct a baseline model(Baseline), of which the feature extractor is based on InceptionResNetv1 without pretrained parameters, followed by AU classifiers. Besides, to verify the validity of the pretrained expression featrue encoder, we load parameters pretrained on ImageNet(Baseline-ImageNet) and on FEC(Baseline-FEC) respectively. For further validation of our facial feature decoder($D_f$) and facial mask decoder($D_m$), we gradually add $D_f$(Baseline-FEC-DF ) and $D_m$(Baseline-FEC-DF-DM) .  

%Furthermore, as shown in Table \ref{tab:F1 on Ablation 2}, to explore the effectiveness of each implementation, we replace or remove certain individual modules of the full framework and test the model performance. For instance, freezing the pretrained Feature Encoder weights(w.fixed FE), replacing the activation function of mask decoder with softmax(w. Softmax), etc. The experiments results will be analysed in detail in the following paragraphs.   %既然这里提到了表格4，这里就定义出表格4中各种消融方法的定义
%anrudong: 表格中涉及到的各个消融实验方法的定义下文有分模块详细介绍，如果在这里再写一遍显得有些重复,因此删掉

\begin{table*}[!t]
%\small
\footnotesize
\setlength{\tabcolsep}{8pt}
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Ablation study on BP4D measured by F1 scores(\%).}
  \vspace{-1em}
  \label{tab:F1 on Ablation}
 \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{F1-Score} \\[1pt]
    \hline\hline
    % Baseline        &- &-  &- &- &52.6\\
    % Baseline-ImageNet         &$\surd$ &- &- &- &61.6 \\
    Baseline-FEC         &- &$\surd$ &- &- &63.3 \\
    Baseline-FEC-DF          &- &$\surd$ &$\surd$ &- &63.8 \\
    Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &- &63.7 \\
    Baseline-FEC-DF-DM/GLEE-Net(Full)       &- &$\surd$ &$\surd$ &$\surd$ &66.3 \\
    % Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\
    \hline
  \end{tabular}}
\end{table*}

\begin{table*}[!t]
%\small
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Ablation study on BP4D measured by F1 scores(\%). }
  \vspace{-1em}
  \label{tab:F1 on Ablation 2}
 \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline\hline
    w/o pretrain &34.9 &24.2 &36.7 &76.1 &71.4 &81.0 &86.3 &58.7 &25.9 &51.9 &27.4 &31.6 &50.5\\
    w. FE Emotion &48.1 &41.6 &53.9 &78.6 &77.9 &83.2 &88.8 &60.5 &39.3 &65.5 &38.0 &47.6 &60.3 \\
    w. FE ImageNet &49.6 &39.7 &60.5 &77.3 &78.7 &83.1 &88.6 &[64.6] &48.2 &63.2 &47.5 &48.0 &62.4 \\
    w. FE fixed &52.3 &45.8 &59.8 &[79.4] &78.1 &\textbf{84.8} &89.0 &64.0 &46.5 &64.0 &38.6 &49.8 &63.5\\
    % w. ResNet &[56.9] &46.5 &57.2 &78.1 &[79.2] &84.2 &87.9 &63.8 &51.0 &64.7 &49.5 &[53.5] &[64.4]\\
    \hline
    w/o DM  &53.3 &44.2 &58.7 &78.6 &76.9 &83.9 &[89.8] &62.2 &48.9 &65.1 &[52.5] &51.8 &63.8\\
    w/o DM\&DF &55.4 &\textbf{65.1} &\textbf{73.9} &49.0 &46.9 &77.1 &\textbf{92.9} &54.1 &48.1 &64.7 &[52.5] &47.5 &63.3\\
   % w. PE & 54.8 &45.3 &[63.4] &78.4 &79.1 &[84.6] &89.1 &60.7 &49.7 &64.2 &50.7 &50.3 & 64.2\\
    
    \hline
    w. None & 53.7 &44.6 &55.4 &78.6 &78.4 &83.7 &89.2 &[64.6] &[51.4] &\textbf{65.9} &51.2 &52.6 &64.1\\
    w. SoftMax & 53.6 &43.8 &58.5 &\textbf{79.7} &[79.2] &84.5 &89.6 &63.4 &50.3 &62.7 &50.8 &53.0 &64.0\\
    w. Tanh &55.1 &46.2 &60.2 &79.1 &\textbf{79.3} &[84.6] &88.d6 &63.0 &49.6 &[65.3] &51.8 &50.2 &[64.4]\\ 
  
    \hline
    \textbf{GLEE-Net(Full)} &\textbf{58.2} &[48.7] &[61.5] &78.7 &[79.2] &84.2 &[89.8] &\textbf{66.3} &\textbf{56.7} &64.8 &\textbf{53.5} &\textbf{53.6} &\textbf{66.3}\\
    %GLEE-Net(Full) & 53.7 &[48.4] & 59.8 & \textbf{79.7} & 78.9 &83.5 & 89.5 &\textbf{64.0} &[50.6] &64.1 &50.2 &[53.4] &\textbf{64.7}\\
    \hline
  \end{tabular}}
\end{table*}

%\textcolor{red}{here we need a head text to briefly introduce what we will presents.}
\textbf{Prior Knowledge.} 
% \textcolor{red}{here we have to make a head paragraph to introduce what we will presents. What will we study? It looks three ablation studiese here.}
Our framework proposes a vision feature encoder $E_f$ that is pretrained on the FEC dataset via expression similarity learning, which refers to our prior knowledge. As shown in table~\ref{tab:F1 on Ablation 2}, to test the efficiency of prior knowledge, we design ablation experiments with different approaches to initialize $E_f$ in the training of $GLEE-Net$, including:
\begin{itemize}
    \item [(1) ]
    $E_f$ is randomly initialized(w/o pretrain);
    \item [(2) ]
    $E_f$ is initialized via a pretrained classifier of seven discrete facial expression emotion categories trained on the AffectNet dataset(w. FE Emotio);
    \item [(3) ]
     $E_f$ is initialized via a pretrained image object classifier built on imageNet(GLEE-Net(Full));  
    \item [(4) ]
     $E_f$ is our proposed method, initialized via the facial expression similarity(w/o pretrain); 
    \item [(5) ]
     $E_f$ is parameterized by the facial expression similarity approach but it not updated in the training of $GLEE-Net$ (w. FE fixed).
\end{itemize}

1-{2-4}: prior k is necessary;
4-2/3: ours is ok;
4-5: finetuning


To test the efficiency of prior knowledge, involving pretraining on various datasets (FEC, AffectNet, etc) and tasks(expression similarity learning, emotion recognition, etc) , we set ablation experiments from three aspects. 

Firstly, we design a baseline model, which is constructed with the feature encoder(without pretrained parameters) followed by the AU classifier module.
Particularly, the followed AU classifier has a similar structure to the AU classifier of the full network but with a different size due to the input feature size difference. As shown in table~\ref{tab:F1 on Ablation}, we test the baseline without pretrained parameters(Baseline), with parameters pretrained on ImageNet(Baseline-ImageNet) and with parameters pretrained on FEC(Baseline-FEC). The Baseline-FEC and the Baseline-ImageNet achieve  63.3\%  and 61.6\%, respectively.  Compared with the baseline model(52.6\%), they bring over 10.7 and 9\% improvements, which validates the importance of pretraining. Moreover, the Baseline-FEC achieves an improvement of 1.7\% compared with the Baseline-ImageNet, proving the superiority of our pretraining on FEC with expression similarity task.

Secondly, based on our full framework(GLEE-Net), we load the feature encoder with various pretrained weights. As shown in table~\ref{tab:F1 on Ablation 2}, we first test the full network without any pretrained weights(w/o pretrain), then load the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), AffectNet(w. FE Emotion) and FEC(GLEE-Net) respectively.  Specifically, the whole networks of the above experiments(except for w/o pretrain) are finetuned on BP4D. The results in table~\ref{tab:F1 on Ablation 2} show that when loading the parameters pretrained with the expression similarity task(GLEE-Net), it achieves the best F1-Score(66.3\%), while loading parameters pretrained on AffectNet(w. FE Emotion) and ImageNet(w. FE ImageNet) it declines 3.9\% and 6\%. This further verifies the effectiveness of the prior knowledge of expression similarity learning. 

Thirdly, we also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in Table \ref{tab:F1 on Ablation 2}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. It shows that the finetuning operation is effective to improve the performance of our framework.  

%gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.

%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.

%We first evaluate the effectiveness of pretraining. As illustrated in Table~\ref{tab:F1 on Ablation}, the baseline has the same structure as the feature encoder($E_f$) of our full network but does not load any pretrained parameters(\textit{Baseline}), which is followed by a classifier module \textcolor{red}{what does a classifier module refer to?}. Then we test it with pretrained parameters on ImageNet, namely, \textit{Baseline-ImageNet}. As shown in Table \ref{tab:F1 on Ablation}, the Baseline-ImageNet achieves 61.6\% and brings over 9\% improvement than the baseline(52.6\%), which validates the importance of pretraining.

%the baseline is constructed based merely on an InceptionResNetV1 network without pretraining. It has the same structure as the feature encoder of our full network, using the intermediate features which has a resolutioin of 16 x 16. The feature encoder of the baseline is followed by several classifer modules similar to AU Classifer Module. The number of classifier modules is corresponding to the AU classes. Each classifier module predicts a specific AU's probability and shares the same structure that contains 3 CNN layers and a Sigmoid activation at the last layer. Then we test the baseline with pretrained parametes on ImageNet, namely Baseline-ImageNet. As shown in Table \ref{tab:F1 on Ablation}, it achieves 61.6\% and brings over 9\% improvement compared with baseline(52.6\%), proving the importance of pretraining.
% 我感觉直接介绍pretrained feature model 部分即可，无需再介绍后面的classifier啥的结构了。

%To test the efficiency of our feature encoder pretrained on FEC with the facial expression similarity task, we replaced the feature encoder of our full network with different architectures or parameters and then fine-tuned the whole network on BP4D. 

%As shown in Table \ref{tab:F1 on Ablation 2}, we first load the weights of the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), then load the weights with parameters pretrained on an emotion dataset(AffectNet) by the emotion recognition task(w. FE Emotion). We also take ResNet50 pretrained on ImageNet as the feature encoder of our full network(w. ResNet50). 

%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.
%\textcolor{red}{looks no table for the above results. I dont know why the above uses DISFA and teh below uses the other two datsets.}

%To futher indicate the significance of the pretrained facial expression embedding network, we also test it on the BP4D dataset. First, we replace the feature encoder with a ResNet~\cite{Resnet34}~(w. ResNet50 in Table~\ref{tab:F1 on Ablation 2}). The results show that using pretrained facial expression embedding network as backbone improves the score by 3\% on BP4D. 


%We also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in the Table \ref{tab:F1 on Ablation}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. This shows that the fine-tuned operation is effective to improve the performance of our framework. 
%\textcolor{red}{Any more discussion here?.}



\textbf{Facial Components.}
As shown in Table~\ref{tab:F1 on Ablation}, to validate the effectiveness of the representations extracted by the Facial Components module(FCM), we conducted some ablation experiments on BP4D. Specifically, based on the feature encoder pretrained on FEC(Baseline-FEC in Table~\ref{tab:F1 on Ablation} or w/o DM\&DF in Table~\ref{tab:F1 on Ablation 2}), we gradually added the $D_f$ branch(Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation} or w/o DM in Table~\ref{tab:F1 on Ablation 2}) and the $D_m$ branch(Baseline-FEC-DF-DM in Table~\ref{tab:F1 on Ablation} or GLEE-Net in Table~\ref{tab:F1 on Ablation 2}). In addition, we replaced the facial feature decoder of Baseline-FEC-DF with a CNN structure module(Baseline-FEC-CNN) to further validate the effectiveness of the facial feature decoder. %\textcolor{red}{Why BP4D only? why not the other two datasets.}
%Firstly, based on the feature encoder pretrained on FEC(Baseline-FEC), when adding the $D_f$ branch(Baseline-FEC-DF), the F1-score improves 0.5\%(from 63.3\% to 63.8\%). Further introducing the  $D_f$ and the $D_m$(Baseline-FEC-DF-DM), the results improves 2.5\%. 
%we construct the model only with the Feature Encoder ~(w/o MD \& FD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC in Table~\ref{tab:F1 on Ablation}) or the Facial Decoder branch~(w/o MD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation}) individually. %a decline of 2.5\%(from 66.3\% to 63.8\%) is caused when the Mask Decoder is removed(Baseline-FEC-DF) and 3\% decline(from 66.3\% to 63.3\%) when the Facial Decoder is also removed(Baseline-FEC) respectively. 

%%%%%%%%%%%%%pipeline figure
\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/sample1.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the decoded mask attention maps:(Left) samples from DISFA, and(Right) samples from BP4D and BP4D+. The learned masks(odd rows) are also visualized and overlaid on the corresponding face images(even rows). The colors covering on the face images from blue to red indicate the attention values from low to high.}
    \label{fig:figure1}
\end{figure}
%%%%%%%%%%%%%

%%%%%%%%%%%%%mask figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample2.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the mask attention maps overlaid onto the corresponding input images in BP4D. The first column shows face images with different expressions. We can observe that similar AU-related local mask distributions can be learned by our framework even though the identities and expressions vary significantly.  }
    \label{fig:mask visualization}
\end{figure*}
%%%%%%%%%%%%%avtivation figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample3.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the mask maps generated by different activation functions(Sigmoid, softmax, and Tanh, from top to bottom) on each AU from the BP4D dataset. The masks of softmax are more sparse than those of Sigmoid and Tanh because it has an extra restriction between AU channels. Therefore, softmax may filter out some related regions.}
    \label{fig:avtivation}
\end{figure*}
%%%%%%%%%%%%%
Note that the inclusion of the facial feature decoder alone brings an improvement of 0.5\%(from 63.3\% to 63.8\%) over the Baseline-FEC. When the facial feature decoder is replaced by the CNN module, the performance declines by 0.1\%(from 63.8\% to 63.7\%) on F1-Score. Moreover, the performance improves by 2.3\% when we further added the facial mask decoder module and constructed our full network, GLEE-Net. These study results validate the effectiveness of our attention and local feature learning.
% In the experiment without pretraining on the expression dataset~(w/o pretrain), we can see an apparent drop in average F1-score of .

%\textcolor{red}{[It seems the two rows(w/o DM, and w/o DM\&DF) in Table 7 are not used/cited in the main texts. So, reviewers may question why you put the two rows in Table 7?]}\textcolor{blue}{[has been referred]}

\textbf{Mask Activations. }
To study the effect of activation functions on attention mask generation, we tried various activation methods on the outputs of the Mask Decoder. The results on the BP4D dataset are shown in Table \ref{tab:F1 on Ablation 2}. When there is no activation on the mask decoder's outputs(w. None), it achieves an F1 score of 64.1\%. As expected, the Sigmoid function(GLEE-Net(Full)) obtains the best result of F1-score 66.3\%. While Softmax(w. SoftMax) achieves an F1-score of 64.0\% and Tanh(w. Tanh) achieves 64.4\%. The possible reason is that the masks generated by Softmax tend to get sparse attention maps and exclude other parts including regions related to the target AU in most cases. This may result in the downstream recognition task being unable to learn sufficient information. While Sigmoid and Tanh can avoid the above shortcoming and retain the regions that are closely related to the target AU, making the subsequent Classifier Module have a better performance. 


%%%%%%%%%%%%%tsne figure
\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/tsne.pdf}
    %\vspace{-0.5em}
    \caption{t-SNE visualization of the AU embeddings generated by our framework w/ or w/o the mask decoder module on the BP4D dataset. }
    \label{fig:tsne}
\end{figure}
%%%%%%%%%%%%%

\subsection{Visual Analysis}
We also visualize the feature and mask results of our framework to further validate its effectiveness.

\textbf{Mask Attention Learning.} Due to its anatomical definition, each AU involves a group of muscle motions and is relative to a specific region in the face. For instance, AU1 is inner brow raising and AU9 is nose wrinkle. Theoretically our framework should learn a regional mask activation map for each AU, corresponding to its muscle actions. To validate the effectiveness of our mask feature learning, in Figure~\ref{fig:figure1} we visualize the attention mask maps of several 
examples from DISFA, BP4D and BP4D+, learned by our network. As shown in this figure, we can see that our method successfully captures a discriminative attention mask for each AU. Taking AU4(brow low) and AU7(lid tight) as examples, the learned spatial masks are around the brows and 
lower eyelids, respectively, which demonstrates that our proposed mask decoder is effective for AU-related local regional attention learning.

From Figure~\ref{fig:mask visualization}, we can see that each AU's mask is closely related to its muscle region, even for different expressions such as happy, sad, and fear.
We also notice that several different AUs may cover the same or similar area. This is attributed to that different AUs may share the same or similar muscle distributions. For instance, all of AU1, AU2, and AU4 are involved with the forehead, while all of AU14, AU15, AU17, AU23, and AU24 are closely related to the mouth area. Besides, considering the existence of potential mutual relations among different AUs, the masks learned merely supervised by AU labels may include other facial regions of correlated AUs. For instance, the masks of AU1, AU2, and AU4 not only cover the regions of the brows but also contain the mouth area.

\textbf{Mask Features Analysis.} Baseline-FEC-DF is a network of the encoder-decoder structure. On top of it, we can further add a mask decoder(DM) to obtain our full framework, namely, Baseline-FEC-DF-DM. The only difference between them is the absence/presence of the mask decoder sub-module. To validate the importance of mask learning, we visualize the embeddings of the AU classifiers of the above two structures. We sampled some images and obtained the t-SNE visualization of their AU embeddings. As illustrated in Figure~\ref{fig:tsne}, each color refers to a class of AU presentations. Obviously, the presentations learned with the mask decoder are more compact and have better distribution than that without the mask decoder. Moreover, all the AU embeddings learned with the mask decoder tend to gather into two clusters(positive and negative). By contrast, the presentations generated without the mask decoder display like a long strip and are not divided into two clusters for the cases of AU2, AU4, AU15, AU17, and AU23. As a result, these AUs cannot be well distinguished between positive and negative samples. This validates that the mask learning module in our framework is effective to capture discriminative local features that are beneficial to AU recognition.

\textbf{Analysis of Different Mask Activation Functions}.
Each mask  is responsible for an AU in our framework, and the mask indicates the spatial locations that are important for the recognition of the target AU. We compared three different activation functions to obtain our masks, namely, Softmax, Tanh and Sigmoid. As shown in Figure~\ref{fig:avtivation}, different activations on the outputs of the Mask Decoder bring various mask attention maps. As expected, the masks generated by the Softmax activation function are the most sparse among the three activation functions. This attribute to the restriction on the sum of all AU masks: their values must be in the range from 0 to 1, and thus reducing the overlap between masks. In comparison, the other two activation functions, Sigmoid and Tanh, can obtain a more dense map for each AU because there is no restriction between different masks. Besides, Sigmoid learns better mask maps than Tanh for the reason that its estimation value domain exactly matches the attention. Sigmoid can also capture the relation between different AUs. For instance, AU1, AU2, and AU4 activate not only the location of brows but also the mouth area, because expressions with brow movements usually accompany mouth movements in the training dataset. 


%\textcolor{red}{[Figure 8 is not cited anywhere in the main texts. If not cited/used in the main texts, reviewers may question why Figure 8 should be included into the paper.]}\textcolor{blue}{[has been deleted]}









['DJTest','female_damimao','yinxiaonv_demo1','yinxiaonv_demo2']

==> experiment_bk3.tex <==
\section{Experimental Results}

% \begin{table*}[!t]
% %\small
% \footnotesize
% \setlength{\tabcolsep}{2pt}
% \renewcommand\arraystretch{1.5} 
% \centering
% {
%   \caption{Ablation study on BP4D measured by F1 scores(\%).}
%   \vspace{-1em}
%   \label{tab:F1 on Ablation}
%  \begin{tabular}{l|cccccccccccc|c}
%     \hline
%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Classifier} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{Position-Encoding} &\textbf{F1-Score} \\[1pt]
%     \hline\hline
%     Baseline        &- &- &$\surd$  &- &- &- &52.6\\
%     Baseline-ImageNet         &$\surd$ &- &$\surd$ &- &- &- &61.6 \\
%     Baseline-FEC         &- &$\surd$ &$\surd$ &- &- &- &63.3 \\
%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &$\surd$ &- &- &63.8 \\
%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &$\surd$ &- &- &64.0 \\
%     Baseline-FEC-DF-DM       &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &- &66.3 \\
%     Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\
%     \hline
%   \end{tabular}}
% \end{table*}

%To validate our proposed method, the evaluation is conducted on three public datasets commonly-used for AU detection. These datasets contain face expression images with manually-annotated action unit labels. For fair comparisons, our evaluation follows the prior works, using three-fold cross validation. The reported results are the averages from three-fold experiments. This section introduces the detail experiment settings, evaluate the effectiveness on each module, and visualize the intermediate results generated by the framework at last.





In this section we report extensive experiments to validate the effectiveness of our method. These experiments are conducted on three public benchmarks commonly-used for AU detection, all of which contain face expression images with manually-annotated AU labels. 

We first introduce the used three datasets in detail and then describe the implementation details of the training and validation processes. Furthermore, we compare our method with the start-of-the-art methods to demonstrate the superiority of our approach. For fair comparisons, our evaluation follows the prior works \cite{li2018eac,shao2021jaa}, using three-fold cross-validation and also their specific division of training and validation data(see below). The reported results are the averages from three-fold experiments. To further obtain insight into our method, we designed ablation experiments to study the impact of the built sub-modules. Finally, we visualize several samples to further validate our method.

% -datasets
% - impletmenttation dedails
% - results, validate our method by comparing with baselines
% - further to get insight to our method, validate our careful-designe, ablation study...
% - visual reatuls

\subsection{Datasets}
As mentioned above, our evaluation was performed on three widely-used AU detection datasets: BP4D \cite{BP4D}, DISFA \cite{MavadatiDISFA}, and BP4D+ \cite{zhang2016multimodal}. All the above datasets were annotated with AU labels by certified experts for each frame.

%可以展开说下标注过程，比如观看视频，还是观察单帧，等等。如果标注过程没有区别，那么就集中写在前面，否则可以写在每个数据集文字内部。
%anrudong: 三个数据集均在视频序列上逐帧进行标注，标注方式写在了每个数据集各自的介绍部分
%yuding: 是的，我知道，需要在前面整体说一下三个数据集的共性和区别（概括说就好），说了之后，你再分数据集单独说，读者读起来就顺，知道下面三个数据集是在对上面共性和差异性的展开。如果不说，下面三个数据集就像三块砖头摆在那里，没有语言把它们拎起来。
\textbf{BP4D} consists of 328 video clips from 41 participants(23 females and 18 males). Each video frame was annotated with the occurrence or absence of 12 AUs(1, 2, 4, 6, 7, 10,
12, 14, 15, 17, 23, and 24. Their definition can be seen in Table \ref{tab:AUs definition}). In total, about 140,000 frames were annotated frame-by-frame by a group of FACS experts. Following the same subject division \cite{li2018eac,shao2021jaa}, we performed three-fold, subject-exclusive, cross-validations for all experiments.
%（哪12个，列出来，AU1, AU2,...AU12。可以提供一张图把三个数据集涉及到的所有AU的样例图都集中画出来，让读者看起来舒服，能快速明白AU对应是哪一个）.

%%%%%%%BP4D%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*} 
\footnotesize
%\small
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art methods on BP4D in terms of F1 scores(\%). The best results are shown in bold, and the second best results are in brackets.}
  \vspace{-1em}
%   \vspace{-1em}
  \label{tab:F1 on Bp4D}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline 
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4}&\textbf{AU6}&\textbf{AU7}&\textbf{AU10}&\textbf{AU12}&\textbf{AU14}&\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline 
    LSVM    &23.2 &22.8 &23.1 &27.2 &47.1 &77.2 &63.7 &64.3 &18.4 &33.0 &19.4 &20.7 &35.3 \\
    JPML    &32.6 &25.6 &37.4 &42.3 &50.5 &72.2 &74.1 & 65.7 &38.1 &40.0 &30.4 &42.3 &45.9\\
    DRML    &36.4 &41.8 &43.0 &55.0 &67.0 &66.3 &65.8 &54.1 &33.2 &48.0 &31.7 &30.0 &48.3\\
    EAC-Net &39.0 &35.2 &48.6 &76.1 &72.9 &81.9 &86.2 &58.8 &37.5 &59.1 &35.9 &35.8 &55.9\\
    % ROI     &36.2 &31.6 &43.4 &77.1 &73.7 &85.0 &87.0 &62.6 &45.7 &58.0 &38.3 &37.4 &56.4\\
    %JAA-Net &47.2 &44.0 &54.9 &7 7.5 &74.6 &84.0 &86.9 &61.9 &43.6 &60.3 &42.7 &41.9 &60.0\\
    DSIN    &51.7 &40.4 &56.0 &76.1 &73.5 &79.9 &85.4 &62.7 &37.3 &62.9 &38.8 &41.6 &58.9\\
    ARL     &45.8 &39.8 &55.1 &75.7 &77.2 &82.3 &86.6 &58.8 &47.6 &62.1 &47.4 &55.4 &61.1\\
    LP-Net  &43.4 &38.0 &54.2 &77.1 &76.7 &83.8 &87.2 &63.3 &45.3 &60.5 &48.1 &54.2 &61.0\\
    AU-GCN &46.8 &38.5 &60.1 &[80.1] &79.5 &84.8 &88.0 &67.3 &52.0 &63.2 &40.9 &52.8 &62.8 \\
    SRERL   &46.9 &45.3 &55.6 &77.1 &78.4 &83.5 &87.6 &63.9 &52.2 &63.9 &47.1 &53.3 &62.9\\
    AU-RCNN &50.2 &43.7 &57 &78.5 &78.5 &82.6 &87 &67.7 &49.1 &62.4 &50.4 &49.3 &63.0 \\
    UGN-B   &54.2 &46.4 &56.8 &76.2 &76.7 &82.4 &86.1 &64.7 &51.2 &63.1 &48.5 &53.6 &63.3\\
    J{\^A}A-Net &53.8 &47.8 &58.2 &78.5 &75.8 &82.7 &88.2 &63.7 &43.3 &61.8 &45.6 &49.9 &62.4\\
    SEV-Net &\textbf{58.2} &\textbf{50.4} &58.3 &\textbf{81.9} &73.9 &\textbf{87.8} &87.5 &61.6 &[52.6] &62.2 &44.6 &47.6 &63.9\\
    HMP-PS &53.1 &46.1 &56.0 &76.5 &76.9 &82.1 &86.4 &64.8 &51.5 &63.0 &[49.9] &54.5 &63.4\\
    MHSA-FFN &51.7 &[49.3] &[61.0] &77.8 &\textbf{79.5} &82.9 &86.3 & \textbf{67.6} &51.9 &63.0 &43.7 &[56.3] &64.2\\
    CISNet &54.8 &48.3 &57.2 &76.2 &76.5 &85.2 &87.2 &66.2 &50.9 &[65.0] &47.7 &\textbf{56.5} &64.3\\
    D-PAttNe$t^{tt}$ &50.7 &42.5 &59.0 &79.4 &79.0 &85.0 &[89.3] &67.6 &51.6 &\textbf{65.3} &49.6 &54.5 &64.7\\
    CaFNet &[55.1] &49.3 &57.7 &78.3 &78.6 &[85.1] &86.2 &[67.4] &52.0 &64.4 &48.3 &56.2 &[64.9]\\
    \hline
    \textbf{GLEE-Net(Ours)}  &\textbf{58.2} &48.7 &\textbf{61.5} &78.7 &[79.2] &84.2 &\textbf{89.8} &66.3 &\textbf{56.7} &64.8 &\textbf{53.5} &53.6 &\textbf{66.3}\\
    %Ours  &[57.8] &45.3 &\textbf{61.1} &[80.0] &[78.6] &[85.6] &[87.9] &\textbf{68.2} &[52.3] &[63.8] &[49.0] &\textbf{56.8} &\textbf{65.5}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

\textbf{DISFA} contains 27 video clips from 27 participants(12 females and 15 males). Each video records the facial activity of a participant when watching a 4-minutes video clip. Each clip consists of 4,845 frames evenly. Altogether, around 130,000 frames were annotated with intensities from 0 to 5. Following previous works \cite{jacob2021facial}\cite{li2018eac}\cite{shao2021jaa}\cite{yang2021exploiting}, we regard intensity labels $\{0,1\}$ as absence and others as presence. The evaluation was performed on 8 AUs(1, 2, 4, 6, 9, 12, 25, and 26. Their definition can be seen in Table \ref{tab:AUs definition}).  . We also performed the same three-fold, subject-exclusive, cross validations on 8 AUs as in the previous works \cite{li2018eac}\cite{shao2021jaa}.% following the subject division of \cite{li2018eac, shao2021jaa}.

\textbf{BP4D+} contains 1400 video clips from 140 participants(82 females and 58 males). Compared to BP4D, it has larger identity variations and video numbers. About 198,000 frames were annotated with the same 12 AUs in BP4D. We performed three-fold, subject-exclusive, cross-validations to compare our method with the state-of-the-art. Besides, to evaluate the generalization performance, our method was trained on BP4D and then evaluated on BP4D+, following the previous works \cite{attnetionTrans2019}\cite{shao2021jaa}.

To sum up, the order from largest to smallest of the three datasets is BP4D+, BP4D, and DISFA. BP4D and BP4D+ were recorded in similar shooting environments and lighting conditions. Both of them share the same 12 AU classes. In comparison, DISFA is the smallest dataset containing only 8 AU classes and was captured in quite different lighting conditions.

%以上是列举了三个数据，接下来可以做一个数据集的总结，比如说从数据量来说，xxx最少，xxx居中，最多是xxxx。也包括AU的个数也可以提一下，这里重在讲三个数据集的区别。这样方便后面实验讨论，比如我们工作可能在数据量大的数据集上表现好，等等，分析讨论结果的时候可以到这里来找理由，找依据。



% \begin{table}[!t]
% %\small
% \footnotesize
% %\setlength{\tabcolsep}{6.5pt} 
% \renewcommand\arraystretch{1.5} 
% \centering
% {
%   \caption{Ablation study of different global feature encoder pretrained on different dataset and task. Measured on BP4D by F1 scores(\%). InpResNetv1 is the abbreviation of InceptionResNetv1 }
%   \vspace{-1em}
%   \label{tab:F1 on pretrain}
%  \begin{tabular}{l|cccccccc|c}
%     \hline
%   %\textbf{Arch.} &\textbf{ResNet50} &\textbf{InceptionResNetv1} &\textbf{InceptionResNetv1}\\[1pt]
%     \textbf{Arch.} &ResNet50 &InpResNetv1 &InpResNetv1\\[1pt]
%     \hline\hline
%     \textbf{Data.} &ImageNet &ImageNet &FEC\\[1pt]
%     \textbf{Task.} &Classification &Classification &Expression similarity \\[1pt]
%     \hline
%     \textbf{F1-Score} &64.4 &63.5 & 66.3\\
%     \hline
%   \end{tabular}}
% \end{table}

%%%%%%%DISFA%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[t]
\footnotesize
\setlength{\tabcolsep}{0.9pt} 
\renewcommand\arraystretch{1.5} 
\centering
{ 
  \caption{Comparisons of our method and the state-of-the-art methods on DISFA in terms of F1 scores(\%). 
%   The best results are shown in bold, and the second best are in brackets.
  }
  \vspace{-1em}
  %\vspace{-1em}
  \label{tab:F1 on DISFA}
 % \setlength{\tabcolsep}{1.9mm}{
  \begin{tabular}{l|cccccccc|c}
   \hline 
 \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU9} &\textbf{AU12} &\textbf{AU25} &\textbf{AU26} &\textbf{Avg.}\\[1pt]
    \hline\hline
    LSVM       &10.8 &10.0 &21.8 &15.7 &11.5 &70.4 &12.0 &22.1 &21.8\\
    DRML       &17.3 &17.7 &37.4 &29.0 &10.7 &37.7 &38.5 &20.1 &26.7\\
    APL        &11.4 &12.0 &30.1 &12.4 &10.1 &65.9 &21.4 &26.9 &23.8\\
    EAC-Net        &41.5 &26.4 &66.4 &50.7 &8.5 &\textbf{89.3} &88.9 &15.6 &48.5\\
    %JAA-Net    &43.7 &46.2 &56.0 &41.4 &44.7 &69.6 &88.3 &58.4 &56.0\\
    DSIN       &42.4 &39.0 &68.4 &28.6 &46.8 &70.8 &90.4 &42.2 &53.6\\
    ARL        &43.9 &42.1 &63.6 &41.8 &40.0 &76.2 &[95.2] &66.8 &58.7\\
    LP-Net     &29.9 &24.7 &72.7 &46.8 &49.6 &72.9 &93.8 &56.0 &56.9\\
    AU-GCN      &32.3 &19.5 &55.7 &57.9 &61.4 &62.7 &90.9 &60.0 &55.0\\
    AU-RCNN  &32.1 &25.9 &59.8 &55.4 &39.8 &67.7 &77.4 &52.6 &51.3 \\
    SRERL      &45.7 &47.8 &56.9 &47.1 &45.6 &73.5 &84.3 &43.6 &55.9\\
    UGN-B      &43.3 &48.1 &63.4 &49.5 &48.2 &72.9 &90.8 &59.0 &60.0\\
    J{\^A}A-Net    &[62.4] &[60.7] &67.1 &41.1 &45.1 &73.5 &90.9 &[67.4] &63.5\\
    MHSA-FFN   &46.1 &48.6 &72.8 &\textbf{56.7} &50.0 &72.1 &90.8 &55.4 &61.5\\
    SEV-Net    &55.3 &53.1 &61.5 &[53.6] &38.2 &71.6 &\textbf{95.7} &41.5 &58.8\\
    HMP-PS     &38.0 &45.9 &65.2 &50.9 &50.8 &76.0 &93.3 &\textbf{67.6} &61.0\\
    CISNet     &48.8 &50.4 &[78.9] &51.9 &47.1 &[80.1] &[95.4] &65.0 &64.7\\
    CaFNet     &45.6 &55.7 &\textbf{80.2} &51.0 &\textbf{54.7} &79.0 &95.2 &65.3 &[65.8]\\
    \hline
    \textbf{GLEE-Net(Ours)}    &\textbf{63.5} &\textbf{62.5} &69.8 &48.6 &[53.9] &75.6 &94.7 &64.4 &\textbf{66.6}\\
    \hline
  \end{tabular}}%}
\end{table}

%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art methods on BP4D+ in terms of F1 scores(\%). 
%   The best results are shown in bold.
  }
 \vspace{-1em}
  \label{tab:F1 on ThreeFoldBp4DPlus}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline
    FACS3D-Net     &43.0 &38.1 &\textbf{49.9} &82.3 &85.1 &87.2 &87.5 &66.0 &48.4 &[47.4] &50.0 &[31.9] &59.7\\
    ML-GCN &40.2 &36.9 &32.5 &84.8 &[88.9] &89.6 &[89.3] &81.2 &[53.3] &43.1 &55.9 &28.3 &60.3\\
    MS-CAM &38.3 &37.6 &25.0 &85.0 &\textbf{90.9} &\textbf{90.9} &89.0 &[81.5] &\textbf{60.9} &40.6 &58.2 &28.0 &60.5\\
    SEV-Net &[47.9] &\textbf{40.8} &31.2 &\textbf{86.9} &87.5 &89.7 &88.9 &\textbf{82.6} &39.9 & \textbf{55.6} &[59.4] &27.1 &[61.5]\\
    \hline
    \textbf{GLEE-Net(Ours)}  &\textbf{51.5} &[46.6] &[43.5] &[86.8] &89.6 &[91.0] &\textbf{89.8} &82.3 &46.8 & 49.3 &\textbf{60.9} &\textbf{50.9} &\textbf{65.7}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!t]
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art on cross-dataset evaluation(trained on BP4D and evaluated on BP4D+) in terms of F1 scores(\%). 
%   The best results are shown in bold.
  }
 \vspace{-1em}
  \label{tab:F1 on Bp4DPlus}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline
    EAC-Net     &38.0 &[37.5] &[32.6] &82.0 &83.4 &87.1 &85.1 &62.1 &44.5 &43.6 &45.0 &32.8 &56.1\\
    ARL         &29.9 &33.1 &27.1 &81.5 &83.0 &84.8 &86.2 &59.7 &[44.6] &43.7 &48.8 &32.3 &54.6\\
    J{\^A}A-Net &\textbf{39.7} &35.6 &30.7 &[82.4] &[84.7] &[88.8] &[87.0] &[62.2] &38.9 &[46.4] &[48.9] &\textbf{36.6} &56.8\\
    \hline
    \textbf{GLEE-Net(Ours)}  &[39.5] &\textbf{37.7} &\textbf{44.0} &\textbf{84.5} &\textbf{84.9} &\textbf{89.6} &\textbf{87.7} &\textbf{72.3} &\textbf{44.9} & [45.3] &\textbf{52.6} &[33.9] &\textbf{59.7}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

\subsection{Implementation Details}

Face images were first aligned and cropped according to landmark detection results. Before feeding to our networks, the input images were resized to $256\times256$. The resolution of feature maps was reduced to $16\times16$ after passing through the Feature Encoder.

To enhance the feature extraction capability of low-level convolution layers, the feature encoder was initialized with the corresponding network parameters pretrained on the dataset of ImageNet or FEC, and the rest of our networks were set to Kaiming initialization \cite{he2015delving}. Except for the Mask Decoder, the whole model parameters were updated by employing an Adam optimizer with hyper-parameters $\beta = 0.9$ and weight decay $10^{-6}$.
%可能要斟酌一下要不要写MaskDecoder部分参数冻结，要写的话如何说清和证明它的作用

The networks were trained for 20 epochs with an initial learning rate of $10^{-5}$ on each dataset fold. The mini-batch size was set to 10. We used a warm-up stage with $10^3$ steps and then decayed the learning rate exponentially with an exponent $-0.5$. The training and inference pipelines were implemented in Pytorch on 4 GeForce GTX 2080ti GPU. 
%这里就可以给一张训练集和验证集，随着时间，收敛的情况，可以分AU来说，我们也可以观察下，哪些AU收敛快，哪些慢，哪些容易过拟合，哪些比较好泛化，等等，这个图都是可以用来分析后面的实验结果，避免实验结果太干涩，没话说。


\subsection{Comparisons with the State-of-the-Art}
We compared our method with many state-of-the-art AU detection methods, including LSVM \cite{LSVM}, JPML \cite{JPML}, DRML \cite{DRML}, APL \cite{LP48}, EAC-Net \cite{li2018eac}, DSIN \cite{LP8}, ARL \cite{attnetionTrans2019}, SRERL \cite{SRERL}, AU-GCN\cite{liu2020relation},AU-RCNN\cite{ma2019r}, ML-GCN \cite{chen2019multi}, MS-CAM \cite{you2020cross}, LP-Net \cite{LP}, FACS3D-Net \cite{yang2019facs3d}, UGN-B \cite{song2021uncertain}, J{\^A}A-Net \cite{shao2021jaa}, MHSA-FFN \cite{jacob2021facial}, SEV-Net \cite{yang2021exploiting}, HMP-PS \cite{song2021hybrid}, D-PAttNe$t^{tt}$\cite{Onal2019D-PAttNet}, CISNet\cite{chen2022causal} and CaFNet\cite{chen2021cafgraph}. 


Specifically, while EAC-Net, ARL, J{\^A}A-Net, and SEV-Net were evaluated on all three datasets, LSVM, JPML, DRML, APL, DSIN, SRERL, AU-GCN, AU-RCNN, LP-Net, UGN-B, MHSA-FFN, HMP-PS, CISNet and CaFNet were evaluated on both BP4D and DISFA. Particularly, D-PAttNe$t^{tt}$ was only evaluated on BP4D. FACS3D-Net, ML-GCN and MS-CAM were evaluated merely on BP4D+. Since BP4D+ is released later, it is not used by all the methods.
%\textcolor{red}{[Reviewers may question why not evaluate all the methods on all the three datasets? Any particular reasons doing so? If so, it would be better to explain the reasons here.]} %这里就可以说下，哪些方法是在三个数据集上测试，哪些仅仅是两个数据，这些都是为后面分数据集汇报结果准备，避免人家说，为什么不同数据集，baseline方法却不一样。

Following the experimental settings of most previous works, we also employed the F1 score \cite{F1} on the frame level as the evaluation metric. F1-score is a harmonic mean of precision(P) and recall(R), which is defined as $F1 = 2PR/(P+R)$. Since F1-score takes both false positives and false negatives into account, it reflects a more rational measurement of the model's performance than accuracy, especially on datasets with uneven class distributions like BP4D, DISFA, and BP4D+.



\textbf{Evaluation on BP4D.}
The results on BP4D are shown in Table \ref{tab:F1 on Bp4D}. The average F1 score of our method is 66.3\%, which significantly outperforms all the other comparison methods, improving about 1.4\% over the second highest one, CaFNet. In terms of the performances on single AUs, our method achieves the highest F1 scores among all the methods on 5 AUs(i.e., AU1, AU4, AU12, AU15, and AU23) and second highest on 1 AUs(AU7) of the 12 evaluated AUs. Besides, our method shows over 3.5\% superiority on AU15 and AU23 over the second highest ones. 


In terms of AU feature learning, our method outperforms JMPL, DRML, and D-PAttNe$t^{tt}$ about 20.4\%, 18\% and 1.6\%, demonstrating that extracting local features by attention is more effective and our method is superior in AU feature extraction than patch learning. 

Compared with EAC-Net, JAA-Net, and MHSA-FFN, which utilize attention mechanisms with the supervisions of pre-defined AU centers, our method achieves improvements of 10.4\%, 5.2\% and 3.9\% over them(EAC-Net, JAA-Net, and MHSA-FFN), respectively. This validates the superiority of our non-predetermined AU attention learning approach.  %\textcolor{red}{I think we can improve the structure of the above text.}


%\textcolor{red}{Compared to SEV-Net and J{\^A}A-Net that employ textual embedding and facial landmarks as auxiliary training information, our method obtains better results with the compact expression embedding as prior knowledge. WHAT DO WE WANT TO EXPRESS}


\textbf{Evaluation on DISFA.}
Table \ref{tab:F1 on DISFA} shows the evaluation results on DISFA. As shown in this table, our method achieves the average F1 score of 66.6\%, outperforming all the compared state-of-the-art methods. 

Compared to the most recent works SEV-Net, HMP-PS, MHSA-FFN, CISNet and CaFNet, our method achieves an improvement of 7.8\%, 5.6\%, 5.1\%, 1.9\% and 0.8\% over them, respectively. Unlike EAC-Net and J{\^A}A-Net which are supervised by both AU and landmark labels, our method only utilizes AU labels, but still obtains significant improvements of 18.1\% and 3.1\% over EAC-Net and J{\^A}A-Net, respectively, demonstrating the effectiveness of our method in AU feature and attention learning. Note that our method does not explicitly model AU relationships, but significantly exceeds all relation-based methods including JMPL, DSIN, ARL, AU-GCN, and AU-RCNN.

%As the number of subjects in DISFA is smaller than that of BP4D, \textcolor{red}{most of the previous methods suffer from overfitting to the appearance of training subjects more severely. WHY?} Therefore, benefiting from our identity-independent expression representations, our method achieves an even more significant improvement.

\textbf{Evaluation on BP4D+.}
Table \ref{tab:F1 on ThreeFoldBp4DPlus} shows the evaluation results of the three-fold cross-validation on BP4D+.
In particular, the results of SEV-Net, ML-DCN and MS-CAM are reported in\cite{yang2021exploiting} while the results of EAC-Net are reported in \cite{shao2021jaa}. 
Our method achieves the F1 score of 65.7\% and outperforms all the state-of-the-art methods, exceeding SEV-Net over 4.2\%.

%%%%%%%%%%%%%
% %%%%%%%%%%%%%pose_mask figure
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[ width=18cm]{images/sample4.pdf}
%     %\vspace{-0.5em}
%     \caption{Illustration of attention map on different head pose. The Mask Decoder generates  similar masks with various pose images input, demonstrates that the mask decoder is robust to head pose}
%     \label{fig:pose_mask}
% \end{figure*}
% %%%%%%%%%%%%%

To further evaluate the generalization performance of our method on large-scale test identities, we trained our method on BP4D and evaluated it on the full BP4D+ of 140 subjects. The results are shown in Table \ref{tab:F1 on Bp4DPlus}. We use the reported results in the work \cite{shao2021jaa} for comparison. Again, our method outperforms all the compared methods under the large-scale cross-dataset evaluation. It indicates that our method can extract identity-independent information and generalize well to new identities.

%\textcolor{red}{[if possible, I suggest to move the tables/figures to the same page as the first cited place/page. Or if it cannot be achieved, the place of tables/figures should be as close as possible to the first cited place/page. This would increase the readability.]}

%From the evaluation results on the three datasets, we can see that AU7, AU12 and AU17 rechieve best performances on BP4D, and AU1 and AU2 gets best results on DISFA. 
%综合看三个数据集的结果，可以谈谈哪些AU，我们的方法总是获胜，哪些总是不好，然后可以分析原因。

\subsection{Ablation Study}
%先简要回顾下我们的算法框架，其实有挑选的介绍，然后再说我们要逐一验证这些框架子模块的设计，才进行了ablation study。（提高文章的过度和可读性）

%As described in Section \ref{sec:methodology}, our framework includes the global feature encoder followed by two branches of feature decoders, namely, facial feature decoder($D_f$) and facial mask decoder($D_m$). While the $D_f$ module creates one initial feature map for each AU, the $D_m$ module is responsible for learning feature masks that filter out the areas irrelevant to current AU. Then, by a point-wise multiplication of the initial feature map $xx$ and the feature mask from $D_f$ and $D_m$, we obtain the feature map  $xx$ of AU-related local regions for each AU. $we have to clearly indicate what we will validate by our ablation studies.$
In this section, we conduct ablation studies to evaluate the effectiveness of each key sub-module in our framework, including: 1) the prior knowledge of expression similarity learning, 2) the facial components module, 3) and mask activation.In particular, all the ablation experiments are conducted on the BP4D dataset due to space limitations. The experimental results are reported in Table~\ref{tab:F1 on Ablation 2}. 

%As shown in Table~\ref{tab:F1 on Ablation}, we firstly construct a baseline model(Baseline), of which the feature extractor is based on InceptionResNetv1 without pretrained parameters, followed by AU classifiers. Besides, to verify the validity of the pretrained expression featrue encoder, we load parameters pretrained on ImageNet(Baseline-ImageNet) and on FEC(Baseline-FEC) respectively. For further validation of our facial feature decoder($D_f$) and facial mask decoder($D_m$), we gradually add $D_f$(Baseline-FEC-DF ) and $D_m$(Baseline-FEC-DF-DM) .  

%Furthermore, as shown in Table \ref{tab:F1 on Ablation 2}, to explore the effectiveness of each implementation, we replace or remove certain individual modules of the full framework and test the model performance. For instance, freezing the pretrained Feature Encoder weights(w.fixed FE), replacing the activation function of mask decoder with softmax(w. Softmax), etc. The experiments results will be analysed in detail in the following paragraphs.   %既然这里提到了表格4，这里就定义出表格4中各种消融方法的定义
%anrudong: 表格中涉及到的各个消融实验方法的定义下文有分模块详细介绍，如果在这里再写一遍显得有些重复,因此删掉

% \begin{table*}[!t]
% %\small
% \footnotesize
% \setlength{\tabcolsep}{8pt}
% \renewcommand\arraystretch{1.5} 
% \centering
% {
%   \caption{Ablation study on BP4D measured by F1 scores(\%).}
%   \vspace{-1em}
%   \label{tab:F1 on Ablation}
%  \begin{tabular}{l|cccccccccccc|c}
%     \hline
%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{F1-Score} \\[1pt]
%     \hline\hline
%     % Baseline        &- &-  &- &- &52.6\\
%     % Baseline-ImageNet         &$\surd$ &- &- &- &61.6 \\
%     Baseline-FEC         &- &$\surd$ &- &- &63.3 \\
%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &- &63.8 \\
%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &- &63.7 \\
%     Baseline-FEC-DF-DM/GLEE-Net(Full)       &- &$\surd$ &$\surd$ &$\surd$ &66.3 \\
%     % Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\
%     \hline
%   \end{tabular}}
% \end{table*}

\begin{table*}[!t]
%\small
\footnotesize
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Ablation study on BP4D measured by F1 scores(\%). }
  \vspace{-1em}
  \label{tab:F1 on Ablation 2}
 \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline\hline
    w/o pretrain &34.9 &24.2 &36.7 &76.1 &71.4 &81.0 &86.3 &58.7 &25.9 &51.9 &27.4 &31.6 &50.5\\
    w. FE Emotion &48.1 &41.6 &53.9 &78.6 &77.9 &83.2 &88.8 &60.5 &39.3 &65.5 &38.0 &47.6 &60.3 \\
    w. FE ImageNet &49.6 &39.7 &60.5 &77.3 &78.7 &83.1 &88.6 &[64.6] &48.2 &63.2 &47.5 &48.0 &62.4 \\
    w. FE fixed &52.3 &45.8 &59.8 &[79.4] &78.1 &\textbf{84.8} &89.0 &64.0 &46.5 &64.0 &38.6 &49.8 &63.5\\
    % w. ResNet &[56.9] &46.5 &57.2 &78.1 &[79.2] &84.2 &87.9 &63.8 &51.0 &64.7 &49.5 &[53.5] &[64.4]\\
    \hline
    w/o DM\&DF &[55.4] &\textbf{65.1} &\textbf{73.9} &49.0 &46.9 &77.1 &\textbf{92.9} &54.1 &48.1 &64.7 &[52.5] &47.5 &63.3\\
    w/o DM  &53.3 &44.2 &58.7 &78.6 &76.9 &83.9 &[89.8] &62.2 &48.9 &65.1 &[52.5] &51.8 &63.8\\
    w/o DM\& w. CNN &51.8 &43.0 &59.1 &79.3 &78.1 &84.4 &89.0 &63.1 &50.5 &64.3 &49.2 &\textbf{55.1} &63.9\\
   % w. PE & 54.8 &45.3 &[63.4] &78.4 &79.1 &[84.6] &89.1 &60.7 &49.7 &64.2 &50.7 &50.3 & 64.2\\
    
    \hline
    w. None & 53.7 &44.6 &55.4 &78.6 &78.4 &83.7 &89.2 &[64.6] &[51.4] &\textbf{65.9} &51.2 &52.6 &64.1\\
    w. SoftMax & 53.6 &43.8 &58.5 &\textbf{79.7} &[79.2] &84.5 &89.6 &63.4 &50.3 &62.7 &50.8 &53.0 &64.0\\
    w. Tanh &55.1 &46.2 &60.2 &79.1 &\textbf{79.3} &[84.6] &88.d6 &63.0 &49.6 &[65.3] &51.8 &50.2 &[64.4]\\ 
  
    \hline
    \textbf{GLEE-Net(Full)} &\textbf{58.2} &[48.7] &[61.5] &78.7 &[79.2] &84.2 &[89.8] &\textbf{66.3} &\textbf{56.7} &64.8 &\textbf{53.5} &[53.6] &\textbf{66.3}\\
    %GLEE-Net(Full) & 53.7 &[48.4] & 59.8 & \textbf{79.7} & 78.9 &83.5 & 89.5 &\textbf{64.0} &[50.6] &64.1 &50.2 &[53.4] &\textbf{64.7}\\
    \hline
  \end{tabular}}
\end{table*}

%\textcolor{red}{here we need a head text to briefly introduce what we will presents.}
\textbf{Prior Knowledge.} 
% \textcolor{red}{here we have to make a head paragraph to introduce what we will presents. What will we study? It looks three ablation studiese here.}
Our framework proposes a vision feature encoder $E_f$ that is pretrained on the FEC dataset via expression similarity learning, which refers to our prior knowledge. To test the efficiency of prior knowledge, we design ablation experiments with different approaches to initialize $E_f$ in the training of $GLEE-Net$, including:
\begin{itemize}
    \item [a) ]
    w/o pretrain: $E_f$ is randomly initialized;
    \item [b) ]
    w. FE Emotion: $E_f$ is initialized via a pretrained classifier of seven discrete facial expression emotion (e.g. neutral, happy, sad, surprise, fear, disgust, angry) categories trained on the AffectNet dataset;
    \item [c) ]
     w. FE ImageNet: $E_f$ is initialized via a pretrained image object classifier built on imageNet \cite{krizhevsky2012imagenet};  
    \item [d) ]
     w. FE fixed: $E_f$ is our proposed method, initialized via the facial expression similarity; 
    \item [e) ]
     GLEE-Net(Full): $E_f$ is parameterized by the facial expression similarity approach but it not updated in the training of $GLEE-Net$.
\end{itemize}


% 1-{2-4}: prior k is necessary;
% 4-2/3: ours is ok;
% 4-5: finetuning

Firstly, in comparison with random initialization (w/o pretrain),
the experiments of b), c) and d) achieve improvements of 9.8\%(from 50.5\% to 60.3\%), 11.9\%(from 50.5\% to 62.4\%) and 15.8\%(from 50.5\% to 66.3\%), respectively. This indicates that the prior knowledge is necessary and the pretraining progress can bring significant improvement for AU detection.

Secondly, compared with the other two pretraining approaches(w. FE Emotion and w. FE ImageNet), the network initialized by our facial expression similarity pretraining(GLEE-Net(Full)) obtains the best performance(66.3\%), exceeds the other two pretraining methods(w. FE Emotion and w. FE ImageNet) about 6\% and 3.9\%. This proves the effectiveness and superiority of the prior knowledge captured by our facial expression similarity learning. 

Lastly, in condition of loading the feature encoder with parameters pretrained by our expression similarity learning, compared with finetuning the whole network(GLEE-Net(Full)), it obtains a lower average F1 of 63.5\% if we fix the feature encoder($E_f$) during training(w. FE fixed). It indicates that finetuning the feature encoder is beneficial for extracting features which are more adaptive to the following FCM module. Thus finetuning operation is essential and efficient to improve the performance of our framework. 

% the experiment e) with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE) obtains a lower average F1 of 63.5\% compared with the experiment d)

% Firstly, we design a baseline model, which is constructed with the feature encoder(without pretrained parameters) followed by the AU classifier module.
% Particularly, the followed AU classifier has a similar structure to the AU classifier of the full network but with a different size due to the input feature size difference. As shown in table~\ref{tab:F1 on Ablation}, we test the baseline without pretrained parameters(Baseline), with parameters pretrained on ImageNet(Baseline-ImageNet) and with parameters pretrained on FEC(Baseline-FEC). The Baseline-FEC and the Baseline-ImageNet achieve  63.3\%  and 61.6\%, respectively.  Compared with the baseline model(52.6\%), they bring over 10.7 and 9\% improvements, which validates the importance of pretraining. Moreover, the Baseline-FEC achieves an improvement of 1.7\% compared with the Baseline-ImageNet, proving the superiority of our pretraining on FEC with expression similarity task.

% Secondly, based on our full framework(GLEE-Net), we load the feature encoder with various pretrained weights. As shown in table~\ref{tab:F1 on Ablation 2}, we first test the full network without any pretrained weights(w/o pretrain), then load the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), AffectNet(w. FE Emotion) and FEC(GLEE-Net) respectively.  Specifically, the whole networks of the above experiments(except for w/o pretrain) are finetuned on BP4D. The results in table~\ref{tab:F1 on Ablation 2} show that when loading the parameters pretrained with the expression similarity task(GLEE-Net), it achieves the best F1-Score(66.3\%), while loading parameters pretrained on AffectNet(w. FE Emotion) and ImageNet(w. FE ImageNet) it declines 3.9\% and 6\%. This further verifies the effectiveness of the prior knowledge of expression similarity learning. 

% Thirdly, we also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in Table \ref{tab:F1 on Ablation 2}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. It shows that the finetuning operation is effective to improve the performance of our framework.  

%gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.

%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.

%We first evaluate the effectiveness of pretraining. As illustrated in Table~\ref{tab:F1 on Ablation}, the baseline has the same structure as the feature encoder($E_f$) of our full network but does not load any pretrained parameters(\textit{Baseline}), which is followed by a classifier module \textcolor{red}{what does a classifier module refer to?}. Then we test it with pretrained parameters on ImageNet, namely, \textit{Baseline-ImageNet}. As shown in Table \ref{tab:F1 on Ablation}, the Baseline-ImageNet achieves 61.6\% and brings over 9\% improvement than the baseline(52.6\%), which validates the importance of pretraining.

%the baseline is constructed based merely on an InceptionResNetV1 network without pretraining. It has the same structure as the feature encoder of our full network, using the intermediate features which has a resolutioin of 16 x 16. The feature encoder of the baseline is followed by several classifer modules similar to AU Classifer Module. The number of classifier modules is corresponding to the AU classes. Each classifier module predicts a specific AU's probability and shares the same structure that contains 3 CNN layers and a Sigmoid activation at the last layer. Then we test the baseline with pretrained parametes on ImageNet, namely Baseline-ImageNet. As shown in Table \ref{tab:F1 on Ablation}, it achieves 61.6\% and brings over 9\% improvement compared with baseline(52.6\%), proving the importance of pretraining.
% 我感觉直接介绍pretrained feature model 部分即可，无需再介绍后面的classifier啥的结构了。

%To test the efficiency of our feature encoder pretrained on FEC with the facial expression similarity task, we replaced the feature encoder of our full network with different architectures or parameters and then fine-tuned the whole network on BP4D. 

%As shown in Table \ref{tab:F1 on Ablation 2}, we first load the weights of the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), then load the weights with parameters pretrained on an emotion dataset(AffectNet) by the emotion recognition task(w. FE Emotion). We also take ResNet50 pretrained on ImageNet as the feature encoder of our full network(w. ResNet50). 

%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.
%\textcolor{red}{looks no table for the above results. I dont know why the above uses DISFA and teh below uses the other two datsets.}

%To futher indicate the significance of the pretrained facial expression embedding network, we also test it on the BP4D dataset. First, we replace the feature encoder with a ResNet~\cite{Resnet34}~(w. ResNet50 in Table~\ref{tab:F1 on Ablation 2}). The results show that using pretrained facial expression embedding network as backbone improves the score by 3\% on BP4D. 


%We also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in the Table \ref{tab:F1 on Ablation}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. This shows that the fine-tuned operation is effective to improve the performance of our framework. 
%\textcolor{red}{Any more discussion here?.}



\textbf{Facial Components.}
To validate the effectiveness of the representations extracted by our facial components module (FCM), we conduct several ablation experiments. Concretely, based on our full framework of GLEE-Net, we remove or replace some specific sub-modules and retrain the whole network, including:
\begin{itemize}
    \item [1) ]
    w/o DM\&DF: removing both the mask decoder(DM) and the feature decoder(DF);
    \item [2) ]
    w/o DM: only removing the mask decoder(DM);
    \item [3) ]
    w/o DM& w. CNN: removing the mask decoder(DM) and replacing the feature decoder(DF) with a CNN block in the meanwhile. Particularly, the CNN block has similar number of parameters with our feature encoder($E_f$).
\end{itemize}

%Specifically, based on the feature encoder pretrained on FEC(Baseline-FEC in Table~\ref{tab:F1 on Ablation} or w/o DM\&DF in Table~\ref{tab:F1 on Ablation 2}), we gradually added the $D_f$ branch(Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation} or w/o DM in Table~\ref{tab:F1 on Ablation 2}) and the $D_m$ branch(Baseline-FEC-DF-DM in Table~\ref{tab:F1 on Ablation} or GLEE-Net in Table~\ref{tab:F1 on Ablation 2}). In addition, we replaced the facial feature decoder of Baseline-FEC-DF with a CNN structure module(Baseline-FEC-CNN) to further validate the effectiveness of the facial feature decoder.

%\textcolor{red}{Why BP4D only? why not the other two datasets.}
%Firstly, based on the feature encoder pretrained on FEC(Baseline-FEC), when adding the $D_f$ branch(Baseline-FEC-DF), the F1-score improves 0.5\%(from 63.3\% to 63.8\%). Further introducing the  $D_f$ and the $D_m$(Baseline-FEC-DF-DM), the results improves 2.5\%. 
%we construct the model only with the Feature Encoder ~(w/o MD \& FD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC in Table~\ref{tab:F1 on Ablation}) or the Facial Decoder branch~(w/o MD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation}) individually. %a decline of 2.5\%(from 66.3\% to 63.8\%) is caused when the Mask Decoder is removed(Baseline-FEC-DF) and 3\% decline(from 66.3\% to 63.3\%) when the Facial Decoder is also removed(Baseline-FEC) respectively. 

%%%%%%%%%%%%%pipeline figure
\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/sample1.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the decoded mask attention maps:(Left) samples from DISFA, and(Right) samples from BP4D and BP4D+. The learned masks(odd rows) are also visualized and overlaid on the corresponding face images(even rows). The colors covering on the face images from blue to red indicate the attention values from low to high.}
    \label{fig:figure1}
\end{figure}
%%%%%%%%%%%%%

%%%%%%%%%%%%%mask figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample2.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the mask attention maps overlaid onto the corresponding input images in BP4D. The first column shows face images with different expressions. We can observe that similar AU-related local mask distributions can be learned by our framework even though the identities and expressions vary significantly.  }
    \label{fig:mask visualization}
\end{figure*}
%%%%%%%%%%%%%avtivation figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/sample3.pdf}
    %\vspace{-0.5em}
    \caption{Visualization of the mask maps generated by different activation functions(Sigmoid, softmax, and Tanh, from top to bottom) on each AU from the BP4D dataset. The masks of softmax are more sparse than those of Sigmoid and Tanh because it has an extra restriction between AU channels. Therefore, softmax may filter out some related regions.}
    \label{fig:avtivation}
\end{figure*}
%%%%%%%%%%%%%
Note that the inclusion of DF alone(w/o DM) brings an improvement of 0.5\%(from 63.3\% to 63.8\%) in comparision to w/o DM\&DF. When the facial feature decoder is replaced by the CNN module, the performance declines by 0.1\%(from 63.8\% to 63.7\%) on F1-Score. Moreover, the performance improves by 2.3\% when we further added the facial mask decoder module and constructed our full network, GLEE-Net. These study results validate the effectiveness of our attention and local feature learning.
% In the experiment without pretraining on the expression dataset~(w/o pretrain), we can see an apparent drop in average F1-score of .

%\textcolor{red}{[It seems the two rows(w/o DM, and w/o DM\&DF) in Table 7 are not used/cited in the main texts. So, reviewers may question why you put the two rows in Table 7?]}\textcolor{blue}{[has been referred]}

\textbf{Mask Activations. }
To explore the effect of activation functions on attention mask generation, we tried three activation methods on the outputs of the mask decoder. The results are shown in Table \ref{tab:F1 on Ablation 2}. When there is no activation on the mask decoder's outputs(w. None), it achieves an F1 score of 64.1\%. The Sigmoid function(GLEE-Net(Full)) obtains the best result of F1-score 66.3\%. While Softmax(w. SoftMax) achieves an F1-score of 64.0\% and Tanh(w. Tanh) achieves 64.4\%. We can see that the Sigmoid and Tanh can achieve better performance than SoftMax. The possible reason is that the masks generated by Softmax tend to get sparse attention maps and exclude other parts including regions related to the target AU in most cases. This may result in the downstream recognition task being unable to learn sufficient information. In contrast, Sigmoid and Tanh can avoid the above shortcoming and retain the regions that are closely related to the target AU, making the subsequent Classifier Module have a better performance. 


%%%%%%%%%%%%%tsne figure
\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/tsne.pdf}
    %\vspace{-0.5em}
    \caption{t-SNE visualization of the AU embeddings generated by our framework w/ or w/o the mask decoder module on the BP4D dataset. }
    \label{fig:tsne}
\end{figure}
%%%%%%%%%%%%%

\subsection{Visual Analysis}
We also visualize the feature and mask results of our framework to further validate its effectiveness.

\textbf{Mask Attention Learning.} Due to its anatomical definition, each AU involves a group of muscle motions and is relative to a specific region in the face. For instance, AU1 is inner brow raising and AU9 is nose wrinkle. Theoretically our framework should learn a regional mask activation map for each AU, corresponding to its muscle actions. To validate the effectiveness of our mask feature learning, in Figure~\ref{fig:figure1} we visualize the attention mask maps of several 
examples from DISFA, BP4D and BP4D+, learned by our network. As shown in this figure, we can see that our method successfully captures a discriminative attention mask for each AU. Taking AU4(brow low) and AU7(lid tight) as examples, the learned spatial masks are around the brows and 
lower eyelids, respectively, which demonstrates that our proposed mask decoder is effective for AU-related local regional attention learning.

From Figure~\ref{fig:mask visualization}, we can see that each AU's mask is closely related to its muscle region, even for different expressions such as happy, sad, and fear.
We also notice that several different AUs may cover the same or similar area. This is attributed to that different AUs may share the same or similar muscle distributions. For instance, all of AU1, AU2, and AU4 are involved with the forehead, while all of AU14, AU15, AU17, AU23, and AU24 are closely related to the mouth area. Besides, considering the existence of potential mutual relations among different AUs, the masks learned merely supervised by AU labels may include other facial regions of correlated AUs. For instance, the masks of AU1, AU2, and AU4 not only cover the regions of the brows but also contain the mouth area.

\textbf{Mask Features Analysis.} Baseline-FEC-DF is a network of the encoder-decoder structure. On top of it, we can further add a mask decoder(DM) to obtain our full framework, namely, Baseline-FEC-DF-DM. The only difference between them is the absence/presence of the mask decoder sub-module. To validate the importance of mask learning, we visualize the embeddings of the AU classifiers of the above two structures. We sampled some images and obtained the t-SNE visualization of their AU embeddings. As illustrated in Figure~\ref{fig:tsne}, each color refers to a class of AU presentations. Obviously, the presentations learned with the mask decoder are more compact and have better distribution than that without the mask decoder. Moreover, all the AU embeddings learned with the mask decoder tend to gather into two clusters(positive and negative). By contrast, the presentations generated without the mask decoder display like a long strip and are not divided into two clusters for the cases of AU2, AU4, AU15, AU17, and AU23. As a result, these AUs cannot be well distinguished between positive and negative samples. This validates that the mask learning module in our framework is effective to capture discriminative local features that are beneficial to AU recognition.

\textbf{Analysis of Different Mask Activation Functions}.
Each mask  is responsible for an AU in our framework, and the mask indicates the spatial locations that are important for the recognition of the target AU. We compared three different activation functions to obtain our masks, namely, Softmax, Tanh and Sigmoid. As shown in Figure~\ref{fig:avtivation}, different activations on the outputs of the Mask Decoder bring various mask attention maps. As expected, the masks generated by the Softmax activation function are the most sparse among the three activation functions. This attribute to the restriction on the sum of all AU masks: their values must be in the range from 0 to 1, and thus reducing the overlap between masks. In comparison, the other two activation functions, Sigmoid and Tanh, can obtain a more dense map for each AU because there is no restriction between different masks. Besides, Sigmoid learns better mask maps than Tanh for the reason that its estimation value domain exactly matches the attention. Sigmoid can also capture the relation between different AUs. For instance, AU1, AU2, and AU4 activate not only the location of brows but also the mouth area, because expressions with brow movements usually accompany mouth movements in the training dataset. 


%\textcolor{red}{[Figure 8 is not cited anywhere in the main texts. If not cited/used in the main texts, reviewers may question why Figure 8 should be included into the paper.]}\textcolor{blue}{[has been deleted]}











==> experiment_bk4.tex <==
\section{\section{Experimental Results}}% \begin{table*}[!t]% \begin{table*}[!t]% %\small% %\small% \footnotesize% \footnotesize% \setlength{\tabcolsep}{2pt}% \setlength{\tabcolsep}{2pt}% \renewcommand\arraystretch{1.5} % \renewcommand\arraystretch{1.5} % \centering% \centering% {% {%   \caption{Ablation study on BP4D measured by F1 scores(\%).}%   \caption{Ablation study on BP4D measured by F1 scores(\%).}%   \vspace{-1em}%   \vspace{-1em}%   \label{tab:F1 on Ablation}%   \label{tab:F1 on Ablation}%  \begin{tabular}{l|cccccccccccc|c}%  \begin{tabular}{l|cccccccccccc|c}%     \hline%     \hline%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Classifier} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{Position-Encoding} &\textbf{F1-Score} \\[1pt]%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Classifier} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{Position-Encoding} &\textbf{F1-Score} \\[1pt]%     \hline\hline%     \hline\hline%     Baseline        &- &- &$\surd$  &- &- &- &52.6\\%     Baseline        &- &- &$\surd$  &- &- &- &52.6\\%     Baseline-ImageNet         &$\surd$ &- &$\surd$ &- &- &- &61.6 \\%     Baseline-ImageNet         &$\surd$ &- &$\surd$ &- &- &- &61.6 \\%     Baseline-FEC         &- &$\surd$ &$\surd$ &- &- &- &63.3 \\%     Baseline-FEC         &- &$\surd$ &$\surd$ &- &- &- &63.3 \\%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &$\surd$ &- &- &63.8 \\%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &$\surd$ &- &- &63.8 \\%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &$\surd$ &- &- &64.0 \\%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &$\surd$ &- &- &64.0 \\%     Baseline-FEC-DF-DM       &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &- &66.3 \\%     Baseline-FEC-DF-DM       &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &- &66.3 \\%     Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\%     Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\%     \hline%     \hline%   \end{tabular}}%   \end{tabular}}% \end{table*}% \end{table*}%To validate our proposed method, the evaluation is conducted on three public datasets commonly-used for AU detection. These datasets contain face expression images with manually-annotated action unit labels. For fair comparisons, our evaluation follows the prior works, using three-fold cross validation. The reported results are the averages from three-fold experiments. This section introduces the detail experiment settings, evaluate the effectiveness on each module, and visualize the intermediate results generated by the framework at last.%To validate our proposed method, the evaluation is conducted on three public datasets commonly-used for AU detection. These datasets contain face expression images with manually-annotated action unit labels. For fair comparisons, our evaluation follows the prior works, using three-fold cross validation. The reported results are the averages from three-fold experiments. This section introduces the detail experiment settings, evaluate the effectiveness on each module, and visualize the intermediate results generated by the framework at last.We first introduce the used three datasets in detail and then describe the implementation details of the training and validation processes. Furthermore, we compare our method with the start-of-the-art methods to demonstrate the superiority of our approach. For fair comparisons, our evaluation follows the prior works \cite{li2018eac,shao2021jaa} \cite{li2018eac,shao2021jaa}, using three-fold cross-validation and also their specific division of training and validation data(see below). The reported results are the averages from three-fold experiments. To further obtain insight into our method, we designed ablation experiments to study the impact of the built sub-modules. Finally, we visualize several samples to further validate our method.% -datasets% -datasets% - impletmenttation dedails% - impletmenttation dedails% - results, validate our method by comparing with baselines% - results, validate our method by comparing with baselines% - further to get insight to our method, validate our careful-designe, ablation study...% - further to get insight to our method, validate our careful-designe, ablation study...% - visual reatuls% - visual reatuls\subsection{\subsection{Datasets}}As mentioned above, our evaluation was performed on three widely-used AU detection datasets: BP4D \cite{BP4D}, DISFA \cite{Ma \cite{BP4D}, DISFA \cite{MavadatiDISFA}, and BP4D+ \cite{zhang2016multimodal} \cite{zhang2016multimodal}. All the above datasets were annotated with AU labels by certified experts for each frame.%可以展开说下标注过程，比如观看视频，还是观察单帧，等等。如果标注过程没有区别，那么就集中写在前面，否则可以写在每个数据集文字内部。%可以展开说下标注过程，比如观看视频，还是观察单帧，等等。如果标注过程没有区别，那么就集中写在前面，否则可以写在每个数据集文字内部。%anrudong: 三个数据集均在视频序列上逐帧进行标注，标注方式写在了每个数据集各自的介绍部分%anrudong: 三个数据集均在视频序列上逐帧进行标注，标注方式写在了每个数据集各自的介绍部分%yuding: 是的，我知道，需要在前面整体说一下三个数据集的共性和区别（概括说就好），说了之后，你再分数据集单独说，读者读起来就顺，知道下面三个数据集是在对上面共性和差异性的展开。如果不说，下面三个数据集就像三块砖头摆在那里，没有语言把它们拎起来。%yuding: 是的，我知道，需要在前面整体说一下三个数据集的共性和区别（概括说就好），说了之后，你再分数据集单独说，读者读起来就顺，知道下面三个数据集是在对上面共性和差异性的展开。如果不说，下面三个数据集就像三块砖头摆在那里，没有语言把它们拎起来。12, 14, 15, 17, 23, and 24. Their definition can be seen in Table \ref{tab:AUs definition}\ref{tab:AUs definition}). In total, about 140,000 frames were annotated frame-by-frame by a group of FACS experts. Following the same subject division \cite{li2018eac,shao2021jaa} \cite{li2018eac,shao2021jaa}, we performed three-fold, subject-exclusive, cross-validations for all experiments.%（哪12个，列出来，AU1, AU2,...AU12。可以提供一张图把三个数据集涉及到的所有AU的样例图都集中画出来，让读者看起来舒服，能快速明白AU对应是哪一个）.%（哪12个，列出来，AU1, AU2,...AU12。可以提供一张图把三个数据集涉及到的所有AU的样例图都集中画出来，让读者看起来舒服，能快速明白AU对应是哪一个）.%%%%%%%BP4D%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%BP4D%%%%%%%%%%%%%%%%%%%%%%%\begin{table*}\begin{table*} %\small%\small\centering\centering  \caption{ \caption{Comparisons of our method and the state-of-the-art methods on BP4D in terms of F1 scores(\\%). The best results are shown in bold, and the second best results are in brackets.}}   \vspace{-1em}%   \vspace{-1em}%   \vspace{-1em}  \label{tab:F1 on Bp4D} \label{tab:F1 on Bp4D}  %\setlength{\tabcolsep}{1.5mm}{ %\setlength{\tabcolsep}{1.5mm}{  \begin{tabular} \begin{tabular}{l|cccccccccccc|c}      \hline     \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4}&\textbf{AU6}&\textbf{AU7}&\textbf{AU10}&\textbf{AU12}&\textbf{AU14}&\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\\\[1pt]      \hline \hline       LSVM      &23.2 &22.8 &23.1 &27.2 &47.1 &77.2 &63.7 &64.3 &18.4 &33.0 &19.4 &20.7 &35.3 \\\\      JPML      &32.6 &25.6 &37.4 &42.3 &50.5 &72.2 &74.1 & 65.7 &38.1 &40.0 &30.4 &42.3 &45.9\\\\      DRML      &36.4 &41.8 &43.0 &55.0 &67.0 &66.3 &65.8 &54.1 &33.2 &48.0 &31.7 &30.0 &48.3\\\\      EAC-Net &39.0 &35.2 &48.6 &76.1 &72.9 &81.9 &86.2 &58.8 &37.5 &59.1 &35.9 &35.8 &55.9\\\\    % ROI     &36.2 &31.6 &43.4 &77.1 &73.7 &85.0 &87.0 &62.6 &45.7 &58.0 &38.3 &37.4 &56.4\\  % ROI     &36.2 &31.6 &43.4 &77.1 &73.7 &85.0 &87.0 &62.6 &45.7 &58.0 &38.3 &37.4 &56.4\\    %JAA-Net &47.2 &44.0 &54.9 &7 7.5 &74.6 &84.0 &86.9 &61.9 &43.6 &60.3 &42.7 &41.9 &60.0\\  %JAA-Net &47.2 &44.0 &54.9 &7 7.5 &74.6 &84.0 &86.9 &61.9 &43.6 &60.3 &42.7 &41.9 &60.0\\      DSIN      &51.7 &40.4 &56.0 &76.1 &73.5 &79.9 &85.4 &62.7 &37.3 &62.9 &38.8 &41.6 &58.9\\\\      ARL       &45.8 &39.8 &55.1 &75.7 &77.2 &82.3 &86.6 &58.8 &47.6 &62.1 &47.4 &55.4 &61.1\\\\      LP-Net   &43.4 &38.0 &54.2 &77.1 &76.7 &83.8 &87.2 &63.3 &45.3 &60.5 &48.1 &54.2 &61.0\\\\      AU-GCN &46.8 &38.5 &60.1 &[80.1] &79.5 &84.8 &88.0 &67.3 &52.0 &63.2 &40.9 &52.8 &62.8 \\\\      SRERL    &46.9 &45.3 &55.6 &77.1 &78.4 &83.5 &87.6 &63.9 &52.2 &63.9 &47.1 &53.3 &62.9\\\\      AU-RCNN &50.2 &43.7 &57 &78.5 &78.5 &82.6 &87 &67.7 &49.1 &62.4 &50.4 &49.3 &63.0 \\\\      UGN-B    &54.2 &46.4 &56.8 &76.2 &76.7 &82.4 &86.1 &64.7 &51.2 &63.1 &48.5 &53.6 &63.3\\\\      J{\^A}A-Net &53.8 &47.8 &58.2 &78.5 &75.8 &82.7 &88.2 &63.7 &43.3 &61.8 &45.6 &49.9 &62.4\\\\      SEV-Net &\textbf{58.2} &\textbf{50.4} &58.3 &\textbf{81.9} &73.9 &\textbf{87.8} &87.5 &61.6 &[52.6] &62.2 &44.6 &47.6 &63.9\\\\      HMP-PS &53.1 &46.1 &56.0 &76.5 &76.9 &82.1 &86.4 &64.8 &51.5 &63.0 &[49.9] &54.5 &63.4\\\\      MHSA-FFN &51.7 &[49.3] &[61.0] &77.8 &\textbf{79.5} &82.9 &86.3 & \textbf{67.6} &51.9 &63.0 &43.7 &[56.3] &64.2\\\\      CISNet &54.8 &48.3 &57.2 &76.2 &76.5 &85.2 &87.2 &66.2 &50.9 &[65.0] &47.7 &\textbf{56.5} &64.3\\\\      D-PAttNe$t^{tt}$ &50.7 &42.5 &59.0 &79.4 &79.0 &85.0 &[89.3] &67.6 &51.6 &\textbf{65.3} &49.6 &54.5 &64.7\\\\      CaFNet &[55.1] &49.3 &57.7 &78.3 &78.6 &[85.1] &86.2 &[67.4] &52.0 &64.4 &48.3 &56.2 &[64.9]\\\\      \hline      \textbf{GLEE-Net(Ours)}   &\textbf{58.2} &48.7 &\textbf{61.5} &78.7 &[79.2] &84.2 &\textbf{89.8} &66.3 &\textbf{56.7} &64.8 &\textbf{53.5} &53.6 &\textbf{66.3}\\\\    %Ours  &[57.8] &45.3 &\textbf{61.1} &[80.0] &[78.6] &[85.6] &[87.9] &\textbf{68.2} &[52.3] &[63.8] &[49.0] &\textbf{56.8} &\textbf{65.5}\\  %Ours  &[57.8] &45.3 &\textbf{61.1} &[80.0] &[78.6] &[85.6] &[87.9] &\textbf{68.2} &[52.3] &[63.8] &[49.0] &\textbf{56.8} &\textbf{65.5}\\      \hline  \end{tabular} \end{tabular}}  %} %}\end{table*}\end{table*}\textbf{DISFA} contains 27 video clips from 27 participants(12 females and 15 males). Each video records the facial activity of a participant when watching a 4-minutes video clip. Each clip consists of 4,845 frames evenly. Altogether, around 130,000 frames were annotated with intensities from 0 to 5. Following previous works \cite{jacob2021facial}\cite{li2018eac}\cite{shao2021jaa}\cite{yang2021exploiting} \cite{jacob2021facial}\cite{li2018eac}\cite{shao2021jaa}\cite{yang2021exploiting}, we regard intensity labels $\{0,1\}$ as absence and others as presence. The evaluation was performed on 8 AUs(1, 2, 4, 6, 9, 12, 25, and 26. Their definition can be seen in Table \ref{tab:AUs definition}).  . We also performed the same three-fold, subject-exclusive, cross validations on 8 AUs as in the previous works \cite{li2018eac}\cite{shao2021jaa}.% following the subject division of \cite{li2018eac, shao2021jaa} \cite{li2018eac}\cite{shao2021jaa}.% following the subject division of \cite{li2018eac, shao2021jaa}.\textbf{BP4D+} contains 1400 video clips from 140 participants(82 females and 58 males). Compared to BP4D, it has larger identity variations and video numbers. About 198,000 frames were annotated with the same 12 AUs in BP4D. We performed three-fold, subject-exclusive, cross-validations to compare our method with the state-of-the-art. Besides, to evaluate the generalization performance, our method was trained on BP4D and then evaluated on BP4D+, following the previous works \cite{attnetionTrans2019}\cite{shao2021jaa} \cite{attnetionTrans2019}\cite{shao2021jaa}.%以上是列举了三个数据，接下来可以做一个数据集的总结，比如说从数据量来说，xxx最少，xxx居中，最多是xxxx。也包括AU的个数也可以提一下，这里重在讲三个数据集的区别。这样方便后面实验讨论，比如我们工作可能在数据量大的数据集上表现好，等等，分析讨论结果的时候可以到这里来找理由，找依据。%以上是列举了三个数据，接下来可以做一个数据集的总结，比如说从数据量来说，xxx最少，xxx居中，最多是xxxx。也包括AU的个数也可以提一下，这里重在讲三个数据集的区别。这样方便后面实验讨论，比如我们工作可能在数据量大的数据集上表现好，等等，分析讨论结果的时候可以到这里来找理由，找依据。% \begin{table}[!t]% \begin{table}[!t]% %\small% %\small% \footnotesize% \footnotesize% %\setlength{\tabcolsep}{6.5pt} % %\setlength{\tabcolsep}{6.5pt} % \renewcommand\arraystretch{1.5} % \renewcommand\arraystretch{1.5} % \centering% \centering% {% {%   \caption{Ablation study of different global feature encoder pretrained on different dataset and task. Measured on BP4D by F1 scores(\%). InpResNetv1 is the abbreviation of InceptionResNetv1 }%   \caption{Ablation study of different global feature encoder pretrained on different dataset and task. Measured on BP4D by F1 scores(\%). InpResNetv1 is the abbreviation of InceptionResNetv1 }%   \vspace{-1em}%   \vspace{-1em}%   \label{tab:F1 on pretrain}%   \label{tab:F1 on pretrain}%  \begin{tabular}{l|cccccccc|c}%  \begin{tabular}{l|cccccccc|c}%     \hline%     \hline%   %\textbf{Arch.} &\textbf{ResNet50} &\textbf{InceptionResNetv1} &\textbf{InceptionResNetv1}\\[1pt]%   %\textbf{Arch.} &\textbf{ResNet50} &\textbf{InceptionResNetv1} &\textbf{InceptionResNetv1}\\[1pt]%     \textbf{Arch.} &ResNet50 &InpResNetv1 &InpResNetv1\\[1pt]%     \textbf{Arch.} &ResNet50 &InpResNetv1 &InpResNetv1\\[1pt]%     \hline\hline%     \hline\hline%     \textbf{Data.} &ImageNet &ImageNet &FEC\\[1pt]%     \textbf{Data.} &ImageNet &ImageNet &FEC\\[1pt]%     \textbf{Task.} &Classification &Classification &Expression similarity \\[1pt]%     \textbf{Task.} &Classification &Classification &Expression similarity \\[1pt]%     \hline%     \hline%     \textbf{F1-Score} &64.4 &63.5 & 66.3\\%     \textbf{F1-Score} &64.4 &63.5 & 66.3\\%     \hline%     \hline%   \end{tabular}}%   \end{tabular}}% \end{table}% \end{table}%%%%%%%DISFA%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%DISFA%%%%%%%%%%%%%%%%%%%%%%%\begin{table}[t]\begin{table}[t]\centering\centering   \caption{Comparisons of our method and the state-of-the-art methods on DISFA in terms of F1 scores(\\%). %   The best results are shown in bold, and the second best are in brackets.%   The best results are shown in bold, and the second best are in brackets.   }   \vspace{-1em}  %\vspace{-1em} %\vspace{-1em}  \label{tab:F1 on DISFA} \label{tab:F1 on DISFA} % \setlength{\tabcolsep}{1.9mm}{% \setlength{\tabcolsep}{1.9mm}{  \begin{tabular} \begin{tabular}{l|cccccccc|c}    \hline  \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU9} &\textbf{AU12} &\textbf{AU25} &\textbf{AU26} &\textbf{Avg.}\\\\[1pt]      \hline\hline      LSVM          &10.8 &10.0 &21.8 &15.7 &11.5 &70.4 &12.0 &22.1 &21.8\\\\      DRML          &17.3 &17.7 &37.4 &29.0 &10.7 &37.7 &38.5 &20.1 &26.7\\\\      APL            &11.4 &12.0 &30.1 &12.4 &10.1 &65.9 &21.4 &26.9 &23.8\\\\      EAC-Net            &41.5 &26.4 &66.4 &50.7 &8.5 &\textbf{89.3} &88.9 &15.6 &48.5\\\\    %JAA-Net    &43.7 &46.2 &56.0 &41.4 &44.7 &69.6 &88.3 &58.4 &56.0\\  %JAA-Net    &43.7 &46.2 &56.0 &41.4 &44.7 &69.6 &88.3 &58.4 &56.0\\      DSIN          &42.4 &39.0 &68.4 &28.6 &46.8 &70.8 &90.4 &42.2 &53.6\\\\      ARL            &43.9 &42.1 &63.6 &41.8 &40.0 &76.2 &[95.2] &66.8 &58.7\\\\      LP-Net       &29.9 &24.7 &72.7 &46.8 &49.6 &72.9 &93.8 &56.0 &56.9\\\\      AU-GCN         &32.3 &19.5 &55.7 &57.9 &61.4 &62.7 &90.9 &60.0 &55.0\\\\      AU-RCNN   &32.1 &25.9 &59.8 &55.4 &39.8 &67.7 &77.4 &52.6 &51.3 \\\\      SRERL         &45.7 &47.8 &56.9 &47.1 &45.6 &73.5 &84.3 &43.6 &55.9\\\\      UGN-B         &43.3 &48.1 &63.4 &49.5 &48.2 &72.9 &90.8 &59.0 &60.0\\\\      J{\^A}A-Net      &[62.4] &[60.7] &67.1 &41.1 &45.1 &73.5 &90.9 &[67.4] &63.5\\\\      MHSA-FFN    &46.1 &48.6 &72.8 &\textbf{56.7} &50.0 &72.1 &90.8 &55.4 &61.5\\\\      SEV-Net      &55.3 &53.1 &61.5 &[53.6] &38.2 &71.6 &\textbf{95.7} &41.5 &58.8\\\\      HMP-PS       &38.0 &45.9 &65.2 &50.9 &50.8 &76.0 &93.3 &\textbf{67.6} &61.0\\\\      CISNet       &48.8 &50.4 &[78.9] &51.9 &47.1 &[80.1] &[95.4] &65.0 &64.7\\\\      CaFNet       &45.6 &55.7 &\textbf{80.2} &51.0 &\textbf{54.7} &79.0 &95.2 &65.3 &[65.8]\\\\      \hline      \textbf{GLEE-Net(Ours)}      &\textbf{63.5} &\textbf{62.5} &69.8 &48.6 &[53.9] &75.6 &94.7 &64.4 &\textbf{66.6}\\\\      \hline  \end{tabular}}% \end{tabular}}%}\end{table}\end{table}%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%\begin{table*}[!t]\begin{table*}[!t]\centering\centering   \caption{Comparisons of our method and the state-of-the-art methods on BP4D+ in terms of F1 scores(\\%). %   The best results are shown in bold.%   The best results are shown in bold.   }  \label{tab:F1 on ThreeFoldBp4DPlus} \label{tab:F1 on ThreeFoldBp4DPlus}  %\setlength{\tabcolsep}{1.5mm}{ %\setlength{\tabcolsep}{1.5mm}{  \begin{tabular} \begin{tabular}{l|cccccccccccc|c}      \hline    \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\\\[1pt]      \hline \hline      FACS3D-Net       &43.0 &38.1 &\textbf{49.9} &82.3 &85.1 &87.2 &87.5 &66.0 &48.4 &[47.4] &50.0 &[31.9] &59.7\\\\      ML-GCN &40.2 &36.9 &32.5 &84.8 &[88.9] &89.6 &[89.3] &81.2 &[53.3] &43.1 &55.9 &28.3 &60.3\\\\      MS-CAM &38.3 &37.6 &25.0 &85.0 &\textbf{90.9} &\textbf{90.9} &89.0 &[81.5] &\textbf{60.9} &40.6 &58.2 &28.0 &60.5\\\\      SEV-Net &[47.9] &\textbf{40.8} &31.2 &\textbf{86.9} &87.5 &89.7 &88.9 &\textbf{82.6} &39.9 & \textbf{55.6} &[59.4] &27.1 &[61.5]\\\\      \hline      \textbf{GLEE-Net(Ours)}   &\textbf{51.5} &[46.6] &[43.5] &[86.8] &89.6 &[91.0] &\textbf{89.8} &82.3 &46.8 & 49.3 &\textbf{60.9} &\textbf{50.9} &\textbf{65.7}\\\\      \hline  \end{tabular} \end{tabular}}  %} %}\end{table*}\end{table*}%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%BP4D+%%%%%%%%%%%%%%%%%%%%%%%\begin{table*}[!t]\begin{table*}[!t]\centering\centering   \caption{Comparisons of our method and the state-of-the-art on cross-dataset evaluation(trained on BP4D and evaluated on BP4D+) in terms of F1 scores(\\%). %   The best results are shown in bold.%   The best results are shown in bold.   }  \label{tab:F1 on Bp4DPlus} \label{tab:F1 on Bp4DPlus}  %\setlength{\tabcolsep}{1.5mm}{ %\setlength{\tabcolsep}{1.5mm}{  \begin{tabular} \begin{tabular}{l|cccccccccccc|c}      \hline    \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\\\[1pt]      \hline \hline      EAC-Net       &38.0 &[37.5] &[32.6] &82.0 &83.4 &87.1 &85.1 &62.1 &44.5 &43.6 &45.0 &32.8 &56.1\\\\      ARL             &29.9 &33.1 &27.1 &81.5 &83.0 &84.8 &86.2 &59.7 &[44.6] &43.7 &48.8 &32.3 &54.6\\\\      J{\^A}A-Net &\textbf{39.7} &35.6 &30.7 &[82.4] &[84.7] &[88.8] &[87.0] &[62.2] &38.9 &[46.4] &[48.9] &\textbf{36.6} &56.8\\\\      \hline      \textbf{GLEE-Net(Ours)}   &[39.5] &\textbf{37.7} &\textbf{44.0} &\textbf{84.5} &\textbf{84.9} &\textbf{89.6} &\textbf{87.7} &\textbf{72.3} &\textbf{44.9} & [45.3] &\textbf{52.6} &[33.9] &\textbf{59.7}\\\\      \hline  \end{tabular} \end{tabular}}  %} %}\end{table*}\end{table*}\subsection{\subsection{Implementation Details}}To enhance the feature extraction capability of low-level convolution layers, the feature encoder was initialized with the corresponding network parameters pretrained on the dataset of ImageNet or FEC, and the rest of our networks were set to Kaiming initialization \cite{he2015delving} \cite{he2015delving}. Except for the Mask Decoder, the whole model parameters were updated by employing an Adam optimizer with hyper-parameters $\beta = 0.9$ and weight decay $10^{-6}$.%可能要斟酌一下要不要写MaskDecoder部分参数冻结，要写的话如何说清和证明它的作用%可能要斟酌一下要不要写MaskDecoder部分参数冻结，要写的话如何说清和证明它的作用%这里就可以给一张训练集和验证集，随着时间，收敛的情况，可以分AU来说，我们也可以观察下，哪些AU收敛快，哪些慢，哪些容易过拟合，哪些比较好泛化，等等，这个图都是可以用来分析后面的实验结果，避免实验结果太干涩，没话说。%这里就可以给一张训练集和验证集，随着时间，收敛的情况，可以分AU来说，我们也可以观察下，哪些AU收敛快，哪些慢，哪些容易过拟合，哪些比较好泛化，等等，这个图都是可以用来分析后面的实验结果，避免实验结果太干涩，没话说。\subsection{\subsection{Comparisons with the State-of-the-Art}}We compared our method with many state-of-the-art AU detection methods, including LSVM \cite{LSVM}, JPML \cite{JPML}, DRML \cite{DRML}, APL \cite{LP48}, EAC-Net \cite{li2018eac}, DSIN \cite{LP8}, ARL \cite{attnetionTrans2019}, SRERL \cite{SRERL}, AU-GCN\cite{liu2020relation},AU-RCNN\cite{ma2019r}, ML-GCN \cite{chen2019multi}, MS-CAM \cite{you2020cross}, LP-Net \cite{LP}, FACS3D-Net \cite{yang2019facs3d}, UGN-B \cite{song2021uncertain}, J{\^A}A-Net \cite{shao2021jaa}, MHSA-FFN \cite{jacob2021facial}, SEV-Net \cite{yang2021exploiting}, HMP-PS \cite{song2021hybrid}, D-PAttNe$t^{tt}$\cite{Onal2019D-PAttNet}, CISNet\cite{chen2022causal} and CaFNet\cite{chen2021cafgraph}. %\textcolor{red}{[Reviewers may question why not evaluate all the methods on all the three datasets? Any particular reasons doing so? If so, it would be better to explain the reasons here.]} %这里就可以说下，哪些方法是在三个数据集上测试，哪些仅仅是两个数据，这些都是为后面分数据集汇报结果准备，避免人家说，为什么不同数据集，baseline方法却不一样。%\textcolor{red}{[Reviewers may question why not evaluate all the methods on all the three datasets? Any particular reasons doing so? If so, it would be better to explain the reasons here.]} %这里就可以说下，哪些方法是在三个数据集上测试，哪些仅仅是两个数据，这些都是为后面分数据集汇报结果准备，避免人家说，为什么不同数据集，baseline方法却不一样。Following the experimental settings of most previous works, we also employed the F1 score \cite{F1} \cite{F1} on the frame level as the evaluation metric. F1-score is a harmonic mean of precision(P) and recall(R), which is defined as $F1 = 2PR/(P+R)$. Since F1-score takes both false positives and false negatives into account, it reflects a more rational measurement of the model's performance than accuracy, especially on datasets with uneven class distributions like BP4D, DISFA, and BP4D+.The results on BP4D are shown in Table \ref{tab:F1 on Bp4D}\ref{tab:F1 on Bp4D}. The average F1 score of our method is 66.3\\%, which significantly outperforms all the other comparison methods, improving about 1.4\\% over the second highest one, CaFNet. In terms of the performances on single AUs, our method achieves the highest F1 scores among all the methods on 5 AUs(i.e., AU1, AU4, AU12, AU15, and AU23) and second highest on 1 AUs(AU7) of the 12 evaluated AUs. Besides, our method shows over 3.5\\% superiority on AU15 and AU23 over the second highest ones. In terms of AU feature learning, our method outperforms JMPL, DRML, and D-PAttNe$t^{tt}$ about 20.4\\%, 18\\% and 1.6\\%, demonstrating that extracting local features by attention is more effective and our method is superior in AU feature extraction than patch learning. Compared with EAC-Net, JAA-Net, and MHSA-FFN, which utilize attention mechanisms with the supervisions of pre-defined AU centers, our method achieves improvements of 10.4\\%, 5.2\\% and 3.9\\% over them(EAC-Net, JAA-Net, and MHSA-FFN), respectively. This validates the superiority of our non-predetermined AU attention learning approach.  %\textcolor{red}{I think we can improve the structure of the above text.} %\textcolor{red}{I think we can improve the structure of the above text.}%\textcolor{red}{Compared to SEV-Net and J{\^A}A-Net that employ textual embedding and facial landmarks as auxiliary training information, our method obtains better results with the compact expression embedding as prior knowledge. WHAT DO WE WANT TO EXPRESS}%\textcolor{red}{Compared to SEV-Net and J{\^A}A-Net that employ textual embedding and facial landmarks as auxiliary training information, our method obtains better results with the compact expression embedding as prior knowledge. WHAT DO WE WANT TO EXPRESS}Table \ref{tab:F1 on DISFA}\ref{tab:F1 on DISFA} shows the evaluation results on DISFA. As shown in this table, our method achieves the average F1 score of 66.6\\%, outperforming all the compared state-of-the-art methods. Compared to the most recent works SEV-Net, HMP-PS, MHSA-FFN, CISNet and CaFNet, our method achieves an improvement of 7.8\\%, 5.6\\%, 5.1\\%, \1.9\% and 0.8\\% over them, respectively. Unlike EAC-Net and J{\^A}A-Net which are supervised by both AU and landmark labels, our method only utilizes AU labels, but still obtains significant improvements of 18.1\\% and 3.1\\% over EAC-Net and J{\^A}A-Net, respectively, demonstrating the effectiveness of our method in AU feature and attention learning. Note that our method does not explicitly model AU relationships, but significantly exceeds all relation-based methods including JMPL, DSIN, ARL, AU-GCN, and AU-RCNN.%As the number of subjects in DISFA is smaller than that of BP4D, \textcolor{red}{most of the previous methods suffer from overfitting to the appearance of training subjects more severely. WHY?} Therefore, benefiting from our identity-independent expression representations, our method achieves an even more significant improvement.%As the number of subjects in DISFA is smaller than that of BP4D, \textcolor{red}{most of the previous methods suffer from overfitting to the appearance of training subjects more severely. WHY?} Therefore, benefiting from our identity-independent expression representations, our method achieves an even more significant improvement.Table \ref{tab:F1 on ThreeFoldBp4DPlus}\ref{tab:F1 on ThreeFoldBp4DPlus} shows the evaluation results of the three-fold cross-validation on BP4D+.In particular, the results of SEV-Net, ML-DCN and MS-CAM are reported in\cite{yang2021exploiting}\cite{yang2021exploiting} while the results of EAC-Net are reported in \cite{shao2021jaa} \cite{shao2021jaa}. Our method achieves the F1 score of 65.7\\% and outperforms all the state-of-the-art methods, exceeding SEV-Net over 4.2\\%.%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%pose_mask figure% %%%%%%%%%%%%%pose_mask figure% \begin{figure*}[!t]% \begin{figure*}[!t]%     \centering%     \centering%     \includegraphics[ width=18cm]{images/sample4.pdf}%     \includegraphics[ width=18cm]{images/sample4.pdf}%     %\vspace{-0.5em}%     %\vspace{-0.5em}%     \caption{Illustration of attention map on different head pose. The Mask Decoder generates  similar masks with various pose images input, demonstrates that the mask decoder is robust to head pose}%     \caption{Illustration of attention map on different head pose. The Mask Decoder generates  similar masks with various pose images input, demonstrates that the mask decoder is robust to head pose}%     \label{fig:pose_mask}%     \label{fig:pose_mask}% \end{figure*}% \end{figure*}% %%%%%%%%%%%%%% %%%%%%%%%%%%%To further evaluate the generalization performance of our method on large-scale test identities, we trained our method on BP4D and evaluated it on the full BP4D+ of 140 subjects. The results are shown in Table \ref{tab:F1 on Bp4DPlus}\ref{tab:F1 on Bp4DPlus}. We use the reported results in the work \cite{shao2021jaa} \cite{shao2021jaa} for comparison. Again, our method outperforms all the compared methods under the large-scale cross-dataset evaluation. It indicates that our method can extract identity-independent information and generalize well to new identities.%\textcolor{red}{[if possible, I suggest to move the tables/figures to the same page as the first cited place/page. Or if it cannot be achieved, the place of tables/figures should be as close as possible to the first cited place/page. This would increase the readability.]}%\textcolor{red}{[if possible, I suggest to move the tables/figures to the same page as the first cited place/page. Or if it cannot be achieved, the place of tables/figures should be as close as possible to the first cited place/page. This would increase the readability.]}%From the evaluation results on the three datasets, we can see that AU7, AU12 and AU17 rechieve best performances on BP4D, and AU1 and AU2 gets best results on DISFA. %From the evaluation results on the three datasets, we can see that AU7, AU12 and AU17 rechieve best performances on BP4D, and AU1 and AU2 gets best results on DISFA. %综合看三个数据集的结果，可以谈谈哪些AU，我们的方法总是获胜，哪些总是不好，然后可以分析原因。%综合看三个数据集的结果，可以谈谈哪些AU，我们的方法总是获胜，哪些总是不好，然后可以分析原因。\subsection{\subsection{Ablation Study}}%先简要回顾下我们的算法框架，其实有挑选的介绍，然后再说我们要逐一验证这些框架子模块的设计，才进行了ablation study。（提高文章的过度和可读性）%先简要回顾下我们的算法框架，其实有挑选的介绍，然后再说我们要逐一验证这些框架子模块的设计，才进行了ablation study。（提高文章的过度和可读性）%As described in Section \ref{sec:methodology}, our framework includes the global feature encoder followed by two branches of feature decoders, namely, facial feature decoder($D_f$) and facial mask decoder($D_m$). While the $D_f$ module creates one initial feature map for each AU, the $D_m$ module is responsible for learning feature masks that filter out the areas irrelevant to current AU. Then, by a point-wise multiplication of the initial feature map $xx$ and the feature mask from $D_f$ and $D_m$, we obtain the feature map  $xx$ of AU-related local regions for each AU. $we have to clearly indicate what we will validate by our ablation studies.$%As described in Section \ref{sec:methodology}, our framework includes the global feature encoder followed by two branches of feature decoders, namely, facial feature decoder($D_f$) and facial mask decoder($D_m$). While the $D_f$ module creates one initial feature map for each AU, the $D_m$ module is responsible for learning feature masks that filter out the areas irrelevant to current AU. Then, by a point-wise multiplication of the initial feature map $xx$ and the feature mask from $D_f$ and $D_m$, we obtain the feature map  $xx$ of AU-related local regions for each AU. $we have to clearly indicate what we will validate by our ablation studies.$In this section, we conduct ablation studies to evaluate the effectiveness of each key sub-module in our framework, including: 1) the prior knowledge of expression similarity learning, 2) the facial components module, 3) and mask activation. In particular, all the ablation experiments are conducted on the BP4D dataset due to space limitations. The experimental results are reported in Table~\ref{tab:F1 on Ablation 2}\ref{tab:F1 on Ablation 2}. %As shown in Table~\ref{tab:F1 on Ablation}, we firstly construct a baseline model(Baseline), of which the feature extractor is based on InceptionResNetv1 without pretrained parameters, followed by AU classifiers. Besides, to verify the validity of the pretrained expression featrue encoder, we load parameters pretrained on ImageNet(Baseline-ImageNet) and on FEC(Baseline-FEC) respectively. For further validation of our facial feature decoder($D_f$) and facial mask decoder($D_m$), we gradually add $D_f$(Baseline-FEC-DF ) and $D_m$(Baseline-FEC-DF-DM) .  %As shown in Table~\ref{tab:F1 on Ablation}, we firstly construct a baseline model(Baseline), of which the feature extractor is based on InceptionResNetv1 without pretrained parameters, followed by AU classifiers. Besides, to verify the validity of the pretrained expression featrue encoder, we load parameters pretrained on ImageNet(Baseline-ImageNet) and on FEC(Baseline-FEC) respectively. For further validation of our facial feature decoder($D_f$) and facial mask decoder($D_m$), we gradually add $D_f$(Baseline-FEC-DF ) and $D_m$(Baseline-FEC-DF-DM) .  %Furthermore, as shown in Table \ref{tab:F1 on Ablation 2}, to explore the effectiveness of each implementation, we replace or remove certain individual modules of the full framework and test the model performance. For instance, freezing the pretrained Feature Encoder weights(w.fixed FE), replacing the activation function of mask decoder with softmax(w. Softmax), etc. The experiments results will be analysed in detail in the following paragraphs.   %既然这里提到了表格4，这里就定义出表格4中各种消融方法的定义%Furthermore, as shown in Table \ref{tab:F1 on Ablation 2}, to explore the effectiveness of each implementation, we replace or remove certain individual modules of the full framework and test the model performance. For instance, freezing the pretrained Feature Encoder weights(w.fixed FE), replacing the activation function of mask decoder with softmax(w. Softmax), etc. The experiments results will be analysed in detail in the following paragraphs.   %既然这里提到了表格4，这里就定义出表格4中各种消融方法的定义%anrudong: 表格中涉及到的各个消融实验方法的定义下文有分模块详细介绍，如果在这里再写一遍显得有些重复,因此删掉%anrudong: 表格中涉及到的各个消融实验方法的定义下文有分模块详细介绍，如果在这里再写一遍显得有些重复,因此删掉% \begin{table*}[!t]% \begin{table*}[!t]% %\small% %\small% \footnotesize% \footnotesize% \setlength{\tabcolsep}{8pt}% \setlength{\tabcolsep}{8pt}% \renewcommand\arraystretch{1.5} % \renewcommand\arraystretch{1.5} % \centering% \centering% {% {%   \caption{Ablation study on BP4D measured by F1 scores(\%).}%   \caption{Ablation study on BP4D measured by F1 scores(\%).}%   \vspace{-1em}%   \vspace{-1em}%   \label{tab:F1 on Ablation}%   \label{tab:F1 on Ablation}%  \begin{tabular}{l|cccccccccccc|c}%  \begin{tabular}{l|cccccccccccc|c}%     \hline%     \hline%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{F1-Score} \\[1pt]%   \textbf{Method} &\textbf{Param-ImageNet} &\textbf{Param-FEC} &\textbf{Facial Decoder} &\textbf{Mask Decoder} &\textbf{F1-Score} \\[1pt]%     \hline\hline%     \hline\hline%     % Baseline        &- &-  &- &- &52.6\\%     % Baseline        &- &-  &- &- &52.6\\%     % Baseline-ImageNet         &$\surd$ &- &- &- &61.6 \\%     % Baseline-ImageNet         &$\surd$ &- &- &- &61.6 \\%     Baseline-FEC         &- &$\surd$ &- &- &63.3 \\%     Baseline-FEC         &- &$\surd$ &- &- &63.3 \\%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &- &63.8 \\%     Baseline-FEC-DF          &- &$\surd$ &$\surd$ &- &63.8 \\%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &- &63.7 \\%     Baseline-FEC-CNN        &- &$\surd$ &$\surd$ &- &63.7 \\%     Baseline-FEC-DF-DM/GLEE-Net(Full)       &- &$\surd$ &$\surd$ &$\surd$ &66.3 \\%     Baseline-FEC-DF-DM/GLEE-Net(Full)       &- &$\surd$ &$\surd$ &$\surd$ &66.3 \\%     % Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\%     % Baseline-FEC-DF-DM-PE    &- &$\surd$ &$\surd$ &$\surd$ &$\surd$ &$\surd$ &64.2 \\%     \hline%     \hline%   \end{tabular}}%   \end{tabular}}% \end{table*}% \end{table*}\begin{table*}[!t]\begin{table*}[!t]%\small%\small\centering\centering  \caption{ \caption{Ablation study on BP4D measured by F1 scores(\\%). }}   \vspace{-1em}  \label{tab:F1 on Ablation 2} \label{tab:F1 on Ablation 2} \begin{tabular}\begin{tabular}{l|cccccccccccc|c}      \hline    \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4} &\textbf{AU6} &\textbf{AU7} &\textbf{AU10} &\textbf{AU12} &\textbf{AU14} &\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\\\[1pt]      \hline\hline      w/o pretrain &34.9 &24.2 &36.7 &76.1 &71.4 &81.0 &86.3 &58.7 &25.9 &51.9 &27.4 &31.6 &50.5\\\\      w. FE Emotion &48.1 &41.6 &53.9 &78.6 &77.9 &83.2 &88.8 &60.5 &39.3 &65.5 &38.0 &47.6 &60.3 \\\\      w. FE ImageNet &49.6 &39.7 &60.5 &77.3 &78.7 &83.1 &88.6 &[64.6] &48.2 &63.2 &47.5 &48.0 &62.4 \\\\      w. FE fixed &52.3 &45.8 &59.8 &[79.4] &78.1 &\textbf{84.8} &89.0 &64.0 &46.5 &64.0 &38.6 &49.8 &63.5\\\\    % w. ResNet &[56.9] &46.5 &57.2 &78.1 &[79.2] &84.2 &87.9 &63.8 &51.0 &64.7 &49.5 &[53.5] &[64.4]\\  % w. ResNet &[56.9] &46.5 &57.2 &78.1 &[79.2] &84.2 &87.9 &63.8 &51.0 &64.7 &49.5 &[53.5] &[64.4]\\      \hline      w/o DM\\&DF &[55.4] &\textbf{65.1} &\textbf{73.9} &49.0 &46.9 &77.1 &\textbf{92.9} &54.1 &48.1 &64.7 &[52.5] &47.5 &63.3\\\\      w/o DM   &53.3 &44.2 &58.7 &78.6 &76.9 &83.9 &[89.8] &62.2 &48.9 &65.1 &[52.5] &51.8 &63.8\\\\      w/o DM\\& w. CNN &51.8 &43.0 &59.1 &79.3 &78.1 &84.4 &89.0 &63.1 &50.5 &64.3 &49.2 &\textbf{55.1} &63.9\\\\   % w. PE & 54.8 &45.3 &[63.4] &78.4 &79.1 &[84.6] &89.1 &60.7 &49.7 &64.2 &50.7 &50.3 & 64.2\\ % w. PE & 54.8 &45.3 &[63.4] &78.4 &79.1 &[84.6] &89.1 &60.7 &49.7 &64.2 &50.7 &50.3 & 64.2\\            \hline    % w. None & 53.7 &44.6 &55.4 &78.6 &78.4 &83.7 &89.2 &[64.6] &[51.4] &\textbf{65.9} &51.2 &52.6 &64.1\\  % w. None & 53.7 &44.6 &55.4 &78.6 &78.4 &83.7 &89.2 &[64.6] &[51.4] &\textbf{65.9} &51.2 &52.6 &64.1\\      w. SoftMax & 53.6 &43.8 &58.5 &\textbf{79.7} &[79.2] &84.5 &89.6 &63.4 &50.3 &62.7 &50.8 &53.0 &64.0\\\\    % w. Tanh &55.1 &46.2 &60.2 &79.1 &\textbf{79.3} &[84.6] &88.d6 &63.0 &49.6 &[65.3] &51.8 &50.2 &[64.4]\\   % w. Tanh &55.1 &46.2 &60.2 &79.1 &\textbf{79.3} &[84.6] &88.d6 &63.0 &49.6 &[65.3] &51.8 &50.2 &[64.4]\\          \hline      \textbf{GLEE-Net(Full)} &\textbf{58.2} &[48.7] &[61.5] &78.7 &[79.2] &84.2 &[89.8] &\textbf{66.3} &\textbf{56.7} &64.8 &\textbf{53.5} &[53.6] &\textbf{66.3}\\\\    %GLEE-Net(Full) & 53.7 &[48.4] & 59.8 & \textbf{79.7} & 78.9 &83.5 & 89.5 &\textbf{64.0} &[50.6] &64.1 &50.2 &[53.4] &\textbf{64.7}\\  %GLEE-Net(Full) & 53.7 &[48.4] & 59.8 & \textbf{79.7} & 78.9 &83.5 & 89.5 &\textbf{64.0} &[50.6] &64.1 &50.2 &[53.4] &\textbf{64.7}\\      \hline  \end{tabular} \end{tabular}}\end{table*}\end{table*}%\textcolor{red}{here we need a head text to briefly introduce what we will presents.}%\textcolor{red}{here we need a head text to briefly introduce what we will presents.}% \textcolor{red}{here we have to make a head paragraph to introduce what we will presents. What will we study? It looks three ablation studiese here.}% \textcolor{red}{here we have to make a head paragraph to introduce what we will presents. What will we study? It looks three ablation studiese here.}\begin{itemize}\begin{itemize}      \item [a) ]      $w/o~pretrain$: $E_f$ is randomly initialized;      \item [b) ]      $w.~FE~Emotion$: $E_f$ is initialized via a pretrained classifier of seven discrete facial expression emotion (e.g. neutral, happy, sad, surprise, fear, disgust, angry) categories trained on the AffectNet dataset;      \item [c) ]       $w.~FE~ImageNet$: $E_f$ is initialized via a pretrained image object classifier built on imageNet \cite{krizhevsky2012imagenet}\cite{krizhevsky2012imagenet};         \item [d) ]       $w.~FE~fixed$: $E_f$ is our proposed method, initialized via the facial expression similarity;       \item [e) ]       $GLEE-Net(Full)$: $E_f$ is parameterized by the facial expression similarity approach but it not updated in the training of $GLEE$-$Net$.\end{itemize}\end{itemize}% 1-{2-4}: prior k is necessary;% 1-{2-4}: prior k is necessary;% 4-2/3: ours is ok;% 4-2/3: ours is ok;% 4-5: finetuning% 4-5: finetuning$w.~FE~Emotion$, $w.~FE~ImageNet$ and $w.~FE~fixed$ achieve improvements of 9.8\\%(from 50.5\\% to 60.3\\%), 11.9\\%(from 50.5\\% to 62.4\\%) and 15.8\\%(from 50.5\\% to 66.3\\%), respectively. This indicates that the prior knowledge is necessary and the pretraining progress can bring significant improvement for AU detection.Secondly, compared with the w. FE Emotion and w. FE ImageNet, the GLEE-Net obtains the best performance(66.3\\%), exceeding the other two pretraining methods about 6\\% and 3.9\\%. This proves the effectiveness and superiority of the prior knowledge captured by our facial expression similarity learning. Lastly, compared with GLEE-Net, w. FE fixed obtains a lower average F1 of 63.5\\%. It indicates that finetuning the feature encoder is beneficial for extracting features which are more adaptive to the following FCM module. Thus finetuning operation is essential and efficient to improve the performance of our framework. % the experiment e) with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE) obtains a lower average F1 of 63.5\% compared with the experiment d)% the experiment e) with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE) obtains a lower average F1 of 63.5\% compared with the experiment d)% Firstly, we design a baseline model, which is constructed with the feature encoder(without pretrained parameters) followed by the AU classifier module.% Firstly, we design a baseline model, which is constructed with the feature encoder(without pretrained parameters) followed by the AU classifier module.% Particularly, the followed AU classifier has a similar structure to the AU classifier of the full network but with a different size due to the input feature size difference. As shown in table~\ref{tab:F1 on Ablation}, we test the baseline without pretrained parameters(Baseline), with parameters pretrained on ImageNet(Baseline-ImageNet) and with parameters pretrained on FEC(Baseline-FEC). The Baseline-FEC and the Baseline-ImageNet achieve  63.3\%  and 61.6\%, respectively.  Compared with the baseline model(52.6\%), they bring over 10.7 and 9\% improvements, which validates the importance of pretraining. Moreover, the Baseline-FEC achieves an improvement of 1.7\% compared with the Baseline-ImageNet, proving the superiority of our pretraining on FEC with expression similarity task.% Particularly, the followed AU classifier has a similar structure to the AU classifier of the full network but with a different size due to the input feature size difference. As shown in table~\ref{tab:F1 on Ablation}, we test the baseline without pretrained parameters(Baseline), with parameters pretrained on ImageNet(Baseline-ImageNet) and with parameters pretrained on FEC(Baseline-FEC). The Baseline-FEC and the Baseline-ImageNet achieve  63.3\%  and 61.6\%, respectively.  Compared with the baseline model(52.6\%), they bring over 10.7 and 9\% improvements, which validates the importance of pretraining. Moreover, the Baseline-FEC achieves an improvement of 1.7\% compared with the Baseline-ImageNet, proving the superiority of our pretraining on FEC with expression similarity task.% Secondly, based on our full framework(GLEE-Net), we load the feature encoder with various pretrained weights. As shown in table~\ref{tab:F1 on Ablation 2}, we first test the full network without any pretrained weights(w/o pretrain), then load the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), AffectNet(w. FE Emotion) and FEC(GLEE-Net) respectively.  Specifically, the whole networks of the above experiments(except for w/o pretrain) are finetuned on BP4D. The results in table~\ref{tab:F1 on Ablation 2} show that when loading the parameters pretrained with the expression similarity task(GLEE-Net), it achieves the best F1-Score(66.3\%), while loading parameters pretrained on AffectNet(w. FE Emotion) and ImageNet(w. FE ImageNet) it declines 3.9\% and 6\%. This further verifies the effectiveness of the prior knowledge of expression similarity learning. % Secondly, based on our full framework(GLEE-Net), we load the feature encoder with various pretrained weights. As shown in table~\ref{tab:F1 on Ablation 2}, we first test the full network without any pretrained weights(w/o pretrain), then load the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), AffectNet(w. FE Emotion) and FEC(GLEE-Net) respectively.  Specifically, the whole networks of the above experiments(except for w/o pretrain) are finetuned on BP4D. The results in table~\ref{tab:F1 on Ablation 2} show that when loading the parameters pretrained with the expression similarity task(GLEE-Net), it achieves the best F1-Score(66.3\%), while loading parameters pretrained on AffectNet(w. FE Emotion) and ImageNet(w. FE ImageNet) it declines 3.9\% and 6\%. This further verifies the effectiveness of the prior knowledge of expression similarity learning. % Thirdly, we also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in Table \ref{tab:F1 on Ablation 2}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. It shows that the finetuning operation is effective to improve the performance of our framework.  % Thirdly, we also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in Table \ref{tab:F1 on Ablation 2}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. It shows that the finetuning operation is effective to improve the performance of our framework.  %gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.%gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.%We first evaluate the effectiveness of pretraining. As illustrated in Table~\ref{tab:F1 on Ablation}, the baseline has the same structure as the feature encoder($E_f$) of our full network but does not load any pretrained parameters(\textit{Baseline}), which is followed by a classifier module \textcolor{red}{what does a classifier module refer to?}. Then we test it with pretrained parameters on ImageNet, namely, \textit{Baseline-ImageNet}. As shown in Table \ref{tab:F1 on Ablation}, the Baseline-ImageNet achieves 61.6\% and brings over 9\% improvement than the baseline(52.6\%), which validates the importance of pretraining.%We first evaluate the effectiveness of pretraining. As illustrated in Table~\ref{tab:F1 on Ablation}, the baseline has the same structure as the feature encoder($E_f$) of our full network but does not load any pretrained parameters(\textit{Baseline}), which is followed by a classifier module \textcolor{red}{what does a classifier module refer to?}. Then we test it with pretrained parameters on ImageNet, namely, \textit{Baseline-ImageNet}. As shown in Table \ref{tab:F1 on Ablation}, the Baseline-ImageNet achieves 61.6\% and brings over 9\% improvement than the baseline(52.6\%), which validates the importance of pretraining.%the baseline is constructed based merely on an InceptionResNetV1 network without pretraining. It has the same structure as the feature encoder of our full network, using the intermediate features which has a resolutioin of 16 x 16. The feature encoder of the baseline is followed by several classifer modules similar to AU Classifer Module. The number of classifier modules is corresponding to the AU classes. Each classifier module predicts a specific AU's probability and shares the same structure that contains 3 CNN layers and a Sigmoid activation at the last layer. Then we test the baseline with pretrained parametes on ImageNet, namely Baseline-ImageNet. As shown in Table \ref{tab:F1 on Ablation}, it achieves 61.6\% and brings over 9\% improvement compared with baseline(52.6\%), proving the importance of pretraining.%the baseline is constructed based merely on an InceptionResNetV1 network without pretraining. It has the same structure as the feature encoder of our full network, using the intermediate features which has a resolutioin of 16 x 16. The feature encoder of the baseline is followed by several classifer modules similar to AU Classifer Module. The number of classifier modules is corresponding to the AU classes. Each classifier module predicts a specific AU's probability and shares the same structure that contains 3 CNN layers and a Sigmoid activation at the last layer. Then we test the baseline with pretrained parametes on ImageNet, namely Baseline-ImageNet. As shown in Table \ref{tab:F1 on Ablation}, it achieves 61.6\% and brings over 9\% improvement compared with baseline(52.6\%), proving the importance of pretraining.% 我感觉直接介绍pretrained feature model 部分即可，无需再介绍后面的classifier啥的结构了。% 我感觉直接介绍pretrained feature model 部分即可，无需再介绍后面的classifier啥的结构了。%To test the efficiency of our feature encoder pretrained on FEC with the facial expression similarity task, we replaced the feature encoder of our full network with different architectures or parameters and then fine-tuned the whole network on BP4D. %To test the efficiency of our feature encoder pretrained on FEC with the facial expression similarity task, we replaced the feature encoder of our full network with different architectures or parameters and then fine-tuned the whole network on BP4D. %As shown in Table \ref{tab:F1 on Ablation 2}, we first load the weights of the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), then load the weights with parameters pretrained on an emotion dataset(AffectNet) by the emotion recognition task(w. FE Emotion). We also take ResNet50 pretrained on ImageNet as the feature encoder of our full network(w. ResNet50). %As shown in Table \ref{tab:F1 on Ablation 2}, we first load the weights of the feature encoder with parameters pretrained on ImageNet(w. FE ImageNet), then load the weights with parameters pretrained on an emotion dataset(AffectNet) by the emotion recognition task(w. FE Emotion). We also take ResNet50 pretrained on ImageNet as the feature encoder of our full network(w. ResNet50). %It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.%It achieves the best result when loading our parameters pretrained with the expression similarity task, gaining improvement over 2.8\%(from 63.5\% to 66.3\%) and 1.9\%(from 64.4\% to 66.3\%) in comparison to InceptionResNetV1 and ResNet50 pretrained on ImageNet, respectively. This validates the efficiency of prior knowledge from the compact expression embedding.%\textcolor{red}{looks no table for the above results. I dont know why the above uses DISFA and teh below uses the other two datsets.}%\textcolor{red}{looks no table for the above results. I dont know why the above uses DISFA and teh below uses the other two datsets.}%To futher indicate the significance of the pretrained facial expression embedding network, we also test it on the BP4D dataset. First, we replace the feature encoder with a ResNet~\cite{Resnet34}~(w. ResNet50 in Table~\ref{tab:F1 on Ablation 2}). The results show that using pretrained facial expression embedding network as backbone improves the score by 3\% on BP4D. %To futher indicate the significance of the pretrained facial expression embedding network, we also test it on the BP4D dataset. First, we replace the feature encoder with a ResNet~\cite{Resnet34}~(w. ResNet50 in Table~\ref{tab:F1 on Ablation 2}). The results show that using pretrained facial expression embedding network as backbone improves the score by 3\% on BP4D. %We also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in the Table \ref{tab:F1 on Ablation}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. This shows that the fine-tuned operation is effective to improve the performance of our framework. %We also set up an experiment with the feature encoder loaded and fixed the parameters pretrained on FEC(w. fixed FE), which obtains a lower average F1 of 63.5, as shown in the Table \ref{tab:F1 on Ablation}. This indicates that there exists a domain gap  between FEC and BP4D datasets because the facial images in FEC are in the wild, having various illuminations, poses, and backgrounds, compared to the BP4D dataset. This shows that the fine-tuned operation is effective to improve the performance of our framework. %\textcolor{red}{Any more discussion here?.}%\textcolor{red}{Any more discussion here?.}\begin{itemize}\begin{itemize}      \item [f) ]      w/o DM\\&DF: removing both the DM and the DF;      \item [g) ]      w/o DM: only removing DM;      \item [h) ]      w/o DM& w. CNN: removing the DM and replacing the DF with a CNN block in the meanwhile. Particularly, the CNN block has similar number of parameters with our feature encoder($E_f$).\end{itemize}\end{itemize}%Specifically, based on the feature encoder pretrained on FEC(Baseline-FEC in Table~\ref{tab:F1 on Ablation} or w/o DM\&DF in Table~\ref{tab:F1 on Ablation 2}), we gradually added the $D_f$ branch(Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation} or w/o DM in Table~\ref{tab:F1 on Ablation 2}) and the $D_m$ branch(Baseline-FEC-DF-DM in Table~\ref{tab:F1 on Ablation} or GLEE-Net in Table~\ref{tab:F1 on Ablation 2}). In addition, we replaced the facial feature decoder of Baseline-FEC-DF with a CNN structure module(Baseline-FEC-CNN) to further validate the effectiveness of the facial feature decoder.%Specifically, based on the feature encoder pretrained on FEC(Baseline-FEC in Table~\ref{tab:F1 on Ablation} or w/o DM\&DF in Table~\ref{tab:F1 on Ablation 2}), we gradually added the $D_f$ branch(Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation} or w/o DM in Table~\ref{tab:F1 on Ablation 2}) and the $D_m$ branch(Baseline-FEC-DF-DM in Table~\ref{tab:F1 on Ablation} or GLEE-Net in Table~\ref{tab:F1 on Ablation 2}). In addition, we replaced the facial feature decoder of Baseline-FEC-DF with a CNN structure module(Baseline-FEC-CNN) to further validate the effectiveness of the facial feature decoder.%\textcolor{red}{Why BP4D only? why not the other two datasets.}%\textcolor{red}{Why BP4D only? why not the other two datasets.}%Firstly, based on the feature encoder pretrained on FEC(Baseline-FEC), when adding the $D_f$ branch(Baseline-FEC-DF), the F1-score improves 0.5\%(from 63.3\% to 63.8\%). Further introducing the  $D_f$ and the $D_m$(Baseline-FEC-DF-DM), the results improves 2.5\%. %Firstly, based on the feature encoder pretrained on FEC(Baseline-FEC), when adding the $D_f$ branch(Baseline-FEC-DF), the F1-score improves 0.5\%(from 63.3\% to 63.8\%). Further introducing the  $D_f$ and the $D_m$(Baseline-FEC-DF-DM), the results improves 2.5\%. %we construct the model only with the Feature Encoder ~(w/o MD \& FD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC in Table~\ref{tab:F1 on Ablation}) or the Facial Decoder branch~(w/o MD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation}) individually. %a decline of 2.5\%(from 66.3\% to 63.8\%) is caused when the Mask Decoder is removed(Baseline-FEC-DF) and 3\% decline(from 66.3\% to 63.3\%) when the Facial Decoder is also removed(Baseline-FEC) respectively. %we construct the model only with the Feature Encoder ~(w/o MD \& FD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC in Table~\ref{tab:F1 on Ablation}) or the Facial Decoder branch~(w/o MD in Table~\ref{tab:F1 on Ablation 2} or Baseline-FEC-DF in Table~\ref{tab:F1 on Ablation}) individually. %a decline of 2.5\%(from 66.3\% to 63.8\%) is caused when the Mask Decoder is removed(Baseline-FEC-DF) and 3\% decline(from 66.3\% to 63.3\%) when the Facial Decoder is also removed(Baseline-FEC) respectively. %%%%%%%%%%%%%pipeline figure%%%%%%%%%%%%%pipeline figure\begin{figure}[!t]\begin{figure}[!t]    \centering  \centering    \includegraphics[ width=9cm]{images/sample1.pdf}  \includegraphics[ width=9cm]{images/sample1.pdf}    %\vspace{-0.5em}  %\vspace{-0.5em}    \caption{  \caption{Visualization of the decoded mask attention maps:(Left) samples from DISFA, and(Right) samples from BP4D and BP4D+. The learned masks(odd rows) are also visualized and overlaid on the corresponding face images(even rows). The colors covering on the face images from blue to red indicate the attention values from low to high.}}    \label{fig:figure1}  \label{fig:figure1}\end{figure}\end{figure}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%mask figure%%%%%%%%%%%%%mask figure\begin{figure*}[!t]\begin{figure*}[!t]    \centering  \centering    \includegraphics[ width=18cm]{images/sample2.pdf}  \includegraphics[ width=18cm]{images/sample2.pdf}    %\vspace{-0.5em}  %\vspace{-0.5em}    \caption{  \caption{Visualization of the mask attention maps overlaid onto the corresponding input images in BP4D. The first column shows face images with different expressions. We can observe that similar AU-related local mask distributions can be learned by our framework even though the identities and expressions vary significantly.  } }    \label{fig:mask visualization}  \label{fig:mask visualization}\end{figure*}\end{figure*}%%%%%%%%%%%%%avtivation figure%%%%%%%%%%%%%avtivation figure% \begin{figure*}[!t]% \begin{figure*}[!t]%     \centering%     \centering%     \includegraphics[ width=18cm]{images/sample3.pdf}%     \includegraphics[ width=18cm]{images/sample3.pdf}%     %\vspace{-0.5em}%     %\vspace{-0.5em}%     \caption{Visualization of the mask maps generated by different activation functions(Sigmoid, softmax, and Tanh, from top to bottom) on each AU from the BP4D dataset. The masks of softmax are more sparse than those of Sigmoid and Tanh because it has an extra restriction between AU channels. Therefore, softmax may filter out some related regions.}%     \caption{Visualization of the mask maps generated by different activation functions(Sigmoid, softmax, and Tanh, from top to bottom) on each AU from the BP4D dataset. The masks of softmax are more sparse than those of Sigmoid and Tanh because it has an extra restriction between AU channels. Therefore, softmax may filter out some related regions.}%     \label{fig:avtivation}%     \label{fig:avtivation}% \end{figure*}% \end{figure*}% %%%%%%%%%%%%%% %%%%%%%%%%%%%Note that the inclusion of DF alone(w/o DM) brings an improvement of 0.5\\%(from 63.3\\% to 63.8\\%) in comparision to w/o DM\\&DF. When the DF is replaced by the CNN module, the performance declines by 0.1\\%(from 63.8\\% to 63.7\\%). Moreover, the F1-Score improves by 2.3\\% when we further add the DM module(GLEE-Net). These study results validate the effectiveness of our attention and local feature learning.% In the experiment without pretraining on the expression dataset~(w/o pretrain), we can see an apparent drop in average F1-score of .% In the experiment without pretraining on the expression dataset~(w/o pretrain), we can see an apparent drop in average F1-score of .%\textcolor{red}{[It seems the two rows(w/o DM, and w/o DM\&DF) in Table 7 are not used/cited in the main texts. So, reviewers may question why you put the two rows in Table 7?]}\textcolor{blue}{[has been referred]}%\textcolor{red}{[It seems the two rows(w/o DM, and w/o DM\&DF) in Table 7 are not used/cited in the main texts. So, reviewers may question why you put the two rows in Table 7?]}\textcolor{blue}{[has been referred]}To explore the effect of activation functions on attention mask generation, we tried two activation methods, Sigmoid and SoftMax, on the outputs of the mask decoder. The results are shown in Table \ref{tab:F1 on Ablation 2}. %When there is no activation on the mask decoder's outputs(w. None), it achieves an F1 score of 64.1\%\ref{tab:F1 on Ablation 2}. %When there is no activation on the mask decoder's outputs(w. None), it achieves an F1 score of 64.1\%. The Sigmoid function(GLEE-Net(Full)) obtains a better result of than Softmax(w. SoftMax), improving F1-score of 2.3\\%. The possible reason is that the masks generated by Softmax tend to get sparse attention maps and exclude other parts including regions related to the target AU in most cases. This may result in the downstream recognition task being unable to learn sufficient information. In contrast, Sigmoid can avoid the above shortcoming and retain the regions that are closely related to the target AU, making the subsequent Classifier Module have a better performance. %%%%%%%%%%%%%tsne figure%%%%%%%%%%%%%tsne figure\begin{figure}[!t]\begin{figure}[!t]    \centering  \centering    \includegraphics[ width=9cm]{images/tsne.pdf}  \includegraphics[ width=9cm]{images/tsne.pdf}    %\vspace{-0.5em}  %\vspace{-0.5em}    \caption{  \caption{t-SNE visualization of the AU embeddings generated by our framework w/ or w/o the mask decoder module on the BP4D dataset. }}    \label{fig:tsne}  \label{fig:tsne}\end{figure}\end{figure}%%%%%%%%%%%%%%%%%%%%%%%%%%\subsection{\subsection{Visual Analysis}}Figure~\ref{fig:figure1}\ref{fig:figure1} visualizes the attention mask maps of several From Figure~\ref{fig:mask visualization}\ref{fig:mask visualization}, we can see that each AU's mask is closely related to its muscle region, even for different expressions such as happy, sad, and fear.\textbf{Mask Features Analysis.} The network w/o DM\\&DF is a encoder-decoder structure, based on which further adding the DF sub-module is w/o DF. To validate the importance of mask learning, we visualize the embeddings of the AU classifiers of the w/o DM\\&DF and w/o DF. We sample one thousand images and obtain the t-SNE visualization of their AU embeddings. As illustrated in Figure~\ref{fig:tsne}\ref{fig:tsne}, each color refers to a class of AU presentations. Obviously, the presentations learned with the mask decoder are more compact and have better distribution than that without the mask decoder. Moreover, all the AU embeddings learned with the mask decoder tend to gather into two clusters(positive and negative). By contrast, the presentations generated without the mask decoder display like a long strip and are not divided into two clusters for the cases of AU2, AU4, AU15, AU17, and AU23. As a result, these AUs cannot be well distinguished between positive and negative samples. This validates that the mask learning module in our framework is effective to capture discriminative local features that are beneficial to AU recognition.% \textbf{Analysis of Different Mask Activation Functions}.% \textbf{Analysis of Different Mask Activation Functions}.% Each mask  is responsible for an AU in our framework, and the mask indicates the spatial locations that are important for the recognition of the target AU. We compared three different activation functions to obtain our masks, namely, Softmax, Tanh and Sigmoid. As shown in Figure~\ref{fig:avtivation}, different activations on the outputs of the Mask Decoder bring various mask attention maps. As expected, the masks generated by the Softmax activation function are the most sparse among the three activation functions. This attribute to the restriction on the sum of all AU masks: their values must be in the range from 0 to 1, and thus reducing the overlap between masks. In comparison, the other two activation functions, Sigmoid and Tanh, can obtain a more dense map for each AU because there is no restriction between different masks. Besides, Sigmoid learns better mask maps than Tanh for the reason that its estimation value domain exactly matches the attention. Sigmoid can also capture the relation between different AUs. For instance, AU1, AU2, and AU4 activate not only the location of brows but also the mouth area, because expressions with brow movements usually accompany mouth movements in the training dataset. % Each mask  is responsible for an AU in our framework, and the mask indicates the spatial locations that are important for the recognition of the target AU. We compared three different activation functions to obtain our masks, namely, Softmax, Tanh and Sigmoid. As shown in Figure~\ref{fig:avtivation}, different activations on the outputs of the Mask Decoder bring various mask attention maps. As expected, the masks generated by the Softmax activation function are the most sparse among the three activation functions. This attribute to the restriction on the sum of all AU masks: their values must be in the range from 0 to 1, and thus reducing the overlap between masks. In comparison, the other two activation functions, Sigmoid and Tanh, can obtain a more dense map for each AU because there is no restriction between different masks. Besides, Sigmoid learns better mask maps than Tanh for the reason that its estimation value domain exactly matches the attention. Sigmoid can also capture the relation between different AUs. For instance, AU1, AU2, and AU4 activate not only the location of brows but also the mouth area, because expressions with brow movements usually accompany mouth movements in the training dataset. %\textcolor{red}{[Figure 8 is not cited anywhere in the main texts. If not cited/used in the main texts, reviewers may question why Figure 8 should be included into the paper.]}\textcolor{blue}{[has been deleted]}%\textcolor{red}{[Figure 8 is not cited anywhere in the main texts. If not cited/used in the main texts, reviewers may question why Figure 8 should be included into the paper.]}\textcolor{blue}{[has been deleted]}

==> introduction_bk.tex <==
\else
\section{Introduction}
\label{sec:introduction}
\fi
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

\IEEEPARstart{F}{acial} Behavior Analysis is an active research area in computer vision and affective computing communities. As a universal non-verbal approach to carrying out human communication, facial expressions can be described via a combination of Facial Action Units (AUs)~\cite{FACS}. Facial AUs, coded by the Facial Action Coding System (FACS)~\cite{FACS}, include 32 atomic facial action descriptors based on anatomical facial muscle groups. Each AU defines the movement of a specific face region. For example, AU1 (Inner Brow Raiser) is a descriptor focused on the medial part of frontalis. Generally, they are combined together to represent different full facial expressions. Table \ref{tab:AUs definition} summarizes the information of the 15 AUs used in this paper, including their names and corresponding involved muscles. %AUs are a set of descriptors of facial muscle movements focused on local facial actions.  %They are closely related even though they represent facial behavior in two different levels. 
As AUs play an important role in conveying human emotions and automatic expression analysis, in recent years AU detection has attracted numerous attentions due to its wide application, including emotion recognition \cite{AU4EmoctionRecog}, micro-expression detection \cite{AU4MicroExpression}, and mental health diagnosis \cite{AUD4diagnose}. 

Up to date FACS has been widely regarded as the de facto standard for annotating facial expressions, because it can describe nearly any possible expressions as a specific combination of facial AUs. For instance, as shown in Figure~\ref{fig:AU emotion}, happiness can be achieved with the occurrences of both AU6 and AU12; a doubt expression is related to AU4; and a surprise expression is related to AU1 and AU26. From this perspective, AU features are often considered as a facial expression representation. Considering the relation of expression and AUs, expression recognition has also been introduced to enhance AU recognition task\cite{cui2020knowledge}\cite{liu2015inspired}. However, these works regard expression simply as several discrete classes, do not 
  


\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/figure1.PNG}
    %\vspace{-0.5em}
    \caption{Examples of three expressions and their corresponding AUs. From left to right: doubt, happiness, surprise. Expression is a global description of the face muscle movements, while AUs refer to individual local description of muscle motion.}
    \label{fig:AU emotion}
\end{figure}
%%%%%%%%%%%%%

%Considering the relation of expression and facial action units, several work utilize them to complement each other ~\cite{}~cite\{}.
%考虑到表情与AU存在的这种全局与局部的关系，一些工作将表情分类任务引入AU检测工作作为辅助。然而表情分类仅仅只能涵盖几个离散的表情类别，无法表示表情的连续变化.
%%%%%%%%%%%%%AU emotion figure

With the aid of recent advances on deep learning, numerous approaches have been proposed to improve AU detection performance in recent years. As a facial AU is defined anatomically according to the movements of its related facial muscles, it is inherently related to local facial regions, termed as {\it AU's locality}. To this end, how to effectively extract local features and capture the locality from an input face image is a key yet challenging problem. The most straightforward approach is to divide the input image into several local parts in a pre-defined way, which are then fed into networks to capture local information, known as patch learning~\cite{Zhong2015Patch}\cite{liu2014feature}\cite{Onal2019D-PAttNet}. These methods pre-define AU local regions with prior knowledge, cropping face images into several regular yet coarse-grained patches. Subsequently, the feature extractor is limited to the quality of cropped patches. %AU local representation is captured by individual CNN networks and a self-attention mechanism is then introduced to weight the importance of each branch when detecting specific AUs. 

Another category of approaches is to utilize structured geometric information like landmarks to crop more fine-grained local partitions or obtain Regions Of Interest (ROIs). For instance, selecting a sparse subset of facial patches centered around facial landmarks through joint patch and multi-label learning~\cite{zhao2015joint}, or partition the input face image into a fixed number of basic AU-related ROIs with the help of prior domain knowledge~\cite{liu2020relation}. However, facial action units appear in specific but not limited to landmark points in most cases. Thus predefined AU regions or centers in a uniform way (either by landmarks or prior domain knowledge) are usually error-prone. \textcolor{red}{For example, many prior AUs patches generation progresses are fixed for various head poses, while landmark detection tends to deviate under large head rotation, leading to inaccurate AU patches\cite{Onal2019D-PAttNet}. } %instead of directly taking landmark points or offsets as AU centers,  Ma \textit{et al.} \cite{ma2019r} adopt an elaborate partition rule to reduce the influence of inaccurate landmark positioning.
%Zhao~\textit{et al.}~\cite{zhao2015joint} select a sparse subset of facial patches centered around facial landmarks through joint patch and multi-label learning, and model dependencies not only on AUs but also on features. Liu ~\textit{et al.}~\cite{liu2020relation} partition the input face image into a fixed number of basic AU-related ROIs, taking advantage of prior domain knowledge and landmarks. These AU-specific regions are encoded into informative representation vectors through a series of auto-encoders. Then, a GCN module is used to model the AU relationships and obtain assembled features for downstream detection tasks. Considering that AUs appear in specific but not limited to landmark points, instead of directly taking landmark points or offsets as AU centers,  Ma \textit{et al.} \cite{ma2019r} adopt an elaborate partition rule to reduce the influence of inaccurate landmark positioning. AUs are segmented to groups according to FACS and related muscles, and the AUs in each group share the same ROI regions and mask.
Furthermore, attention learning is also an effective way to extract local information.  Some recent works\cite{li2018eac}\cite{shao2021jaa}\cite{jacob2021facial} focus on learning attention maps by facial landmarks in a supervised manner. The attention maps are usually initialized by predefined AU centers based on landmarks and treated as truths during training. Analogously, the attention learned by these methods are still limited by landmarks position. To summarise, these approaches are sub-optimal on two aspects. First, pre-defined AU centers by domain knowledge and landmarks are limited to landmark position and the pre-define rules\cite{}. Second, the landmark detection errors often influence the final performance\cite{}.
%tend to \textcolor{blue}{focus on regions that author rather than network expected in some cases.} 
%\textcolor{red}{[Deng: difficult to understand this part]}
%Other auxiliary information such as text description has also been exploited to generate AU attention maps \cite{yang2021exploiting}.
%\textcolor{red}{[Deng: the above two paragraphs basically describe some of the previous approaches on AU detection. Questions: (1) the above three paragraphs are somehow duplication of some writing in the related work section? If so, such repeating should be reduced if possible. (2) Maybe these paragraphs in the introduction section should focus on why the previous approaches are not sufficient (i.e., what are their limitations), and/or what are the issues in the detection results by previous approaches? For example, those approaches will fail on what kind of cases?]}

%\textcolor{red}{We have to specify existing challenges here. The challenge introduction is helpful for the description of careful-designed framework.}
AU detection is still challenging due to the lack of annotated data and difficulty in capturing local features. Annotation of action units needs a well-trained expert taking hours of time to label one hundred images manually\cite{zhi2020comprehensive}. Therefore, it is time-consuming and laboring to get large scale well-annotated AUs data\cite{peng2018weakly}\cite{niu2019multi}. The lack of labeled data often makes the training of deep network tends to suffer from the data overfitting. On the other hand, the AU dataset contains limited identities, dozens or hundreds usually, which may lead to the identity overfitting\cite{xiang2017linear}\cite{LP}. Besides, learning expressive local feature is hard because the local facial deformations are not only very subtle and transient \cite{zhi2020comprehensive}\cite{granger2021weakly}, but also vary with each individual\cite{xiang2017linear}\cite{LP}. 
%Researchers have made great effort to promote the feature learning, including patch learning\cite{} and attention learning. 

%Large amounts of unlabeled or  inaccurate annotated data is not well utilized.
By comparison, there are amounts of accessible and easy-to-annotate expression data, which is beneficial for improving AU detection performance~\cite{peng2018weakly}\cite{niu2019multi}\cite{xiang2017linear}. Additionally, as mentioned above, capturing local features based on manually predefined rules with coarse guidance may limit the capability of the local feature extractor. To this end, the sensitive position of each AU in the face feature maps should be depended on the AU detection task and the training dataset. In other words, the attention map learning progress should be data-driven. 

Motivated by the above observation, combining the relation between facial expression representation and AU detection, we consider addressing this problem by learning attention map adaptively without extra supervision. We first pretrain a facial expression representation encoder to extract identity-invariant global expression features on a large-scale emotion dataset, FEC~\cite{vemulapalli2019compact}. Instead of roughly classify expressions into several discrete categories, we project expression into continuous representation space, which is a more suitable and better choice for enhancing AU detection task because AU is also subtle and continuous. Secondly, two decoders are constructed to decode facial attention maps and global features for each AU respectively. The attention map decoder is learned without any intermediate supervision. In other words, the attention only depend on the input data. The facial feature maps are next multiplied by the attention mask, filtering out irrelative fields and retaining informative ones. 

To sum up, the contributions of this paper can be summarized as following:
\begin{itemize}
    \item [(1) ]
    An expression representation learning approach is utilized to pretrain the feature encoder with structured triplet data. This step is proved to be essential for improvement on AU recognition. To our knowledge, this is the first work of introducing expression feature learning through triplet into AU detection.
    \item [(2) ]
    An effective attention learning method by two-branch CNN decoder is proposed to capture AU-related representation, which is crucial in getting more informative local features and boosting up AU detection performance. Visualization analysis proves that it can produce highly AU-related local region mask adaptively.
    \item [(3) ]
    Validated by extensive experiments, the proposed method gets impressive improvement on three widely-used benchmark datasets, outperforming the state-of-art significantly.  
\end{itemize}

The rest of this paper is organized as follows. Related works are presented in section 2. The details of our method design are introduced in section 3. Intensive experiments are reported in section 4. Section 5 provides a series of visualize analysis and section 6 is the eventual conclusion of this article.
% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol

\begin{table}[!t]
%\small
\footnotesize
\setlength{\tabcolsep}{1.5pt} 
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{AU definitions in FACS of description and the corresponding muscles involved. }
  \vspace{-1em}
  \label{tab:AUs definition}
 \begin{tabular}{l|cccccccccccc|c}
    \hline
   \textbf{AU Name} &\textbf{AU Description} &\textbf{Facial Muscle} \\[1pt]
    \hline\hline
    AU1   &Inner Brow Raiser &Frontalis, pars medialis     \\
    AU2   &Outer Brow Raiser &Frontalis, pars lateralis       \\
    AU4   &Brow Lowerer     &Depressor Glabellae\\
    AU6   &Cheek Raiser     &Orbicularis oculi \\
    AU7   &Lid Tightener     &Orbicularis oculi\\
    AU9   &Nose Wrinkler     &Levator labii superioris alaquae nasi\\
    AU10  &Upper Lip Raiser  &Levator Labii Superioris \\
    AU12  &Lip Corner Puller &Zygomatic Major  \\
    AU14 &Dimpler &Buccinator\\
    AU15 &Lip Corner Depressor &Depressor anguli oris\\
    AU17 &Chin Raiser &Mentalis\\
    AU23 &Lip Tightener &Orbicularis oris\\
    AU24 &Lip Pressor &Orbicularis oris\\
    AU25 &Lips part &Depressor labii inferioris \\
    AU26 &Jaw Drop &Masseter\\
    \hline
  \end{tabular}}
\end{table}

%%%%%%%%%%%%%pipeline figure
\begin{figure*}[!t]
    \centering
    \includegraphics[ width=18cm]{images/pipeline2.pdf}
    %\vspace{-0.5em}
    \caption{An overall illustration of our proposed global-to-local expression-aware embeddings AU detection framework. It is composed with five modules: Feature Encoder, Mask Decoder, Feature Decoder, Mask Components and AU classifier. The Feature Encoder is pretrained by expression similarity task with the triplet loss and extracts a global expression feature map from the input image, which is capable of sensing subtle expression changes. The global feature is then fed into the Mask Decoder and the Feature Decoder. The two decoders decode AU attention mask and facial feature map from the global expression feature respectively. AU-related local feature is got by pixel-wise product on the outputs of two decoders, which is fed into the following AU Classifier to get the AU embedding and detection result.}
    \label{fig:pipeline}
\end{figure*}
%%%%%%%%%%%%%

==> method_bk.tex <==
\section{Proposed Method}
% 目前的写法更多像是内部的工作汇报，描述了怎么做，但是没有交代为什么这么做
%1. 问题定义，problem definition,采用数学的语言formalution；
%2. 主要解决了存在的哪几个挑战（比如：图像表征+自适应注意力）；
%3. 然后才是说这个章节的overview,先后每节说什么说什么；

As described in section 1, expression and AUs are two means of description from global and local level respectively. They are highly relative thus can be utilized to promote each other. Moreover, facial expression data is quite easier to obtain because it is a coarse-grained perception of facial emotion, unlike AUs which is more subtle and difficult to annotate. Intuitively, facial action unit information can be decoded form facial expression representation. In consideration of above factors, we firstly pretrain a feature extractor on a large scale facial expression dataset, aiming at obtaining a strong and robust expression feature extractor. For the purpose of capturing AU local features, we construct two branch of decoders, namely facial mask decoder(DM) and facial feature decoder(DF). They separately capture the local attention mask maps and facial features. After an element-wise multiplication in per channel on the outputs of the above two decoders , we obtain the the local feature map more concentrating on AU-related regions. Eventually, these local features are further fed into AU classifiers to get AU embeddings and detection results individually. In the following subsections, we discuss each proposed module in detail.

\subsection{Pre-trained Feature Extractor}
To enhance the model generalization, we introduce the compact and continuous expression embedding~\cite{vemulapalli2019compact,zhang2021learning} as the prior auxiliary information. In practical, we pre-trained our feature extractor on the expression similarity task~(See Fig. ) using the FEC dataset~\cite{vemulapalli2019compact}. The FEC dataset contains numerous facial image triplets along with the annotations 
indicating which one has the most different expression in each triplet. 
We pre-trained the feature extractor using the triplet loss to constrain the more similar expressions has a closer embedding distance.
In each triplet, we call the image with the most different expression as the Negative~($N$) and the other two images as the Anchor~($A$) and Positive~($P$), respectively. For a triplet~(A,P,N), our feature extractor outputs three expression embedding $E_{A}$, $E_{P}$ and $E_{N}$. The pre-trained training process utilize the triplet loss as follows:
\begin{equation}\small
\begin{aligned}
\mathcal{L}_{tri} &=\max(0,\|E_{A}-E_{P}\|_2^2-\|E_{A}-E_{N}\|_2^2+m) \\
                  &+\max(0,\|E_{A}-E_{P}\|_2^2-\|E_{P}-E_{N}\|_2^2+m) .
\end{aligned}
\end{equation}
Due to the large number of triplets, the pre-trained feature extractor can produce the compact and identity-invariant expression representation, which is beneficial for the downstream expression related tasks like AU detection.  

We choose the structure of DLN~\cite{zhang2021learning} as our feature extractor.  DLN~\cite{zhang2021learning} models the expression feature as the difference of the full face feature vector and the identity feature vector. After the dimensionality reduction, it output a 16-dimensional vector as the expression embedding. We pre-trained the feature extractor and reserve the networks before the last layer to finetune the AU detection. 

% Specifically, DLN~\cite{zhang2021learning} models the expression feature as the difference of the full face feature vector and the identity feature vector. After the dimensionality reduction, it output a 16-dimensional vector as the expression embedding.
% Since the deviation structure of DLN~\cite{zhang2021learning} is not fit in our framework, a InceptionResnet~\cite{schroff2015facenet} distilled from the pretrained DLN~\cite{zhang2021learning} is employed as the feature extractor of our framework based on the distillation mechanism~\cite{hinton2015distilling}. Then our whole framework including feature extractor is finetuned for AU detection.
% 可能要写一下具体用了哪前几层 @rudong
Our intuition is that the parameters initialized from expression embedding instruct
the AU detection framework to capture the more effective expression features at the beginning of training, which helps relieve the problem of the overfitting caused by the limited identities of AU datasets. 

\begin{figure}[!t]
    \centering
    \includegraphics[ width=9cm]{images/tri.pdf}
    %\vspace{-0.5em}
    \caption{Illustration of our pre-trained expression similarity task. In each triplet, Anchor and Positive have the more similar expressions than Negative. By the triplet loss, the pre-trained feature extractor minimizes the distances between the Anchor's and Positive's expression embedding and maximizes the distances between the Anchor's and Negative's, Positive's and Negative's expression embedding. }
    \label{fig:triplet_loss}
\end{figure}

% \subsection{Facial Decoder}
% \subsection{Mask Decoder}
\subsection{Facial Components}
% \ZH{asdad}
%% why multiple RGB
% 这么开始写，读者审稿人是看不懂的，需要交代这么设计的motivation
%%% FCM: why multiple RGB branches and multiple mask branches.
%%% 1. 
% Due to the local definition of the AUs, we design a Facial Component Module to separate the whole face into AU-related local parts. 

% The Facial Component Module consists of a facial feature decoder (DF) and a facial mask decoder (DM). The two decoders share the same Feature Extractor that captures global facial features. With the extracted features, DF aims at generating multiple facial components (eg. eyes, mouths, etc) and DM tries to produce multiple component masks that are used to mask out irrelevant areas for each facial component.
% \ZH{To add decoder}
The expression feature extracted by the pre-trained feature extractor describes the facial movements globally. However, this global representation is not suitable for the subsequent AU detection task, since AUs are defined locally and different AUs are independent of each other. Therefore, it is more natural to extract local fine-grained features for each AU independently. To achieve this goal, we design a Facial Component Module to transform the global expression feature to local AU-related representations. 
% The generated facial components are then sent to AU Classifier for fine-grained feature capturing and AU detection.

Specifically, we first decode the global expression feature to facial components with our designed facial feature decoder. Each component represents a special facial part (eg. eyes, mouth etc.) that is related to a specific AU. However, we find that the facial component generated by the facial feature decoder may contain information from unrelated AUs, so we introduce a facial mask decoder which can focus more on the region of interest of each AU and mask out irrelevant contents. Moreover, we apply a face reconstruction task to avoid information loss during facial components generation.

\textbf{Facial Feature Decoder.} 
The facial feature decoder aims at generating facial components from the global feature. Given the global feature $h$, our facial feature decoder ($D_f$) performs as:
\begin{equation}
[f^1, f^2,...,f^N]= D_f(h),
\end{equation}
where $f^k \in \mathbb{R}^{3\times H \times W}$ is the $k_{th}$ facial component that is related to the $k_{th}$ AU, and $N$ is the total number of all AUs.



% Considering AUs are various in structures and textures, different AU components are better to be predicted with different filters. Therefore, we design the facial feature decoder to predict multiple facial contents with multiple prediction heads instead of one. Each head, which consists of a convolutional layer and an activation layer, is responsible for predicting facial contents related to an independent AU.
% To accurately generate facial components for each AU, we introduce a facial feature decoder (DF) and a facial mask decoder (DM) into the Facial Component Module. DF aims at generating facial contents(eg. eyes, mouths, etc) and DM tries to find the region of interest of each AU and mask out irrelevant contents. 

\textbf{Facial Mask Decoder.} 
The facial feature decoder aims at generating facial component masks from the global feature. Each mask represents the region of interest of each AU. Given the global feature $h$, the component masks are predicted as:
\begin{equation}
[m^1, m^2,...,m^N]= D_m(h),
\end{equation}
where $m^k \in \mathbb{R}^{1\times H \times W}$ is the $k_{th}$ facial mask for the $k_{th}$ AU. 

% The whole procedure of our Facial Component Module can be formulated as follows. First, the facial contents are obtained by DF:
% \begin{equation}
% [f^1, f^2,...,f^N]= DF(h),
% \end{equation}
% where $h$ is the global facial feature extracted by the Feature Extractor, $f^k \in \mathbb{R}^{3\times H \times W}$ is the $k_{th}$ facial component that is related to the $k_{th}$ AU, and $N$ is the total number of all AUs. Then the facial masks are predicted by DM:


To ensure that the values of the predicted facial masks lie in a fixed range of 0 to 1 (0 indicates no attention and 1 means the strongest attention), an activation function is added to the last layer of the DM.
% The DM includes an activation function at last, which projects the mask matrix values to a fixed range of 0 to 1, where 0 indicates no attention and 1 means the strongest attention in this spatial location.
% Intuitively, Sigmoid and SoftMax are both suitable for this purpose. SoftMax constrains each AU to form a mutually exclusive relationship on account of .... In consideration of the existing dependence between different AUs, Sigmoid is better for reserving this relationship.
%zh 
Intuitively, Sigmoid and Softmax are both suitable for this purpose. Softmax activation is applied channel-wise to all N facial masks so that the elements of the N masks sum to 1. It is based on an assumption that AUs are mutually exclusive from each other. Sigmoid activation is applied to each facial mask independently, it assumes that there exists dependence between different AUs. To explore the relationship between AUs, we try both two activations in this work.


\textbf{Reconstruction.} 
Finally, the facial components are generated by multiplying the face contents and the facial masks:
% the facial images are multiplied with the facial masks and the final facial components are generated by:
\begin{equation}
[c^1, c^2,...,c^N]= [m^1 \times f^1, m^2\times f^2,...,m^N\times f^N],
\end{equation}
where $C^*$ are computed facial components which are then used for the subsequent AU detection task.

Comparing to existing works, there are two key points of designing the Facial Component Module: (1) We adopt two different decoders to predict facial images and facial masks, respectively. Unlike previous methods~\cite{?} that produce images and masks in one decoder, the separate design means that parameters in each decoder are only responsible for only one task, thus benefiting for the network training. (2) The facial decoder and mask decoder generate multiple facial images and multiple facial masks simultaneously. In contrast to existing methods~\cite{?} that generate only one facial image and multiple masks, our multiple facial images with multiple masks can model more complex AU combinations.

%%%%%%%BP4D%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*} 
\footnotesize
%\small
\renewcommand\arraystretch{1.5} 
\centering
{
  \caption{Comparisons of our method and the state-of-the-art methods on BP4D in terms of F1 scores (\%). The best results are shown in bold, and the second best are in brackets.}
  \vspace{-1em}
%   \vspace{-1em}
  \label{tab:F1 on Bp4D}
  %\setlength{\tabcolsep}{1.5mm}{
  \begin{tabular}{l|cccccccccccc|c}
    \hline 
   \textbf{Method} &\textbf{AU1} &\textbf{AU2} &\textbf{AU4}&\textbf{AU6}&\textbf{AU7}&\textbf{AU10}&\textbf{AU12}&\textbf{AU14}&\textbf{AU15} &\textbf{AU17} &\textbf{AU23} &\textbf{AU24} &\textbf{Avg.}\\[1pt]
    \hline \hline 
    LSVM    &23.2 &22.8 &23.1 &27.2 &47.1 &77.2 &63.7 &64.3 &18.4 &33.0 &19.4 &20.7 &35.3 \\
    JPML    &32.6 &25.6 &37.4 &42.3 &50.5 &72.2 &74.1 & 65.7 &38.1 &40.0 &30.4 &42.3 &45.9\\
    DRML    &36.4 &41.8 &43.0 &55.0 &67.0 &66.3 &65.8 &54.1 &33.2 &48.0 &31.7 &30.0 &48.3\\
    EAC-Net &39.0 &35.2 &48.6 &76.1 &72.9 &81.9 &86.2 &58.8 &37.5 &59.1 &35.9 &35.8 &55.9\\
    % ROI     &36.2 &31.6 &43.4 &77.1 &73.7 &85.0 &87.0 &62.6 &45.7 &58.0 &38.3 &37.4 &56.4\\
    %JAA-Net &47.2 &44.0 &54.9 &7 7.5 &74.6 &84.0 &86.9 &61.9 &43.6 &60.3 &42.7 &41.9 &60.0\\
    DSIN    &51.7 &40.4 &56.0 &76.1 &73.5 &79.9 &85.4 &62.7 &37.3 &62.9 &38.8 &41.6 &58.9\\
    ARL     &45.8 &39.8 &55.1 &75.7 &77.2 &82.3 &86.6 &58.8 &47.6 &62.1 &47.4 &55.4 &61.1\\
    LP-Net  &43.4 &38.0 &54.2 &77.1 &76.7 &83.8 &87.2 &63.3 &45.3 &60.5 &48.1 &54.2 &61.0\\
    AU-GCN &46.8 &38.5 &60.1 &[80.1] &79.5 &84.8 &88.0 &67.3 &52.0 &63.2 &40.9 &52.8 &62.8 \\
    SRERL   &46.9 &45.3 &55.6 &77.1 &78.4 &83.5 &87.6 &63.9 &52.2 &63.9 &47.1 &53.3 &62.9\\
    AU-RCNN &50.2 &43.7 &57 &78.5 &78.5 &82.6 &87 &67.7 &49.1 &62.4 &50.4 &49.3 &63.0 \\
    UGN-B   &54.2 &46.4 &56.8 &76.2 &76.7 &82.4 &86.1 &64.7 &51.2 &63.1 &48.5 &53.6 &63.3\\
    J{\^A}A-Net &53.8 &47.8 &58.2 &78.5 &75.8 &82.7 &[88.2] &63.7 &43.3 &61.8 &45.6 &49.9 &62.4\\
    MHSA-FFN &51.7 &[49.3] &[61.0] &77.8 &\textbf{79.5} &82.9 &86.3 & \textbf{67.6} &51.9 &63.0 &43.7 &\textbf{56.3} &64.2\\
    SEV-Net &\textbf{58.2} &\textbf{50.4} &58.3 &\textbf{81.9} &73.9 &\textbf{87.8} &87.5 &61.6 &[52.6] &62.2 &44.6 &47.6 &63.9\\
    HMP-PS &53.1 &46.1 &56.0 &76.5 &76.9 &82.1 &86.4 &64.8 &51.5 &63.0 &[49.9] &54.5 &63.4\\
    CaFNet &[55.1] &49.3 &57.7 &78.3 &78.6 &[85.1] &86.2 &[67.4] &52.0 &[64.4] &48.3 &[56.2] &[64.9]\\
    \hline
    Ours  &\textbf{58.2} &48.7 &\textbf{61.5} &78.7 &[79.2] &84.2 &\textbf{89.8} &66.3 &\textbf{56.7} &\textbf{64.8} &\textbf{53.5} &53.6 &\textbf{66.3}\\
    %Ours  &[57.8] &45.3 &\textbf{61.1} &[80.0] &[78.6] &[85.6] &[87.9] &\textbf{68.2} &[52.3] &[63.8] &[49.0] &\textbf{56.8} &\textbf{65.5}\\
    \hline
  \end{tabular}}
  %}
\end{table*}

\subsection{AU Classifier}
Since the outputs of the Facial Components are a seris of RGB feature maps in a resolution of 256x256, of which the number equals to the number of AU in the dataset. So the following AU classifer module, indicated as $g^i(\cdot)$, is designed to a muti-layer CNN architecture, which contains 6 convolution blocks and a global average pooling layer. For the first five convolution layer, each convolution is followed by a batchnorm and a ELU activation function and the output channels of them are set to {16, 32, 64, 128, 256} respectively. To make sure the sub-module has a wide receptive field, these five CNN kernel size, stride and padding is seted to 7, 2 and 3 respectively.  The global average pooling layer is set after the fifth convolution block, aiming to aggregate the feature map into AU Embedding. In this way, more pure information closely related to the specific AU will be extracted from the input RGB component feature map. After that, the AU embeddings are fed into the last convolution layers, whose output channel, kernel size, stride and padding are all set to 1. This procedure can be formulated as the following function:
\begin{equation}
[y^1, y^2,...,y^N]= [g^1(c^1), g^2(c^2),...,g^N(c^N)].
\end{equation}
The $y^i$ indicates the output of the last convolution layer of i-th AU. To get the final prediction of AU's probability, we use a Sigmoiod activation on the $y^i$ and get the eventual prediction $o^i$:
\begin{equation}
[o^1, o^2,...,o^N]= [\sigma(y^1), \sigma(y^2),...,\sigma(y^N)].
\end{equation}

\subsection{Loss Function}
As illustrated in Figure~\ref{fig:pipeline}, our proposed framework referred two tasks, namely, AU detection and facial image reconstruction. So the training loss $E_{total}$ contains two parts:
\begin{equation}
E_{total} = E_{au} + \lambda E_{rec}.
\end{equation}
Where $E_{au}$ is the AU classification loss and $E_{rec}$ refers to the facial image reconstruction loss. $\lambda$ is a hyperparameter for adjusting the loss ratio. AU detection is usually regarded as a multi-label binary classification problem, so the AU detection loss is defined as:
\begin{equation}
E_{au} = -\sum_{i=1}^{N} [p_i log \hat{p}_i + (1 - p_i) log(1-\hat{p}_i)].
\end{equation}

Where $N$ is the num of AU classes. $p_i$ is the predicted probability and $\hat{p}_i$ is the ground truth of the $i_{th}$ AU. As for the image reconstruction, we use a pixel-level MSE loss between the input image and the reconstructed image:
\begin{equation}
E_{rec} = -\frac{1}{2} \sum_{i=1}^{n}(|| y_i - \hat{y}_i ||^2_2).
\end{equation}

Where the $n$ is the num of image pixels and equals to $h_{img}$ \times $w_{img}$. Besides, $\hat{y}_i$ and $y_i$ are the $i_{th}$ pixel truth value of input image and reconstruction value respectively.


